Distributed Weighted Min-Cut in Nearly-Optimal Time

Minimum-weight cut (min-cut) is a basic measure of a network's connectivity strength. While the min-cut can be computed efficiently in the sequential setting [Karger STOC'96], there was no efficient way for a distributed network to compute its own min-cut without limiting the input structure or dropping the output quality: In the standard CONGEST model, existing algorithms with nearly-optimal time (e.g. [Ghaffari, Kuhn, DISC'13; Nanongkai, Su, DISC'14]) can guarantee a solution that is $(1+\epsilon)$-approximation at best while the exact $\tilde O(n^{0.8}D^{0.2} + n^{0.9})$-time algorithm [Ghaffari, Nowicki, Thorup, SODA'20] works only on *simple* networks (no weights and no parallel edges). Here $n$ and $D$ denote the network's number of vertices and hop-diameter, respectively. For the weighted case, the best bound was $\tilde O(n)$ [Daga, Henzinger, Nanongkai, Saranurak, STOC'19]. In this paper, we provide an *exact* $\tilde O(\sqrt n + D)$-time algorithm for computing min-cut on *weighted* networks. Our result improves even the previous algorithm that works only on simple networks. Its time complexity matches the known lower bound up to polylogarithmic factors. At the heart of our algorithm are a clever routing trick and two structural lemmas regarding the structure of a minimum cut of a graph. These two structural lemmas considerably strengthen and generalize the framework of Mukhopadhyay-Nanongkai [STOC'20] and can be of independent interest.

==> 1.5-technical-overview.tex <==
%\mtodo{These are some challenges that can be discussed before technical overview. One is that the previous algorithm requires linear number of queries, hence it is not clear how to use it to get a *sub-linear* complexity. The main challenge in a distributed setting is to break the problem into many smaller problems that we can solve in parallel. A natural candidate for this is to break the problem into short sub-paths. Now while comparing two short paths can indeed be done in a time proportional to the length of paths, the main challenge to get a fast algorithm is to find a decomposition where each short path only participates in small number of computations. While the previous algorithm could bound the number of computations each edge participates in, as now our main building block is a path, we would like to be able to bound the number of computations each path participates in. This is problematic, as we may have cases where a path "is interested" in many different paths (maybe we can add here the figure we have with an example of this case). To overcome it, we show that if we restrict our attention to paths that have a nice structure we can indeed bound the number of computations, and we show how to decompose the problem to paths that satisfy this nice structure - I guess some examples for it would be discussed in technical overview, so probably no need to explain in detail the structure here.}

\section{Technical Overview}\label{sec:overview}

As discussed above, our goal is to solve the min 2-respecting cut problem, i.e., given a tree $T$ find two tree edges $e,e'$ such that the cut obtained by removing them from the tree is minimal. We denote by $\cut(e,e')$ the cut value defined by $e,e'$. 
The starting point of our algorithm is the following observation. If we only want to find the min 2-respecting cut where $e,e'$ are in two short paths $P,P'$, we can actually solve it in a time which is proportional to the length of the paths (see Section \ref{sec:alg_short_path}). The high level intuition for the algorithm is as follows. If we fix an edge $e \in P$, and want to find an edge $e' \in P'$ such that $\cut(e,e')$ is minimal, we can show that most of the computation needed for this task is to run an aggregate computation in $P'$, that intuitively allows to sum the cost of edges crossing the cut.\sagnik{What does it mean to do aggregate computation in a path path $P'$?} \mtodo{added some clarification, feel free to edit if it's not clear.} If we want to do it for all edges $e \in P$, we can pipeline multiple such computations and get a complexity which is proportional to the length of the paths. Note that most of the computation described is done only in one of the paths, $P'$, and we will exploit this asymmetry in our algorithm.
But here we only discussed two short paths. To get a fast complexity for the whole algorithm, our goal is to be able to decompose our tree into many short paths and show that each path only participates in small number of computations. For this, we use several different ingredients that we review next.
\yuval{Reviewer suggested to replace the second to last sentence with: `` To solve the min 2-respecting cut problem we possibly need to process many
pairs of such short paths. We show that we can decompose the tree into many
short paths and each path participates only in small number of computations,
which in turn allows us to design a fast algorithm that processes all the
necessary pairs of paths we need to process in order to solve the min
2-respecting cut problem." I support this, any other thoughts?}

\paragraph{First step: Decomposition.}
First, we bring into our construction a decomposition of the tree into fragments described in \cite{ghaffari2016near,Dory18} (see Section \ref{ssec:-decompFragment}).  At a high-level, we decompose our graph into $O(\sqrt{n})$ edge-disjoint fragments of diameter $O(\sqrt{n})$. Each fragment $F$ has a very specific structure: it has one main path, called the \emph{highway} of the fragment, between two vertices that are called the root $r_F$ and descendant $d_F$ of the fragment, and additional sub-trees attached to it, which are contained inside the fragment. The paths in these sub-trees are called \emph{non-highways}. The only vertices that may be connected directly to other fragments are $r_F$ and $d_F$. While many distributed algorithms use fragment decompositions, this specific decomposition has the following nice properties that are crucial for our algorithm:
%The following properties are useful for us later:
\begin{enumerate}
\item Non-highways have small length and are completely contained in one fragment.
\item We have $O(\sqrt{n})$ different highways.
\end{enumerate}

\yuval{In the paragraph above, as a reviewer suggested, I moved the sentence ``while many distributed algorithms.." to the end of the paragraph.}
When we look for the min 2-respecting cut, we break into cases according to whether the edges $e,e'$ are part of a non-highway or a highway. But first, we need an additional ingredient. %we next describe briefly how we deal with each one of these cases. 

%\mtodo{I've added here a short description of the interesting paths part. I'm not sure in what detail you want to discuss this in intro and in what detail to discuss it here, so one option is to move this or some part of it before technical overview if it fits there better. Also, feel free to edit.}

\paragraph{Second step: Finding and Bounding Interesting Paths.}
Another crucial ingredient in our algorithm is the notion of \emph{interesting paths}, which is based on and extends ideas from \cite{mukhopadhyay2019weighted}. In a nutshell, for each edge $e$ we can show that there is only a small number of ancestor to descendant paths that may contain the edge $e'$ that minimizes $\cut(e,e')$. We call these paths \emph{interesting paths} with respect to $e$. In addition, we can identify interesting paths using sampling, where the high-level intuition for this is that there are many edges that go from the subtree below $e$ towards these paths, which can be identified using sampling (see the beginning of Section \ref{sec:lemma_and_samp} for a more detailed description). This is useful for bounding the number of paths each edge should be compared to.
However, as the main building block in our algorithm is a path and not an edge, we actually need to bound the number of comparisons between different sub-paths, and not between an edge and a path. This turns out to be challenging, as there are examples where each one of the edges of a path is interested in a different path, in such cases we cannot bound the number of comparisons needed. To overcome it, we show that if we only focus on paths that have some nice structure, we can actually bound the number of paths a path is interested in, where a path $P$ is interested in a path $P'$ if one of the edges in $P$ is interested in $P'$. We next describe the intuition for a very simple case of a spider graph, similar ideas work also for more general cases.

Assume we have a spider graph: we have a root $r$ and attached to it there are $k=\sqrt{n}$ paths $P_1,...,P_k$ of length $\sqrt{n}$. For each one of these paths, we want to bound the number of other paths it is interested in. The intuition is simple, if some edge $e \in P_i$ is interested in some path $P_j$ it means that the total cost of edges going from the subpath $P_e$ of $P_i$ below $e$ towards $P_j$ is large, and is at least half of the cost of edges that goes from $P_e$ towards any of the other paths $P_{i'}$ for $i' \neq i$. Now we start scanning the path $P_i$ from the lowest edge to the highest, and stop each time we find some edge $e$ that is interested in some new path $P_j$, each time we reach such edge $e$, there is a large fraction of edges that goes from $P_e$ to $P_j$, we use it to show that after we reach a constant number of such edges the total cost of edges going from $P_e$ to any other path $P_i'$ for $i' \neq i$ grows by a constant factor (note that for any edge $e'$ below $e$, $P_{e'}$ is contained in $P_e$, hence all edges going from $P_{e'}$ towards other paths also go from $P_e$ to other paths). Since the total cost of edges is polynomially bounded it can only grow by a constant factor logarithmic number of times, which shows that $P_i$ can be only interested in $O(\log n)$ different paths.

One issue in implementing this idea, is that we cannot really identify the actual paths an edge is interested in, but rather find a small set of paths that contains the ones an edge is interested in but also other paths. We call them the paths $e$ is \emph{potentially interested} in. We show that these paths still satisfy nice properties, that allow to bound the total number of paths a path is potentially interested in. For simplicity of presentation, in the technical overview we refer to all these paths as paths $e$ is interested in. We next describe how we use these ideas in our algorithm.
At a high-level, we use the specific structure of the fragment decomposition together with a certain layering to bound the number of highway and non-highway paths each path is potentially interested in.

\paragraph{Third step: Finding the min 2-respecting cut.}
After computing the fragment decomposition and interesting paths, we now describe how we find the min 2-respecting cut. We divide into cases, according to whether the edges defining the cut are part of a non-highway or a highway and discuss additional ingredients needed for the different cases, such as \emph{layering decomposition} and \emph{monotonicity}.

\paragraph{Both edges are in non-highways.} Here our goal is to exploit the small length of non-highways to get a fast algorithm. As discussed above if we only want to compare two paths of small length we can do it in a complexity which is proportional to the length of paths, $O(\sqrt{n})$. However, the main challenge here is to bound the number of such computations, naively we may want to compare any two different non-highways, which is too expensive. To bound the number of computations, we bring to our construction a certain \emph{layering} (see Section \ref{ssec:-layerDecomp}), that decomposes all non-highway paths into $O(\log n)$ layers, each layer is composed of a set of disjoint paths in different root to leaf paths. Using the special structure of the layering, we can show that each non-highway path $P'$ of layer $i$ is only interested in small number of non-highway paths of layers at least $i$. Hence, we can process the graph according to layers, and in iteration $i$ compare all non-highway paths of layer $i$ to paths of layer at least $i$ they are interested in. Note that we exploit here the asymmetry of the path algorithm, where we let the lower layer paths be responsible for the computation (a path of higher layer may be interested in many different paths of lower layers, hence letting it do the computations would be too expensive). \yuval{A reviewer wanted more elaboration on how the relevant information is routed to the path performing the computation. I guess we can discuss what to write exactly. } Another important property of the layering is that all paths of the same layer are in completely different root to leaf paths, and the subtrees below them are disjoint, this allows us to process all paths of the same layer \emph{simultaneously}. As the paths have length $O(\sqrt{n})$, and we have $O(\log n)$ iterations, this results in a complexity of $\tilde{O}(\sqrt{n})$.


\paragraph{Exactly one edge in a non-highway.} To explain this case, we first focus on the special case that we have one non-highway $P'$, that we want to compare to a long path composed of many highways $P_H$ (see Figure \ref{partitioning_overview_pic}), later we explain how to do many such computations in parallel. The main challenge here compared to the previous case is the length of $P_H$. While comparing $P'$ to one short highway $P \in P_H$ contained in a specific fragment can be done efficiently, $P_H$ may be composed of $\Omega(\sqrt{n})$ different highways, which requires linear time for comparing $P'$ to all highways in $P_H$. A natural approach would be to let the different highways of $P_H$ do the computation instead of $P'$. For this approach, however, we need $P'$ to send some information to each one of the highways $P \in P_H$, the information sent is different for each one of the highways, and if we want to compare all edges of $P'$ to all highways $P \in P_H$, the total amount of information is linear which is too expensive. To overcome it, we exploit a certain monotone structure of the min 2-respecting cuts, described in \cite{mukhopadhyay2019weighted}, to partition the edges of $P'$ into almost disjoint sets $E'_1,...,E'_k$ such that each one of these sets should be only compared to one of the highways $P_1,...,P_k$ of $P_H$ (See Figure \ref{partitioning_overview_pic} and Section \ref{sec:mon_part}). We show that we can compute such partitioning efficiently. As now each edge of $P'$ should only be compared to small number of highways in $P_H$, now we can afford to send the relevant information from $P'$ to each one of the highways in $P_H$. \yuval{Again reviewer wanted more explanation about the how the relevant information is sent. Along the lines of if there is no appropriate edge on which to send information in the sub-tree, then we have nice structure that allows us to take care  of $E_i$ and $P_i$ with bery little communication. } We send to $P_i$ only information about edges in $E'_i$. Then we let the different highways in $P_H$ compute the min 2-respecting cuts having one edge in $E'_i$ and one edge in $P_i$, taking the minimum of those gives the minimum 2-respecting cut.

\setlength{\intextsep}{2pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.5]{partitioning.pdf}
 \caption{Illustration of the non-highway-highway case}
\label{partitioning_overview_pic}
\end{figure}

For now, we only described how to compare one non-highway to one long path composed of highways. To be able to do many such computations in parallel we need to show that each path only participates in small number of computations. For this, we use the special structure of non-highways and highways to show that each non-highway is only interested in small number of long paths composed of highways, and to show that each specific highway contained in some fragment, is only interested in small number of non-highways in different fragments (the case they are in the same fragment can be handled easily). In the algorithm described above, a highway $P$ in some fragment only participates if it is indeed interested in the non-highway $P'$ that sent it the information, which is enough, as to find the min 2-respecting cut, it is enough to focus on pairs of paths that are interested in each other. Overall, we get a complexity of $\tilde{O}(D+\sqrt{n})$ for this part. 

\paragraph{Both edges in highways.} The most challenging case is that both edges are contained in highways. To illustrate this case, we first focus on a setting where we have two long paths $P_{H_1},P_{H_2}$ composed of highways that we want to compare to each other. Again, while comparing one short highway in $P_{H_1}$ to one short highway in $P_{H_2}$ is efficient, comparing all possible pairs is clearly too expensive. Here again we would like to use monotonicity to partition the paths and break the problem to small sub-problems we can solve in parallel. The issue is that even if we just want to compute such partitioning, it seems that we need to compare at least a constant number of edges in each short highway to the highways in the second path. To be able to do so, we need to broadcast a constant amount of information for each one of the possible pairs. As we may have $\Omega(\sqrt{n})$ different highways in each one of the paths, this results in broadcasting linear amount of information. We remark that if we just want to get a sub-linear complexity, we can play with the number of fragments and their diameter (say, have $O(n^{1/3})$ fragments of diameter $O(n^{2/3})$), and get a complexity of $O(D+n^{2/3})$ rounds for this part, however, it is not clear how to compute such partitioning in the optimal $O(D+\sqrt{n})$ complexity. 

To overcome it, we design a two stage algorithm. First, we show that if we want to compare a short highway contained in a fragment to a long path of highways, we can do it efficiently, this uses monotonicity and extends ideas from the non-highway-highway case. Next, we use it as a black-box to get an algorithm comparing two long highways. The idea is as follows. Let $P_{H_1}$ and $P_{H_2}$ be two long highways we want to compare. First, we take the middle fragment $P$ in the long path $P_{H_1}$, and compare it to the path $P_{H_2}$ using the black-box algorithm. Note that since we only compare one fragment $P \in P_{H_1}$ to the different fragments in $P_{H_2}$, and not all the pairs of fragments in $P_{H_1}$ and $P_{H_2}$, the number of pairs we compare is linear in the number of fragments, $O(\sqrt{n})$, and not quadratic, which allows obtaining an efficient algorithm. After the computation, we know about the fragment $P' \in P_{H_2}$ such that the min 2-respecting cut of $P$ and $P_{H_2}$ has an edge in $P'$. We next compare $P'$ to $P_{H_1}$ using the black-box algorithm. After these computations, we either already found the min 2-respecting cut of $P_{H_1}$ and $P_{H_2}$ (in the case it has an edge in $P$ or $P'$), or we can use monotonicity to break the remaining problem into two disjoint problems that we can solve in parallel (see Figure \ref{fig:two-highway_overview}). We continue in the same manner, until we remain with disjoint problems where one of the sides has only one fragment, they can then be solved directly using the black-box algorithm. Overall we have $O(\log n)$ iterations, each one takes $\tilde{O}(D+\sqrt{n})$ time using the black-box algorithm, as we work on different disjoint problems in parallel. This completes the description of comparing two long highway paths $P_{H_1}$ and $P_{H_2}$. We next explain how to do many such computations in parallel.

\begin{figure}[h!]
    \centering
    \includegraphics[scale =0.6]{two-highway_intro.pdf}
    \caption{Illustration of the highway-highway case. After one iteration, we are left with the disjoint red and blue problems we can solve in parallel.}
    \label{fig:two-highway_overview}
\end{figure}

To find the min 2-respecting cut that has two edges in highways, we show that we can divide all the highways in the graph into pairs of long highways $(P_{H_1},P_{H_2})$, such that any specific highway $P$ contained in a single fragment is only \emph{active} in small number of computations. We use the term active, for a path $P \in P_{H_1}$ that is interested in $P_{H_2}$ (or vice verse), it may be the case that a path $P$ is included in many different pairs, but it is only active in small number of them. As we only want to find the min 2-respecting cut it would be enough to focus on active highways in each pair. To do so, we adapt our algorithm for comparing two long highways to a scenario that each one of the highways also has some set of active fragments (which can be much smaller than the total number of highways in the path), and we show that if we only want to find the min 2-respecting cut that has edges in active fragments, we can work in a way that we either work inside active fragments or broadcast information related only to the active fragments. As each specific fragment is active in small number of computations, the total amount of information to broadcast would be $\tilde{O}(\sqrt{n})$. Based on these ingredients, we get our final $\tilde{O}(D+\sqrt{n})$ algorithm.


\paragraph{Organization.}
The paper is organized as follows. First, in Section \ref{sec:prelim}, we give some useful notation and claims.
In Section \ref{sec:building_blocks}, we discuss the fragment and layering decompositions. In Section \ref{sec:lemma_and_samp}, we explain how we compute and bound the number of paths each path is interested in. In Section \ref{sec:alg_short_path}, we show how to compare two short paths. In Section \ref{sec:mon_part}, we show how to use monotonicity to partition our problem to small sub-problems. Finally, in Section \ref{sec:2_respecting}, we combine all the ingredients to obtain our algorithm for finding the min 2-respecting cut. A schematic description of the algorithm appears in Section \ref{sec:schematic_description}.

==> 5.2-NewSection.tex <==
The main lemma and goal of this section is to find for each tree edge $e$ the set $\int(e)$. 
Our starting point is the fragment decomposition defined in Section \ref{ssec:-decompFragment}, and we divide this task to two main cases:
\begin{enumerate}
    \item Finding $\int(e)$ for non-highway edges $e$.
    \item Finding $\int(e)$ for highway edges $e$.
\end{enumerate}

We start by giving a high level overview of our approach.
For the first case, given some non-highway edge $e$ in some fragment $F$, our approach is to compute $\cov(e,e')$ (henceforth called \emph{to compare} $e$ to $e'$) for all edges $e'$ which are the first highway edges in each fragment. $e$ knows these edges since $e$ knows the topology of the skeleton tree (see Claim \ref{claim:time-fragment}) and there are $O(\sqrt{n})$ such edges by the fact that $\nfrag=O(\sqrt{n})$.
The comparison itself is performed with an aggregate computation in $T(\dw{e})$ (See Section \ref{sec:preliminaries_paths}).

Using this information, $e$ can identify the fragment $F'$ that $e$ is interested in the first highway edge $e'$ of $F'$, but not in any of the descendants of $F'$ in the skeleton tree. $F'$ now represents to $e$ the path that $e$ is interested in, starting from $\lca{e,e'}$ and ending at some edge in $F'$ ($e$ is later compared to all edges of $F$, so the specific end edge doesn't matter).

If it is the case that $e$ is not interested in any first edge of any fragment, this means that $e$ is possibly interested in a path contained entirely in $F$. This case is east, since we actually compute $\cut(e,e')$  for all pairs of edges $e,e'$ which are in the same fragment (See Section \ref{sec:non_highway_simple}).

The above procedure is for a specific non-highway edge $e$, however we can not afford sequentially going over all non-highway edges and do this computation.

An important observation though is that for each fragment $F$, the comparison of all non-highway edges $e'$ not in $F$ to $F$ can be done in parallel using a single aggregate computation. We further elaborate on this later in the section.

For the second case, i.e., finding $int(e)$ for a high-way edge $e$, we employ an idea that appeared in \yuval{Cite the new simplified paper}. by performing a binary search 





==> 5.9-trees.tex <==
\section{Basic subroutines on a tree} \label{sec:preliminaries_paths}

During our algorithm many times we run basic computations in trees, mostly in the trees $T(P)$ of non-highways, on the trees $F_P$ defined by fragments, and on a BFS tree of the graph. We next discuss such computations and explain how to run many such computations in a pipelined manner.

\paragraph{Broadcast.} In a broadcast computation, the root of the fragment has a message of size $O(\log n)$ to pass to the whole tree. 
This requires time proportional to the diameter of the tree, as the root starts by sending the message to its children, that in the next round pass it to their children, and so on. Note that the computation requires sending only one message on each one of the edges of the tree.

\remove{
\begin{claim}
Let $T'$ be a tree of diameter $O(D_{T'})$, and let $z$ be a message of size $O(\log n)$ initially known to the root. In $O(D_{T'})$ rounds, all vertices in $T'$ learn $z$. Moreover, the computation uses only edges of $T'$.
\end{claim}
}

\paragraph{Aggregate computation in a tree.} 

\mtodo{I discuss here aggregate computations, should see if we need it earlier, currently some variant appears earlier in the file.}

In an aggregate computation in a tree $T'$ (sometimes called convergecast), we have an associative and commutative function $f$ with inputs and output of size $O(\log n)$ (for example, $f$ can be sum or minimum).
Each vertex $v \in T'$ initially has some value $x_v$ of $O(\log n)$ bits, and the goal of each vertex is to learn the output of $f$ on the inputs $\set{x_v}_{v\in T'_{v}}$, where $T'_{v}$ is the subtree rooted at $v$. 

Computing an aggregate function is done easily, as follows. We start in the leaves, each one of them $v$ sends to its parent its value $x_v$, each internal vertex applies $f$ on its input and the inputs it receives from its children, and passes the result to its parent. The time complexity is proportional to the diameter of the tree. Moreover, the algorithm requires sending only one message on each one of the tree edges, which allows to pipeline such computations easily.

\begin{claim} \label{claim_pipeline}
Let $T'$ be a tree of diameter $D_{T'}$, and assume we want to compute $c_1$ broadcast computations and $c_2$ aggregate computations in $T'$. Then, we can do all computations in $O(D_{T'} + c_1 + c_2)$ time. Moreover, we can work in parallel in trees that are edge-disjoint.
\end{claim}

\begin{proof}
As explained above, each broadcast or aggregate computation requires $O(D_{T'})$ time, and the computation requires only communication on edges of the tree. To complete the proof, we explain how to pipeline the computations efficiently. By the description, each broadcast requires sending only one message from each vertex to each one of its children, when we go over the tree from the root to the leaves, hence clearly we can pipeline such computations. Similarly, an aggregate computation requires sending one message from each vertex to its parent, when we go over the tree from the leaves to the root, which can also be pipelined easily. Since the two types of computations send messages in opposite directions, they do not interfere with one another, and we can run broadcast and aggregate computations in the same time, which results in a complexity of $O(D_{T'} + c_1 + c_2)$ time.
\end{proof}

\paragraph{Tree computations in a fragment $F_P$.}

When we work on fragments $F_P$ during the algorithm, we use aggregate computations in two different directions. Recall that each fragment $F_P$, has a highway $P$, which is a path between the root $r_P$ and descendant $d_P$ of the fragment, and additional sub-trees attached to $P$ that are contained entirely in the fragment. We will need to do \emph{standard} aggregate computations as described above, where $r_P$ is the root, but also computation \emph{in the reverse direction}, where we think about $d_P$ as the root and orient all edges in the fragment accordingly. See Figure \ref{orientation_pic} for an illustration. 

\setlength{\intextsep}{2pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.5]{orientation.pdf}
 \caption{Possible orientations of the fragment $F_P$. On the left appears a standard orientation where $r_P$ is the root, and on the right appears an orientation where $d_P$ is the root. Note that the only edges that changed their orientation are highway edges.}
\label{orientation_pic}
\end{figure}

We next show that we can pipeline aggregate computations in both directions and broadcast computations efficiently.

\begin{claim} \label{claim_pipeline_fragment}
Let $F_P$ be a fragment with highway $P$, and assume we want to compute $c_1$ broadcast computations, $c_2$ aggregate computations, and $c_3$ aggregate computations in the reverse direction in $F_P$. Then, we can do all computations in $O(\dfrag + c_1 + c_2 + c_3)$ time. Moreover, we can work in parallel in different fragments.
\end{claim}

\begin{proof}
Pipelining of broadcast and aggregate computations is already discussed in the proof of Claim \ref{claim_pipeline}. We next explain how we pipeline also aggregate computations where $d_P$ is the root. To pipeline aggregate computations in two different directions (where $r_P$ and $d_P$ are the roots in the two computations), we work as follows. Note that orienting edges towards $d_P$ only changes the orientation of highway edges (see Figure \ref{orientation_pic} for an illustration), hence in all subtrees attached to the highway, the communication pattern in the two computations is identical, and we can just pipeline them as before. On highway edges, we send messages in opposite directions in both computations, hence they do not interfere and we can run them on the same time. To pipeline a broadcast (from $r_P$) and an aggregate computation with root $d_P$, we work as follows. On the subtrees attached to the highway, we send messages on opposite directions in these computations, hence they do not interfere. On highway edges, we send messages on the same direction, from $r_P$ towards $d_P$, since both computations send one message per edge in the same direction, we can just pipeline them, as we would pipeline two broadcast computations. This completes the proof.
\end{proof}


We next discuss additional notation and claims required.
We denote by $p(v)$ the parent of $v$.
For the algorithm, we first make sure that the highest and lowest edges in each highway are known to all vertices, which takes $O(D+\nfrag)$ time.

\begin{claim} \label{claim_high_low}
In $O(D+\nfrag)$ time all vertices can learn the highest and lowest edges in each highway.
\end{claim}

\begin{proof}
This requires collecting and sending $O(1)$ information per fragment, which can be done in $O(D+\nfrag)$ time using upcast and broadcast in a BFS tree.
\end{proof}

==> 6-tmp.tex <==
 During our algorithm, many times we consider two ancestor to a descendant sub-paths $P',P$ of length $O(\dfrag)$, and find the min 2-respecting cut that has one edge in $P'$, and one edge in $P$. In this section, we describe how to compare two such sub-paths.
We divide to cases according to whether $P'$ and $P$ are in a highway or not. In all our claims we assume that each edge $e$ knows the value $\cov(e)$, which can be obtained from Claim \ref{claim_learn_cov}.
Before explaining the algorithm, we start with some simple claims that would be useful later.

 \subsection{Preliminaries: Basic subroutines on a tree} \label{sec:preliminaries_paths}

During our algorithm many times we run basic computations in trees, mostly in the trees $T(P)$ of non-highways, on the trees $F_P$ defined by fragments, and on a BFS tree of the graph. We next discuss such computations and explain how to run many such computations in a pipelined manner.

\paragraph{Broadcast.} In a broadcast computation, the root of the fragment has a message of size $O(\log n)$ to pass to the whole tree. 
This requires time proportional to the diameter of the tree, as the root starts by sending the message to its children, that in the next round pass it to their children, and so on. Note that the computation requires sending only one message on each one of the edges of the tree.

\remove{
\begin{claim}
Let $T'$ be a tree of diameter $O(D_{T'})$, and let $z$ be a message of size $O(\log n)$ initially known to the root. In $O(D_{T'})$ rounds, all vertices in $T'$ learn $z$. Moreover, the computation uses only edges of $T'$.
\end{claim}
}

\paragraph{Aggregate computation in a tree.} 

In an aggregate computation in a tree $T'$ (sometimes called convergecast), we have an associative and commutative function $f$ with inputs and output of size $O(\log n)$ (for example, $f$ can be sum or minimum).
Each vertex $v \in T'$ initially has some value $x_v$ of $O(\log n)$ bits, and the goal of each vertex is to learn the output of $f$ on the inputs $\set{x_v}_{v\in T'_{v}}$, where $T'_{v}$ is the subtree rooted at $v$. 

Computing an aggregate function is done easily, as follows. We start in the leaves, each one of them $v$ sends to its parent its value $x_v$, each internal vertex applies $f$ on its input and the inputs it receives from its children, and passes the result to its parent. The time complexity is proportional to the diameter of the tree. Moreover, the algorithm requires sending only one message on each one of the tree edges, which allows to pipeline such computations easily.

\begin{claim} \label{claim_pipeline}
Let $T'$ be a tree of diameter $D_{T'}$, and assume we want to compute $c_1$ broadcast computations and $c_2$ aggregate computations in $T'$. Then, we can do all computations in $O(D_{T'} + c_1 + c_2)$ time. Moreover, we can work in parallel in trees that are edge-disjoint.
\end{claim}

% \begin{proof}
% As explained above, each broadcast or aggregate computation requires $O(D_{T'})$ time, and the computation requires only communication on edges of the tree. To complete the proof, we explain how to pipeline the computations efficiently. By the description, each broadcast requires sending only one message from each vertex to each one of its children, when we go over the tree from the root to the leaves, hence clearly we can pipeline such computations. Similarly, an aggregate computation requires sending one message from each vertex to its parent, when we go over the tree from the leaves to the root, which can also be pipelined easily. Since the two types of computations send messages in opposite directions, they do not interfere with one another, and we can run broadcast and aggregate computations in the same time, which results in a complexity of $O(D_{T'} + c_1 + c_2)$ time.
% \end{proof}

\paragraph{Tree computations in a fragment $F_P$.}

When we work on fragments $F_P$ during the algorithm, we use aggregate computations in two different directions. Recall that each fragment $F_P$, has a highway $P$, which is a path between the root $r_P$ and descendant $d_P$ of the fragment, and additional sub-trees attached to $P$ that are contained entirely in the fragment. We will need to do \emph{standard} aggregate computations as described above, where $r_P$ is the root, but also computation \emph{in the reverse direction}, where we think about $d_P$ as the root and orient all edges in the fragment accordingly. See Figure \ref{orientation_pic} for an illustration. 

\setlength{\intextsep}{2pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.5]{orientation.pdf}
 \caption{Possible orientations of the fragment $F_P$. On the left appears a standard orientation where $r_P$ is the root, and on the right appears an orientation where $d_P$ is the root. Note that the only edges that changed their orientation are highway edges.}
\label{orientation_pic}
\end{figure}

We next show that we can pipeline aggregate computations in both directions and broadcast computations efficiently.

\begin{claim} \label{claim_pipeline_fragment}
Let $F_P$ be a fragment with its highway denoted by $P$, and assume we want to compute $c_1$ broadcast computations, $c_2$ aggregate computations, and $c_3$ aggregate computations in the reverse direction in $F_P$. Then, we can do all computations in $O(\dfrag + c_1 + c_2 + c_3)$ time. Moreover, we can work in parallel in different fragments.
\end{claim}
\yuval{Reviewer says that both the above claims follow from the same arguments which is true. He doesn't suggest anything though, do we want to merge them?}
% \begin{proof}
% Pipelining of broadcast and aggregate computations is already discussed in the proof of Claim \ref{claim_pipeline}. We next explain how we pipeline also aggregate computations where $d_P$ is the root. To pipeline aggregate computations in two different directions (where $r_P$ and $d_P$ are the roots in the two computations), we work as follows. Note that orienting edges towards $d_P$ only changes the orientation of highway edges (see Figure \ref{orientation_pic} for an illustration), hence in all subtrees attached to the highway, the communication pattern in the two computations is identical, and we can just pipeline them as before. On highway edges, we send messages in opposite directions in both computations, hence they do not interfere and we can run them on the same time. To pipeline a broadcast (from $r_P$) and an aggregate computation with root $d_P$, we work as follows. On the subtrees attached to the highway, we send messages on opposite directions in these computations, hence they do not interfere. On highway edges, we send messages on the same direction, from $r_P$ towards $d_P$, since both computations send one message per edge in the same direction, we can just pipeline them, as we would pipeline two broadcast computations. This completes the proof.
% \end{proof}


We next discuss additional notation and claims required.
We denote by $p(v)$ the parent of $v$.
For the algorithm, we first make sure that the highest and lowest edges in each highway are known to all vertices, which takes $O(D+\nfrag)$ time.

\begin{claim} \label{claim_high_low}
In $O(D+\nfrag)$ time all vertices can learn the highest and lowest edges in each highway.
\end{claim}

% \begin{proof}
% This requires collecting and sending $O(1)$ information per fragment, which can be done in $O(D+\nfrag)$ time using upcast and broadcast in a BFS tree.
% \end{proof}

\subsection{Simple cases where $P'$ is a non-highway} \label{sec:non_highway_simple}


In this section we discuss the following cases:
\begin{enumerate}
\item $P'$ and $P$ are non-highways.
\item $P'$ is a non-highway and $P$ is the fragment highway in the fragment of $P'$.
\item The two edges defining the cut are in the same non-highway path $P'$.
\end{enumerate}

We start with the following claim that is useful for cases involving a non-highway.

\yuval{If we indeed implement the changes the reviewer suggests and make the size of each fragment $\sqrt{n}$, this case becomes trivial since all nodes of a given fragment can know the topology of the entire fragment. I had an idea I shared with Michal about how to achieve such a fragment decomposition. }

\begin{claim} \label{claim_non_highway}
Let $P'$ be a non-highway path, and let $e$ be an edge outside $T(P')$, such that $\{e,\cov(e)\}$ is known to all vertices in $T(P')$. 
Then, using one aggregate computation in $T(P')$, each edge $e' \in P'$ can compute the value $\cut(e',e).$ In addition, for different paths $P'$ that are not in the same root to leaf path, these computations can be done in parallel.
\end{claim}

% \begin{proof}
% Let $e' \in P'$. By Claim \ref{claim_cover}, $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e)$. Also, $e'$ knows $\cov(e)$ and $\cov(e')$, hence to compute $\cut(e',e)$, the edge $e'$ should compute $\cov(e',e).$ As any edge that covers a tree edge $e'=\{v',p(v')\}$ where $p(v')$ is the parent of $v'$, has one endpoint in the subtree of $v'$ by Claim \ref{claim_subtree}, it follows that the edges that cover $e'$ and $e$ are exactly all the edges that cover $e$ and have exactly one endpoint in the subtree of $v'$. This subtree is contained in $T(P')$. Note that any edge $x$ that covers $e'$ and $e$ cannot have both endpoints in $T(P')$, as otherwise the tree path covered by $x$ is contained entirely in $T(P')$, but as $e$ is outside $T(P')$, $x$ cannot cover $e$ in this case, which leads to a contradiction.
% Hence, to learn about the total cost of the edges that cover $e$ and $e'$ we need to do one aggregate computation in $T(P')$: letting each vertex $v' \in T(P'^{\downarrow})$ learn about the total cost of edges incident on the subtree of $v'$ that cover $e$. This can be done using a convergecast in $T(P')$, where each vertex sends to its parent the total cost of edges in its subtree that cover $e$, this includes the sum of costs of edges it receives from its children and the cost of such edges adjacent to it. To implement this efficiently we need an efficient way to determine for each non-tree edge whether it covers a specific edge $e$, this can be done using Claim \ref{claim_LCA_labels}. Hence, all the edges $e' \in P'$ can compute $\cut(e',e)$ using one aggregate computation in the subtree of $P'$.
% Since the whole computation was done in $T(P')$, the same computation can be done in parallel for other paths not in the same root to leaf path with $P'$.
% \end{proof}

Claim \ref{claim_non_highway} immediately solves the case that $P'$ is a non-highway and $P$ is either a non-highway above $P'$ in the same fragment, or the highway of the fragment of $P$, as we show next.

\begin{claim} \label{claim_non_highway_fragment}
Let $P'$ be a non-highway in the fragment $F_{P'}$ and assume that all vertices in $T(P')$ know the complete structure of $P'$. In $O(\dfrag)$ time, all edges $e' \in P'$, can compute the values $\cut(e',e)$ for all edges $e \in F_{P'}$ that are either above $P'$ in the same fragment, or in the highway of $F_{P'}$. The computation can be done in parallel for different paths $P'$ not in the same root to leaf path.
\end{claim}

% \begin{proof}
% First, using Claim \ref{claim:-fragDecompRouting_inside}, in $O(\dfrag)$ time, all edges $e'$ in the fragment of $P'$ can learn the values $\{e,\cov(e)\}$ for all edges $e$ on the paths between $e'$ to the root $r_{P'}$ and descendant $d_{P'}$ of the fragment $F_{P'}$. This can be done for all edges and all fragments simultaneously. If we focus our attention to edges $e' \in P'$, the paths it learned about contain some non-highway path above $e'$ that connects $e'$ to the highway, and all the edges of the highway $P$ of $F_{P'}$. If we exclude from these paths all edges contained in $P'$ (which can be done easily as $P'$ is known), we have that the rest of edges, denoted by $E'$, include exactly all non-highways above $P'$ in the fragment, and the highway $P$. All the edges of $E'$ are not in $T(P')$. Additionally, $|E'| = O(\dfrag)$, as it is composed of two paths inside the fragment. Hence, we can use Claim \ref{claim_non_highway}, and compute the values $\cut(e',e)$ for all $e' \in P', e \in E'$ using $O(\dfrag)$ aggregate computations. Using pipelining, the overall complexity is $O(\dfrag)$. As the computation was inside $T(P')$, it can be done in parallel for other paths not in the same root to leaf path.
% \end{proof}

Also, we can adapt the proof of Claim \ref{claim_non_highway} to take care of the case that both edges defining the cut are in the same non-highway $P'$.

\begin{claim}\label{clm:both-edge-nh}
Let $P'$ be a non-highway, and assume that all vertices in $T(P')$ know all the values $\{e,\cov(e)\}_{e \in P'}$. Then, in $O(\dfrag)$ time, each edge $e' \in P'$, can compute the values $\cut(e',e)$ for all edges $e$ above it in $P'$. The computation can be done in parallel for different paths $P'$ not in the same root to leaf path.
\end{claim}

% \begin{proof}
% Fix an edge $e = \{v,p(v)\} \in P'$. Let $T_v \subset T(P')$ be the subtree rooted at $v$. We run an aggregate computation in $T_v$ to let all edges $e' \in T_v$ compute the value $\cut(e',e).$ The computation is identical to the computation described in the proof of Claim \ref{claim_non_highway}, with the difference that we stop the computation in $v$, i.e., the computation is only inside $T_v$ and not in $T(P')$, as $e \not \in T_v$, we can follow the same computation. At the end of the computation, all edges $e'$ below $e$ in $P'$ know the value $\cut(e',e).$ To do so for all edges $e \in P$, we pipeline the computations which takes $O(\dfrag)$ time.
% \end{proof}

We are now left with the case that $P'$ and $P$ are orthogonal non-highways. We use Claim \ref{claim_non_highway} again to deal with this case. Note that the non-orthogonal case was already covered in Claim \ref{claim_non_highway_fragment}, as a non-highway path $P$ can be in the same root to leaf path with $P'$ only if they are in the same fragment, as the path from a non-highway path to the root is composed of a non-highway inside the fragment, and highways above it in other fragments. We will later show in our algorithm that we only compare orthogonal non-highway paths $P'$ and $P$ such that there is an edge between $T(P')$ and $T(P)$. Hence, we focus in this case.

\begin{claim} \label{claim_orthogonal_nh}
Let $P'$ be a non-highway and let $P$ be a non-highway path not in the same root to leaf path with $P'$. Assume that there is an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow})$, that is known to all vertices in $T(P')$.
Also, assume that at the beginning of the computation all vertices in $T(P)$ know all values $\{e,\cov(e)\}_{e \in P}$. Then, in $O(\dfrag)$ time, all edges $e' \in P'$ can compute the values $\{e,\cut(e',e)\}_{e \in P}.$ The computation can be done in parallel for different paths $P'$ not in the same root to leaf path.
\end{claim}

% \begin{proof}
% As all vertices in $T(P)$ know the values $\{e,\cov(e)\}_{e \in P}$, and the edge $f$ has an endpoint in $T(P)$ and an endpoint in $T(P')$, it knows this information, and can pass it to all vertices in $T(P')$ using $O(\dfrag)$ aggregate and broadcast computations in $T(P').$ Note that since the subtrees $T(P'^{\downarrow})$ are disjoint for non-highways not in the same root to leaf path, the edge $f$ is different for different such paths $P'$, which allows working in parallel as needed. As $P$ and $P'$ are not in the same root to leaf path, we have that all edges $e \in P$ are not in $T(P')$, hence we can use Claim \ref{claim_non_highway} to let all edges $e' \in P'$ learn the values $\{e,\cut(e',e)\}$, this takes $O(\dfrag)$ time using pipelining, and can be done in parallel for different non-highways $P'$ not in the same root to leaf path. 
% \end{proof}

\remove{
\begin{claim}
Let $P'$ be a non-highway and let $P$ be a non-highway path not in the same root to leaf path with $P'$. Assume that there is an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow})$ \sagnik{What does $\downarrow$ signify?}, that is known to all vertices in $T(P) \cup T(P').$
Also, assume that at the beginning of the computation all vertices in $T(P)$ know all values $\{e,\cov(e)\}_{e \in P}$. Then, in $O(\dfrag)$ time, all edges $e' \in P'$ can compute the values $\{e,\cut(e',e)\}_{e \in P}.$ The computation can be done in parallel for different paths $P'$ not in the same root to leaf path.
\end{claim}

% \begin{proof}
% As all vertices in $T(P)$ know the values $\{e,\cov(e)\}_{e \in P}$, and the edge $f$ has an endpoint in $T(P)$ and an endpoint in $T(P')$ \sagnik{Here you do not use $\downarrow$}, it knows this information, and can pass it to all vertices in $T(P')$ using $O(\dfrag)$ aggregate and broadcast computations in $T(P').$ As $P$ and $P'$ are not in the same root to leaf path, we have that all edges $e \in P$ are not in $T(P')$, hence we can use Claim \ref{claim_non_highway} to let all edges $e' \in P'$ learn the values $\{e,\cut(e',e)\}$, this takes $O(\dfrag)$ time using pipelining.
% \end{proof}
}

\subsection{$P'$ is a non-highway and $P$ is a highway}

Here we focus on the case that $P'$ is a non-highway and $P$ is the highway of a different fragment. The case that $P$ is in the same fragment was already discussed in the previous section.
Let $e' \in P', e \in P$, we next look at the value $\cov(e',e).$ See Figure \ref{non_highway_highway} for an illustration.
We need the following definitions. 
\begin{itemize}
\item $\cov_{F}(e',e)$ is the cost of all edges that cover $e'$ and $e$ and have one endpoint in $T(P'^\downarrow)$ and one endpoint in the fragment $F_P$ of $P$.
\item $\extcov(e',P)$ the cost of all edges that cover $e'$ and the whole highway $P$, and have one endpoint in $T(P')$ and both endpoints outside $F_P$.
\end{itemize}

We next show that all all the edges that cover $e'$ and $e$ are in one of the above categories.

\setlength{\intextsep}{0pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.4]{non_highway_highway.pdf}
 \caption{Examples of a non-highway $P'$ and a highway $P$. On the left, $P'$ and $P$ are orthogonal, and on the right, $P$ is above $P'$. The edges $x_1$ and $y_1$ are examples of edges counted in $\cov_F(e',e)$, and the edges $x_2$ and $y_2$ are examples of edges counted in $\extcov(e',P).$}
\label{non_highway_highway}
\end{figure}
\yuval{Reviewer had some comment here saying that we do not need to require that $P'$ is a non-highway, but I think it is helpful to keep that specific example in mind.}
\begin{claim} \label{cover_non_highway_highway_new}
Let $e' \in P', e \in P$ where $P'$ is a non-highway, and $P$ is a highway in a different fragment $F_P$. Then $\cov(e',e) = \cov_{F}(e',e) + \extcov(e',P)$.
\end{claim}

% \begin{proof}
% First note that by Claim \ref{claim_subtree}, any edge $x$ that covers $e'$ has one endpoint in the subtree $T(P'^\downarrow)$ which is inside the fragment $F_{P'}$ of $P'$. 
% Now the edges that cover $e'$ and $e$ are all the edges with one endpoint in $T(P')$ that cover $e'$ and $e$. If the second endpoint of the edge is in the fragment $F_P$, these edges are counted in $\cov_{F}(e',e)$. To complete the proof, we need to show that any edge $x$ that covers $e'$ and $e$ and has both endpoints outside $F_P$, must cover the whole highway $P$. If $x = \{u,v\}$ covers both $e'$ and $e$ with both endpoints outside $F_P$ and $u \in T(P')$, the unique $u-v$ path in the tree starts in the fragment $F_{P'}$, and then enters and leaves the fragment $F_{P}$. From the structure of the decomposition, the only two vertices in $F_P$ that are connected by an edge to vertices outside the fragment are the ancestor $r_P$ and descendant $d_P$ of the fragment, hence any path that enters and leaves $F_P$ must include $r_P$ and $d_P$ and the whole path between them, which is the highway $P$. Hence, $x$ must cover the whole highway $P$ as needed. 
% \end{proof}

We next explain how $\cov_{F}(e',e)$ and $\extcov(e',P)$ are computed.

\paragraph{Computing $\cov_{F}(e',e)$.}

\begin{claim} \label{claim_covF_nh}
Let $P'$ be a non-highway and let $P$ be a highway of the fragment $F_P$. 
Given an edge $e \in P$, using an aggregate computation in $T(P')$, all edges $e' \in P'$ can compute the value $\cov_{F}(e',e)$.
\end{claim}

% \begin{proof}
% The proof is similar to the proof of Claim \ref{claim_non_highway}. When we fix an edge $e \in P$, computing $\cov_{F}(e',e)$ for all edges $e' \in P'$ is an aggregate computation in $T(P').$ This follows as the edges counted in $\cov_{F}(e',e)$ for $e' = \{v',p(v')\}$ are all the edges with one endpoint in the subtree of $v'$ (which is contained in $T(P')$) and one endpoint in $F_P$ that cover $e'$ and $e$. To compute the cost of those we just run an aggregate computation in $T(P')$. Note that for each edge $x$ with an endpoint $v$ in $T(P')$, $v$ knows if the second endpoint is in $F_P$, and also can deduce from the LCA labels using Claim \ref{claim_LCA_labels} whether $x$ covers $e$ and $e'$, which allows computing the aggregate function. At the end of the computation, each vertex $v' \in T(P')$ knows exactly the cost of edges in its subtree that cover $e'$ and $e$ with the second endpoint in $F_P$, which is exactly $\cov_{F}(e',e)$ for $e' = \{v',p(v')\}.$ 
% \end{proof}

\begin{claim} \label{claim_covF_h}
Let $P'$ be a non-highway and let $P$ be the fragment highway of the fragment $F_P$. 
Given an edge $e' \in P'$, using an aggregate computation in $F_P$, all edges $e \in P$ can compute the value $\cov_{F}(e',e)$.
\end{claim}

% \begin{proof}
% Here we break into cases according to the connection between $P'$ and $P$.
% One case is that they are orthogonal, and one case is that $P$ is a highway above $P'$.
% Note that from the structure of the decomposition, there are no other cases, as any path in the tree between a descendant and an ancestor starts with a non-highway and highways above it, so we cannot have $P'$ above $P$. Note also that all vertices know the complete structure of the skeleton tree, and can deduce accordingly in which one of the two cases we are.

% \emph{Case 1: $P'$ and $P$ are orthogonal.} Here we know that $T(P')$ and $T(P)$ are disjoint, hence from Claim \ref{claim_subtree} it follows that all edges that cover $e' \in P$ and $e \in P$ have one endpoint in $T(P')$ and one endpoint in $T(P).$ Note that $T(P)$ is not necessarily contained in $F_P$, but since we are interested only in computing $\cov_{F}(e',e)$, we are only interested in edges with one endpoint in $T(P')$ and one endpoint in $T(P) \cap F_P$ that cover $e'$ and $e$. Computing the total cost of these edges requires one aggregate computation in $T(P) \cap F_P$, and follows exactly the computation described in the proof of Claim \ref{claim_covF_nh}.

% \emph{Case 2: $P$ is above $P'$.} Here we need to do an aggregate computation in the reverse direction, to explain this we first take a closer look on edges that cover $e'$ and $e$ in this case. Since $e'$ is below $e$ in the tree, any tree path that contains both of them must include the whole tree path between them, which in particular includes a part between the descendent $d_P$ of the fragment $F_P$ to $e \in P.$ Hence, we need to sum the cost of edges that cover $e'$ and $e$ and also the whole path between $e$ and $d_P$. To compute it, it would be helpful to reverse the orientation in the fragment $F_P$, such that now $d_P$ is the \emph{root} of the fragment. Now if $e = \{v,d(v)\}$ where $d(v)$ is the vertex closer to $d_P$, all edges that cover $e'$ and the path between $e$ and $d_P$ and have an endpoint in $F_P$, must have an endpoint in the subtree of $v$ according to the new orientation (the subtree that includes everything below $v$ when we think about $d_P$ as the root). Hence, to compute the total cost of edges that cover $e'$ and $e$ and have one endpoint in $F_P$, we just do one aggregate computation in $F_P$ in the reverse direction to sum the costs of these edges. At the end of the computation, the vertex $v$ such that $e = \{v,d(v)\}$ knows exactly $\cov_F(e',e).$ Similarly, for each edge $e \in P$, one of its endpoints knows $\cov_F(e',e)$ as needed.
% \end{proof}

\paragraph{Computing $\extcov(e',P)$.}
\yuval{Reviewer says we do need to mention layering at all, this lemma is used very frequently so I am not touching anything now.}
\begin{claim} \label{claim_cov_eP_nh}
In $O(\dfrag + \nfrag)$ time, all edges $e'$ in the non-highway $P'$ can compute the values $\extcov(e',P)$ for all highways $P$. Moreover, this computation can be done in all non-highways in the same layer simultaneously.
\end{claim}

% \begin{proof}
% Let $e' = \{v',p(v')\} \in P'$, and fix a highway $P$. The edges that cover $e'$ have one endpoint in $T(P') \subseteq F_{P'}$ by Claim \ref{claim_subtree}. Hence, to compute the total cost of edges that cover $e'$ and the whole highway $P$ we just need to do one aggregate computation in $T(P').$ To implement the computation, we need to explain how given an edge $x$ we know if it covers the whole highway $P$ and if both its endpoints are outside $F_P.$ The second is immediate. For the first, note that $x$ covers the whole highway $P$ iff it covers the highest and lowest edges in the highway, since in this case it must cover the whole path between them which is the highway. As the highest and lowest edges in the highway are known to all vertices by Claim \ref{claim_high_low}, and since we can use LCA labels of edges to learn if $x$ covers some edge by Claim \ref{claim_LCA_labels}, we can compute the aggregate function. At the end of the computation, each vertex $v' \in P'$ knows the total cost of edges in its subtree that cover the whole highway $P$ and have both endpoints outside $F_P$, this is exactly $\extcov(e',P)$ for the edge $\{v',p(v')\}.$
% This requires one aggregate computation. To compute the values $\extcov(e',P)$ for all highways we run $O(\nfrag)$ such computations, which results in $O(\dfrag + \nfrag)$ time as we pipeline the computations. As the whole computation was inside $T(P')$, we can run in parallel in disjoint subtrees, and in particular we can run the computations in parallel for all non-highways $P'$ in the same layer.
% \end{proof}


\paragraph{An algorithm for two paths.}

We next explain how given a non-highway $P_0$ and a highway $P_1$ we compute the values $\{\cut(e',e)\}_{e' \in P_0, e \in P_1}.$ We start by discussing the case that there is an edge between $T(P_0)$ and $F_{P_1}.$

\begin{lemma} \label{lemma_paths_nh_h}
Let $P_0$ be a non-highway in the fragment $F_{P_0}$ and let $P_1$ be the fragment highway of a different fragment $F_{P_1}$, and assume that there is an edge $f$ between $T(P_0^\downarrow)$ and $F_{P_1}$. 
Let $E_0 \subseteq P_0$ be a set of edges in $P_0$ we compare to $P_1$, and $E_1 \subseteq P_1$ be a set of edges in $P_1$ that we compare to $P_0$.
Additionally, assume that at the beginning of the computation the following information is known:
\begin{itemize}
\item All vertices in $T(P_0)$ know the identity of the edge $f$, The identity of all the edges in $E_0$, and for each edge $e' \in E_0$, the values $\cov(e'),\extcov(e',P_1)$.
\item All vertices in $F_{P_1}$ know the identity of the edge $f$, the identity of all the edges in $E_1$, and for each edge $e \in P_1$, the value $\cov(e)$.
\end{itemize}

We can compute the values $\{\cut(e',e)\}_{e' \in P_0, e \in P_1}$ in the following two ways.
\begin{enumerate}
\item In $O(|E_1|)$ aggregate and broadcast computations in $T(P_0)$, where at the end of the computation each edge $e' \in E_0$ would know the values $\cut(e',e)$ for all edges $e \in E_1$. \label{P0_compute}
\item In $O(|E_0|)$ aggregate and broadcast computations in $F_{P_1}$, where at the end of the computation each edge $e \in E_1$ would know the values $\cut(e',e)$ for all edges $e' \in E_0$. \label{P1_compute}
\end{enumerate}
\end{lemma}

% \begin{proof}
% We start by proving Case \ref{P0_compute} where the computations are done in $T(P_0)$.
% First, we use the edge $f$ that has an endpoint in $T(P_0)$ and an endpoint in $F_{P_1}$ to pass information from $F_{P_1}$ to $T(P_0)$.
% As $f$ has an endpoint in $F_{P_1}$ it knows the values $\{e,\cov(e)\}_{e \in E_1}$ and can pass them to all vertices in $T(P_0)$ using $O(|E_1|)$ aggregate and broadcast computations in $T(P_0)$. Let $e' \in E_0, e \in E_1.$
% From Claims \ref{claim_cover} and \ref{cover_non_highway_highway_new}, we have $$\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e,e'),$$ $$\cov(e',e) = \cov_{F}(e',e) + \extcov(e',P_1).$$ An edge $e' \in E_0$ already knows $\cov(e')$ and $\extcov(e',P_1),$ and from the broadcast it also knows the value $\cov(e)$ for all edges $e \in E_1.$ Hence, to compute the value $\cut(e',e)$ for a specific edge $e \in E_1$, it only needs to compute $\cov_{F}(e',e)$. By Claim \ref{claim_covF_nh}, all edges $e' \in P_0$ can compute the value $\cut(e',e)$ for a fixed $e$ using one aggregate computation in $T(P_0).$ To compute this value for all edges $e \in E_1$, we pipeline $|E_1|$ such aggregate computations, which concludes the proof of Case \ref{P0_compute}.   

% We next discuss Case \ref{P1_compute}, where the computations are done in $F_{P_1}.$
% Here we use $f$ to pass the information $\{e',\cov(e'),\extcov(e',P_1)\}_{e' \in E_0}$ from $T(P_0)$ to $F_{P_1}$, which requires $O(|E_0|)$ broadcast and aggregate computation in $F_{P_1}$. Now, after this each edge $e \in E_1$ knows the value $\cov(e)$ as well as the values $\{e',\cov(e'),\extcov(e',P_1)\}_{e' \in E_0}$. As discussed in the proof of Case \ref{P0_compute}, the only information missing to compute $\cut(e',e)$ is $\cov_{F}(e',e)$. Given an edge $e' \in E_0$, all edges $e \in P_1$ can compute $\cut(e',e)$ using one aggregate computation in $F_{P_1}$ by Claim \ref{claim_covF_h}. To do so for all edges $e' \in E_0$, we pipeline $|E_0|$ such aggregate computations, which completes the proof.
% \end{proof}

We next discuss the case that there are no edges between $T(P_0)$ and $F_{P_1}.$
Let $P$ be a highway, we denote by $e^P_{min}$ the edge $e \in P$ such that $\cov(e)$ is minimal. First, we make sure that the values $\cov(e^P_{min})$ are known to all vertices.

\begin{claim} \label{claim_cov_min}
In $O(D+\nfrag + \dfrag)$ time all vertices learn the values $\{e^P_{min}, \cov(e^P_{min})\}$ for all highways $P$.
\end{claim}  

% \begin{proof}
% First, in each highway, finding the edge $e^P_{min}$ requires an aggregate computation inside the fragment, which takes $O(\dfrag)$ time.
% Next we send this information to all vertices.
% As there is only one edge $e^P_{min}$ per highway, and there are $\nfrag$ highways, this only requires collecting and broadcasting $\nfrag$ information in a BFS tree, which takes $O(D+\nfrag)$ time.
% \end{proof}

\begin{lemma} \label{lemma_nh_no_edge}
Let $P_0$ be a non-highway, and $P_1$ be a highway in a different fragment, such that there are no edges between $T(P_0^\downarrow)$ and $F_{P_1}$. Then if each edge $e' \in P_0$ knows the values $\cov(e'),\extcov(e',P_1)$, as well as the values $\{e^{P_1}_{min}, \cov(e^{P_1}_{min})\}$, using one aggregate and broadcast computations in $P_0$, all vertices in $P_0$ learn about the values $\{e',e,\cut(e',e)\}$ for edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal.
\end{lemma}

% \begin{proof}
% Let $e' \in P_0, e \in P_1$.
% Again, from Claims \ref{claim_cover} and \ref{cover_non_highway_highway_new}, we have $$\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e,e'),$$ $$\cov(e',e) = \cov_{F}(e',e) + \extcov(e',P_1).$$
% Now if there are no edges between $T(P_0^\downarrow)$ and $F_{P_1}$, from the definition $\cov_{F}(e',e) = 0$ for any pair of edges $e' \in P_0, e \in P_1$, as this is the sum of costs of edges with one endpoint in $T(P_0^\downarrow)$ and the second in $F_{P_1}$.
% Hence, in this case, we have $$\cut(e,e') = \cov(e) + \cov(e') - 2\extcov(e',P_1).$$ Note that the expression $\cov(e') - 2\extcov(e',P_1)$ does not depend on the specific choice of $e \in P_1$, hence to minimize the expression $\cut(e',e)$ for a specific $e' \in P_0$, we just need to find an edge $e \in P_1$ where $\cov(e)$ is minimal, this is the edge $e^{P_1}_{min}$. As each edge $e' \in P_0$ knows the values $e^{P_1}_{min},\cov(e^{P_1}_{min}), \cov(e'),\extcov(e',P_1)$ it can compute $\cut(e',e)$ for an edge $e \in P_1$ such that $\cut(e',e)$ is minimal. To find the minimum over all choices of $e'$ we just need one aggregate computation in $P_0$ to find the minimum value computed, we can then broadcast the information to let all vertices in $P_0$ learn the values $\{e',e,\cut(e',e)\}$ for edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal.
% \end{proof}

\subsection{$P'$ and $P$ are highways}

Let $e' \in P', e \in P$ be two tree edges in the highways $P',P$ such that $F_{P'},F_P$ are the fragments of $P'$ and $P$, respectively. The value $\cov(e',e)$ is broken up to the following different parts. See Figure \ref{highway_highway} for an illustration.

\begin{enumerate}
\item The cost of edges that cover entirely the highways $P$ and $P'$, with endpoints outside $F_{P'} \cup F_P$: $\extcov(P',P).$ 
\item The cost of edges with one endpoint in $F_{P'}$ and one endpoint outside $F_{P'} \cup F_P$ that cover $e'$ and the whole highway $P$: $\extcov(e',P).$
\item The cost of edges with one endpoint in $F_{P}$ and one endpoint outside $F_{P'} \cup F_P$ that cover $e$ and the whole highway $P'$: $\extcov(e,P').$
\item The cost of edges that cover $e',e$ and have endpoints in both $F_P$ and $F_{P'}$: $\cov_{F}(e',e)$.
\end{enumerate}

To see that these are all the options we use the structure of the decomposition. 

\setlength{\intextsep}{0pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.4]{highway_highway.pdf}
 \caption{\small Example of two highways $P'$ and $P$, for the special case that the tree is a path, and $P$ and $P'$ are subpaths of it. The edges $x_1,x_2,x_3,x_4$ are counted in $\extcov(P',P),\extcov(e',P),\extcov(e,P'),\cov_F(e',e)$, respectively.}
\label{highway_highway}
\end{figure}

\begin{claim} \label{claim_cov_highways}
Let $e' \in P', e \in P$ be two tree edges in the highways $P',P$. Then, $$\cov(e',e) = \extcov(P',P) + \extcov(e',P) + \extcov(e,P') + \cov_{F}(e',e).\footnote{This is a slight abuse of notation of $\cov(\cdot)$ but is clear from the context.}$$
\end{claim}

% \begin{proof}
% First, if $x = \{u,v\}$ is an edge that covers $e \in P$, then the unique tree path between $u$ and $v$ contains $e$. As the the only vertices in $F_{P}$ that are connected by an edge to a vertex outside $F_{P}$ are the root $r_P$ and unique descendant $d_P$ of the fragment, any path in the tree that contains $e$ and have both endpoints outside the fragment, must also contain the whole highway between $r_P$ and $d_P$ (as otherwise, at least one of the endpoints would be inside the fragment). Hence, if both endpoints of $x$ are outside $F_P$, it covers the whole highway $P$. 

% Now any edge $x$ that covers $e'$ and $e$, has the following options.
% \begin{enumerate}
% \item $x$ has both endpoints outside $F_{P'}$ and $F_P$, in this case it follows that $x$ must cover the whole highways $P'$ and $P$, which is exactly counted by $\extcov(P',P).$
% \item $x$ has one endpoint in $F_{P'}$ but two endpoints outside $F_P$, in this case $x$ must cover the whole highway $P$, which is exactly counted in $\extcov(e', P).$
% \item $x$ has one endpoint in $F_{P}$ but two endpoints outside $F_{P'}$, in this case $x$ must cover the whole highway $P'$, which is exactly counted in $\extcov(e, P').$
% \item $x$ has two endpoints in $F_{P'} \cup F_{P}$, in this case it must be the case that $x$ has one endpoint in $F_{P'}$ and one endpoint in $F_{P}$, as otherwise the unique tree path defined by $x$ is contained entirely in one of the fragments and cannot cover both edges $e' \in P', e \in P$. This is counted by $\cov_{F}(e',e)$.
% \end{enumerate} 
% \end{proof}

We next explain how we compute the different ingredients in the expression $\cov(e,e').$

\paragraph{Computing $\extcov(P,P')$.}

\begin{claim}\label{clm:two-short-highway}
Let $P,P'$ be two highways. Using one aggregate and one broadcast computation in a BFS tree, all vertices can learn $\extcov(P,P')$. Computing this value for $k$ different pairs takes $O(D+k)$ time.
\end{claim}

% \begin{proof}
% Given some edge $x = \{u,v\}$, it knows if its endpoints are outside $F_P \cup F_{P'}$. In addition, it can learn if it covers the highway $P$ as follows. An edge $x$ covers the whole highway $P$ iff it covers both the highest and lowest edges in $P$: $e_1, e_2$, because in this case it follows that the unique tree path between $u$ and $v$ contains the unique tree path between $e_1$ and $e_2$ which is the highway $P$. Using the LCA labels of edges and Claim \ref{claim_LCA_labels}, $x$ can learn if it covers $e_1,e_2$. Similarly, $x$ can learn if it covers the whole highway $P'$, and then deduce if it covers both $P$ and $P'$. Now to compute $\extcov(P,P')$ we sum the cost of all edges that cover both $P$ and $P'$ and have both endpoints outside $F_P \cup F_{P'}$, this is a sum of values that can be computed using an aggregate computation in a BFS tree. For each edge $x$ outside $F_P \cup F_{P'}$ that covers both $P$ and $P'$, one of its endpoints represents $x$ in the computation, and adds its cost to the sum computed. To let all vertices learn the value $\extcov(P,P')$ we use a broadcast in the BFS tree. If we have $k$ different pairs, we pipeline the computations to get a complexity of $O(D+k)$.    
% \end{proof}

\paragraph{Computing $\cov_F(e',e)$.}

\begin{claim} \label{claim_covl}
Let $P,P'$ be highways of the fragments $F_P$ and $F_{P'}$, respectively, and let $e \in P$.
Using one aggregate computation in $F_{P'}$, all edges $e' \in P'$ can compute the value $\cov_{F}(e',e)$.
\end{claim}


% \begin{proof}
% If we look at the highways $P$ and $P'$, there are several cases:
% \begin{enumerate}
% \item $P$ and $P'$ are orthogonal. \label{case_or}
% \item $P$ and $P'$ are in the same root to leaf path with $P'$ below $P$. \label{case_below}
% \item $P$ and $P'$ are in the same root to leaf path with $P$ below $P'$. \label{case_above}
% \end{enumerate}
% Note that all vertices know the complete structure of the skeleton tree, hence they can distinguish between the cases.
% We start with the first two cases.

% \emph{Cases \ref{case_or} and \ref{case_below}}. In these cases, we show that any edge $x$ that covers $e \in P$ and some edge $e' = \{v',p(v')\} \in P'$ and has endpoint in $F_{P'}$ has an endpoint in the subtree of $v'$ in $F_{P'}$. 
% This is justified as follows. We know that any edge $x$ that covers $e'$ has an endpoint $u$ in the subtree rooted at $v'$ by Claim \ref{claim_subtree}. Assume to the contrary that $u \not \in F_{P'}$, but rather the second endpoint of $x$, $u'$, is in $F_{P'}$. Now the path between $u$ and $u'$ has a part in $F_{P'}$, and a part below it, as $u$ is in the subtree rooted at $v' \in P'$. This path can only cover edges in $F_{P'}$ or below it, but we are in the case that $P$ is orthogonal to $P'$ or above it, hence it does not have any edge in $F_{P'}$ or below it, which means that $x$ cannot cover $e \in P$, a contradiction.

% Hence, we know that any edge that covers $e \in P$ and $e' \in P'$ and also has an endpoint in $F_{P'}$ has an endpoint in $T(P') \cap F_{P'}$.
% Hence, given an edge $e \in P$, computing the values $\cov_{F}(e',e)$ for all edges $e' \in P'$ requires one aggregate computation in $F_{P'}$, in which every vertex $v' \in F_{P'}$ learns the total cost of edges adjacent to its subtree in $F_{P'}$ that cover also $e$, and have the second endpoint in $F_P$. As explained in the proof of Claim \ref{claim_non_highway} this is an aggregate computation in the subtree, and it can be computed as for each non-tree edge $x$ we can deduce it it covers $e$ using its LCA labels (see Claim \ref{claim_LCA_labels}). At the end of the computation, the vertex $v'$ such that $e' = \{v',p(v')\}$ knows exactly the value $\cov_{F} (e',e).$

% \emph{Case \ref{case_above}.} In this case $P$ and $P'$ are in the same root to leaf path with $P$ below $P'$. 
% Let $e' \in P', e \in P$, we start by analysing the structure of edges that cover $e'$ and $e$ in this case. Since $P$ is below $P'$, any edge $x$ that covers $e'$ and $e$ covers the whole path between $e'$ and $e$. In particular, it covers the whole path between $e' \in P'$ to the unique descendant $d_{P'}$ of the fragment $F_{P'}$. Hence, we need to sum the costs of edges that cover $e'$ and $e$, have endpoints in $F_{P'}$ and $F_P$, and also cover the whole path between $e'$ and $d_P$.
% To compute the cost of these edges, it would be helpful to change the orientation in the fragment $F_{P'}$, such that now $d_{P'}$ is the \emph{root}. We write $e' = \{v,d(v)\}$ where $d(v)$ is the vertex closer to $d_{P'}$ (this is the reverse orientation compared to the previous cases). Now, given an edge $e \in P$, we want to compute the total cost of edges adjacent to the subtree of $v$ in $F_{P'}$ that cover $e,e'$ and have the second endpoint in $F_P$, where the subtree is with respect to the new orientation (having $d_{P'}$ as the new root). This gives exactly $\cov_{F} (e',e).$ Again, this is an aggregate computation in the fragment $F_{P'}.$

% Note that the aggregate computation in Case \ref{case_above} is in a different direction than the aggregate computations in Cases \ref{case_or} and \ref{case_below}. However, since all vertices know the structure of the skeleton tree, they all know in which case we are, and can change the orientation accordingly, which only requires changing the orientation for highway edges, as discussed in Section \ref{sec:preliminaries_paths}.
% \end{proof}

\paragraph{Computing $\extcov(e,P)$.}

\begin{claim} \label{claim_cov_eP}
In $O(\dfrag + \nfrag)$ time, all edges $e$ that are in a highway can compute the values $\extcov(e,P)$ for all highways $P$.
\end{claim}

% \begin{proof}
% First, we fix two highways $P',P$, and show how all edges $e' \in P'$ compute $\extcov(e',P).$ 
% The edges that cover $e'$ and the whole highway $P$ are exactly the edges that cover $e'$ and the highest and lowest edges in $P$: $e_1,e_2.$
% To compute $\extcov(e',P)$, which is the sum of all such edges that have one endpoint in $F_{P'}$ and one endpoint outside $F_{P'} \cup F_{P}$ we use an aggregate computation in $F_{P'}$. This aggregate computation is very similar to the computation done in the proof of Claim \ref{claim_covl}, with the difference that now instead of summing the cost of edges that cover $e'$ and a specific edge $e$, we sum the cost of edges that cover $e'$ and $e_1,e_2$, and also make sure that the second endpoint is not in $F_{P'} \cup F_{P}$, the computation can be done in the same manner. For each highway we have one aggregate computation to compute $\extcov(e',P)$ for all edges $e' \in P'.$ To do so for all highways $P$, we need $\nfrag$ such computations. Since the whole computation was done inside $F_{P'}$, we can do the same computation in all fragments simultaneously, the overall complexity is $O(\dfrag + \nfrag)$.
% \end{proof}

\paragraph{An algorithm for two paths.}

We next explain how given two highways $P_0,P_1$, we compute $\cut(e',e)$ for edges $e' \in P_0, e \in P_1$. We start with the case that there is an edge between $F_{P_0}$ and $F_{P_1}.$

\begin{lemma} \label{lemma_paths}
Let $P_0,P_1$ be two disjoint highways, and assume that there is an edge $f$ between $F_{P_0}$ and $F_{P_1}$. 
Let $E_0 \subseteq P_0$ be a set of edges in $P_0$ we compare to $P_1$, and $E_1 \subseteq P_1$ be a set of edges in $P_1$ that we compare to $P_0$.
For $i \in \{0,1\}$, at the beginning of the computation, the following information is known by all vertices in $F_{P_i}$: 
\begin{enumerate}
\item The identity of all the edges $E_i$.
\item For each edge $e \in E_i$, the values $\cov(e),\extcov(e,P_{1-i})$.
\item The value $\extcov(P_0,P_1).$
\item The identity of the edge $f$.
\end{enumerate}
We can compute the values $\{\cut(e',e)\}_{e' \in P_0, e \in P_1}$ in the following two ways.
\begin{enumerate}
\item In $O(|E_1|)$ aggregate and broadcast computations in $F_{P_0}$, where at the end of the computation each edge $e' \in E_0$ would know the values $\cut(e',e)$ for all edges $e \in E_1$. 
\item In $O(|E_0|)$ aggregate and broadcast computations in $F_{P_1}$, where at the end of the computation each edge $e' \in E_1$ would know the values $\cut(e',e)$ for all edges $e \in E_0$. 
\end{enumerate}
\end{lemma}

% \begin{proof}
% We focus on the case where the computations are done in $F_{P_1}$, the second case is symmetric.
% We work as follows. First, we use the edge $f$ to pass information from $F_{P_0}$ to $F_{P_1}$. Note that all vertices in $F_{P_0}$, know all the values $\{\cov(e),\extcov(e,P_1)\}_{e \in E_0}$. Since $f$ has one endpoint in  $F_{P_0}$ it knows this information and can pass it to all vertices in $F_{P_1}$ using $O(|E_0|)$ aggregate and broadcast computations. Now, for each edge $e \in E_0$, we run one aggregate computation in $F_{P_1}$, that allows each edge $e' \in P_1$ compute $\cut(e,e').$ This is done as follows. First, by Claim \ref{claim_cover}, we know that $\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e,e').$ Also, by Claim \ref{claim_cov_highways}, $\cov(e',e) = \extcov(P_0,P_1) + \extcov(e',P_0) + \extcov(e,P_1) + \cov_{F}(e',e)$. Now, for $e' \in E_1$, it already knows $\cov(e'), \extcov(e',P_0), \extcov(P_0,P_1)$ at the beginning of the computation. Also, it learns the values $\cov(e),\extcov(e,P_1)$ as $f$ passed this information to $F_{P_1}$. Hence, the only thing missing to complete the computation is computing $\cov_{F}(e',e)$ which requires one aggregate computation in $F_{P_1}$ per edge $e \in E_0$ by Claim \ref{claim_covl}. To compute the values $\cut(e',e)$ for all $e \in E_0$, we pipeline $O(|E_0|)$ such computations, which completes the proof.
% \end{proof}

We next consider the case that there is no edge between $F_{P_0}$ and $F_{P_1}$.

\begin{lemma} \label{lem:paths_h_h-noedge}
Let $P_0,P_1$ be two disjoint highways, and assume that there is no edge between $F_{P_0}$ and $F_{P_1}$. 
Then, given the values $\extcov(P_0,P_1)$, using one aggregate computation in $F_{P_0}$ and in $F_{P_1}$, 
and by communicating $O(\log n)$ information over a BFS tree, all vertices learn the values $e',e, \cut(e',e)$ for edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal.
\end{lemma}

% \begin{proof}
% Let $e' \in P_0, e \in P_1$. By Claim \ref{claim_cover}, we have $\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e,e').$ Also, by Claim \ref{claim_cov_highways}, $\cov(e',e) = \extcov(P_0,P_1) + \extcov(e,P_0) + \extcov(e',P_1) + \cov_{F}(e',e)$. Now since there are no edges between $F_{P_0}$ and $F_{P_1}$, by definition $\cov_{F}(e',e) = 0$ as this is the sum of costs of edges between $F_{P_0}$ and $F_{P_1}$ that cover $e'$ and $e$. Also, $\extcov(P_0,P_1)$ does not depend on the specific choice of $e'$ and $e$. Hence, if we want to minimize the expression $\cut(e,e')$, it is equivalent to minimizing the expression $(\cov(e) - 2\extcov(e, P_0)) + (\cov(e') - 2\extcov(e',P_1))$. Note that the expression $\cov(e) - 2\extcov(e, P_0)$ does not depend on $e'$, and the expression $\cov(e') - 2\extcov(e',P_1)$ does not depend on $e$. Hence, minimizing the whole expression is equivalent to minimizing each one of the expressions separately.
% We next show that we can find $e \in P_1$ such that $\cov(e) - 2\extcov(e, P_0)$ is minimal, as well as compute this value using one aggregate computation in $P_1$. Similarly, we can find $e' \in P_0$ such that  $\cov(e') - 2\extcov(e',P_1)$ is minimal using one aggregate computation in $P_0.$
% Then, if $P_0$ sends the message $P_0, e', \cov(e') - 2\extcov(e',P_1)$, and $P_1$ sends the message $P_1, e, \cov(e) - 2\extcov(e, P_0)$, for the minimal edges found, using a BFS tree, all vertices can compute the values $e',e,\cut(e',e)$ for the edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal. As discussed above, this value equals to $(\cov(e) - 2\extcov(e, P_0)) + (\cov(e') - 2\extcov(e',P_1)) - 2\extcov(P_0,P_1)$, and we assume that $\extcov(P_0,P_1)$ is known.

% Hence, to complete the proof, we explain how to compute $\cov(e) - 2\extcov(e, P_0)$ in $P_1$ (the equivalent computation in $P_0$ is done in the same way). From Claim \ref{claim_cov_eP}, all edges $e \in P_1$ know the value $\extcov(e,P_0)$, and they also know $\cov(e)$. Hence, each edge $e \in P_1$ knows the value $\cov(e) - 2\extcov(e, P_0)$. To find the edge $e$ that minimizes this expression, we only need to run one aggregate computation in $P_1$ for finding the minimum.
% \end{proof}

\subsection{Both edges in the same highway}\label{sec:both-edge-highway}

%\mtodo{maybe this should be a subsection of 7.3 that discusses highways? In any case, maybe write "both edges in the same highway, as otherwise the distinction from 7.3 is not clear.}

%\TODO{Put claims and lemmas.}
Here we also cover the case when both edges defining the cut are in the same highway $P$ inside a fragment. Let $e_1$ and $e_2$ be the two edges in a highway $P$ inside a fragment $F$ where $e_1$ is closer to the root than $e_2$. Let us also denote the top edge of $P$ (closest to the root of $G$) inside $F$ to be $e_r$ and the bottom edge of $P$ (farthest from the root of $G$) inside $F$ to be $e_d$. As before, we look at the $\cov(e_1, e_2)$. We see that $\cov(e_1,e_2)$ can be broken up into the following parts (See Figure \ref{fig:both-edge-high})\footnote{This is a slight abuse of notation of $\cov(\cdot)$ but is clear from the context.}:
\begin{itemize}
    \item The cost of edges that cover $e_1, e_2$ and have both end-points inside $F_P$: $\cov_F(e_1,e_2)$,
    
    \item The cost of edges with one end point in $F_P$ and the other end-point is a descendant of $e_d$ outside $F_P$ (i.e., occurs below $e_d$): $\extcov(e_1, e_d)$,
    
    \item The cost of edges with one end point in $F_P$ and the other end-point is an ancestor of $e_r$ outside $F_P$ (i.e., occurs above $e_r$): $\extcov(e_2, e_r)$, and
    
    \item The cost of edges that cover $P$ and both end-points outside $F_P$: $\extcov(P)$.
\end{itemize}

\begin{figure}[h!]
    \centering
    \includegraphics[scale =0.6]{both_edge_high.pdf}
    \caption{\small Example of both cut edges $e_1$ and $e_2$ in the same fragment highway in the fragment $F_P$.}
    \label{fig:both-edge-high}
\end{figure}

%\mtodo{edit the statement such that you don't count the same edge twice (in $\cov(e_1,e_d)$ you need to have only one endpoint inside the fragment, etc.) Explain exactly what is each ingredient, I don't think $\cov(P)$ is defined, also $\cov_F$ was defined in the context of two different fragments. Also add a proof for the statement.}

We make the following observation.

\begin{observation}
Let $e_1$ and $e_2$ be two edges on a fragment highway $P$ inside a fragment $F$. Then,
\begin{align*}
    \cov(e_1,e_2) = \cov_F(e_1, e_2) + \extcov(e_1, e_d) + \extcov(e_r, e_2) + \extcov(P).
\end{align*}
\end{observation}

%\mtodo{Add concrete claims that also explain who knows the result at the end. The different components are known to different edges $e_1$ or $e_2$. Should also have a concluding lemma at the end that explains how for each pair $e_1,e_2$, one of the edges knows $\cov(e_1,e_2)$ + explain that this can be done in different fragments in parallel. Need to route some information in the fragment for this.}

\paragraph{Computing $\cov_F(e_1,e_2)$.} 
\begin{claim}
Let $P$ be the fragment highway of a fragment $F_P$. Using two aggregate computation in time $O(\dfrag)$ all edges $e \in P$ can compute the value $\cov_F(e, e')$ where $e'$ is any other edge in $P$. Moreover, this can be done in all fragments parallely.
\end{claim}

% \begin{proof}
% This is similar to the proof of Claim \ref{clm:both-edge-nh}, but we have to perform both forward and reverse aggregate computation inside the fragment $F$ (as in Claim \ref{claim_pipeline_fragment}). Fix $e_1 \in P$. For any $e \in P$ below $e_1$, $e$ can find out the total weight of the edges that covers $e_1$ and $e$ and have both end-points in $F$ by one forward aggregate computation as follows: Any edge $x$ which has one end point in $F$ on a descendant vertex of $e$ can find out whether it covers $e_1$ and have other end-point inside $F$ by an LCA comparison (as in Claim \ref{claim_LCA_labels}). Hence, by a forward aggregate computation inside $F$, starting from the leaf nodes $T(F_P)$ (i.e., $T$ restricted to $F_P$) and aggregating the weight of such non-tree edges, every $e$ below $e_1$ can learn $\cov_F(e_1, e)$. The aggregate computation takes time $O(\dfrag)$. Moreover, this can be done for all $e_1$ in a pipe-lined fashion. As there are $O(\dfrag)$ many edges in $P$, this takes $O(\dfrag)$-rounds in total. For edges $e \in P$ above $e_1$, we do the exact same aggregate computation but in reverse direction on $T(F_P)$ (See Claim \ref{claim_pipeline_fragment}). This also takes $O(\dfrag)$ times. Moreover, as these are aggregate computations inside $F$, this can be done simultaneously in all fragments.
% \end{proof}

\paragraph{Computing $\extcov(e, e_d)$ and $ \extcov(e_r, e)$.}

\begin{claim}
Let $P$ be the fragment highway of a fragment $F_P$. Also, let all vertices in $F_P$ know the identity of $e_r$ and $e_d$. Then, by two aggregate computation in time $O(\dfrag)$, each edge $e\in P$ know the value of $\extcov(e, e_d)$ and $\extcov(e, e_r)$. Moreover, this can be done in different fragments parallelly.
\end{claim}

% \begin{proof}
%  As in Claim \ref{claim_cov_eP_nh}, any edge $x$ which has one end point inside $F$ and covers $e \in P$ will know whether it covers the last edge of $P$. Similarly any edge $y$ which has one end point inside $F$ and covers $e$ will know whether it covers the first edge of $P$. Hence, by an aggregate computation inside fragment $F$, each edge $e$ will know the value of $\extcov(e, e_r)$ by aggregating all edges which covers $e$ and have one end-point below $e$ and the other end-point outside $F$ covering $e_r$ (can be found using LCA labels, see Claim \ref{claim_LCA_labels}). Similarly, using another aggregate computation inside $F$ in reverse direction (see Claim \ref{claim_pipeline_fragment}), each edge $e$ will know the value of $\extcov(e, e_d)$. By Claim \ref{claim_pipeline_fragment}, this can be done in time $O(\dfrag)$. As these are aggregate computations inside $F$, this can be done simultaneously in all fragments.
%  %Denote the subpath of $P$ from $e_r$ up to $e$ to be $P_{e_r,e}$ and that from $e$ to $e_d$ as $P_{e, e_d}$. Note that $T(P_{e_r,e})$ is completely contained in $F$, \mtodo{why? all the fragments below this fragment are also in this subtree. Why is this needed?} whereas $T(P_{e, e_d})$ is not. We denote the portion of $T(P_{e, e_d})$ contained in $F$ as $T_F(P_{e, e_d})$. By two aggregate computations---one inside $T_F(P_{e, e_d})$ and another inside $T(P_{e_r,e})$ \mtodo{I don't think I understood what you mean by this subtree. I think you need to do one aggregate computation in the reverse direction here (as was done in previous subsections), and then you don't work exactly with this subtree} ---each vertex in $v \in P$ \mtodo{who is $v$? Is it one of the endpoints of $e$? As far as I understand, after running aggregate computations, one endpoint of $e$ would know one value, and the second would know the second one. We later should route information in the fragment to let everybody learn this information for all $e$.} knows two values: (i) The total weight of edges that cover $e$ and have one endpoint in $T_F(P_{e, e_d})$ and the other endpoint outside $F$ (i.e., $\cov(e_r, e)$), and (ii) the total weight of edges that cover $e$ and have one endpoint in $T(P_{e_r,e})$ and the other endpoint outside $F$ (i.e., $\cov(e, e_d)$. Computing these values inside different components can be done in parallel fashion. In total, this takes $O(\dfrag)$ rounds of communication. 
%  \end{proof}

\paragraph{Computing $\extcov(P)$.}
\begin{claim}
Let $P$ be the fragment highway of $F_P$. Using one aggregate and one broadcast computation over a BFS tree of $G$, every vertex will know the value of $\extcov(P)$. For $k$ many fragments, this can be done in time $O(k + D)$.
\end{claim}

% \begin{proof}
% This can be done similar to Claim \ref{clm:two-short-highway}. Every edge knows whether it covers both $e_r$ and $e_d$ or not, and also whether both of its endpoints outside $F_P$ or not. Now, by using one aggregate computation over a BFS tree of $G$, we can compute the total weight of such edges, and then by using the same BFS tree, this information can be broadcasted to all vertices. This takes $O(D)$ rounds of communication. For different fragments, this computation can be pipelined, and hence can be performed in $O(k + D)$ time.
% \end{proof}

\paragraph{An algorithm for a highway path.} We now explain how we can compute $\cut(e, e')$ when both $e$ and $e'$ belong to a  fragment highway path $P$ of a fragment $F$.

\begin{lemma} \label{lem:both-edge-short-high}
Let $P$ be a fragment highway of a fragment $F$. Also, let every edge $e$ know the value of (i) $\cov(e)$, (ii) $\cov_F(e, e')$ for all other edges $e' \in P$, (iii) $\extcov(e, e_r)$ and $\extcov(e, e_d)$, and (iv) $\extcov(P)$. Then, in $O(\dfrag)$ rounds, each pair of edges $(e, e')$ in $P$ can compute the value of $\cut(e, e')$. Moreover, this can be done parallelly in all fragments $F$.
\end{lemma}

% \begin{proof}
% Fix a pair of such edges $(e, e')$ where $e$ is above $e'$. For $e$ and $e'$ to know the value of $\cut(e, e')$, $e$ needs to know the value of $\extcov(e', e_r)$ which is with $e'$ and $e'$ needs to know the value of $\extcov(e, e_d)$ which is with $e$. To this end, each edge $e$ broadcasts the values $\extcov(e, e_r)$ and $\extcov(e, e_d)$ inside the fragment $F$. This is, in total, $\tO(\dfrag)$ bits of information broadcasted over a BFS tree of depth $O(\dfrag)$ (because of the guarantee that the diameter of $F$ is $O(\dfrag)$), hence can be done in time $\tO(\dfrag)$ in pipelined fashion. As the broadcast is happening inside $F$, this can be done parallelly for all fragments $F$.
% \end{proof}



==> 8.1-old-min-2-respecting-cut.tex <==


\mtodo{I think this whole part can be removed for now. Just left it here in case somebody needs it.}

We will next explain how to find the 2 tree edges $e,e'$ that define the minimum cut, we will focus first on the case that $e,e'$ are not in the same root to leaf path. We will divide to cases depending if the edges $e,e'$ are part of a highway or a non-highway.
We need the following definitions and claims.

%\begin{claim} \label{claim_layer}
%Each path in layer $i$ is potentially interested in $O(\log{n})$ paths from layer $j \geq i$.
%\end{claim}














\begin{claim} \label{claim_interested}
In ... time, all edges can learn about $O(\log{n})$ paths they are potentially interested in, that include all the paths they are interested in. \mtodo{what is the exact information they learn about the paths? We should add a clear explanations somewhere and also explain how this information is used in the algorithm.}
\end{claim}

\remove{
\begin{claim} \label{claim_edge}
If $P$ and $P'$ are two paths between an ancestor to a descendant, not in the same root to leaf path, and $P'$ is potentially interested in $P$, then there is an edge between $T(P^{\downarrow})$ and $T(P'^{\downarrow}).$
\end{claim} 

\mtodo{add proof.}
}

\begin{claim}[\sagnik{New}] \label{claim_edge_nonortho}
If $P$ and $P'$ are two paths between an ancestor to a descendant in the same root to leaf path where $P'$ occurs further from the root than $P$, and $P'$ is potentially interested in $P$. Also assume that the deepest node of $P$ is $d_P$. Then there is an edge between $T - T(d_P^{\downarrow})$ and $T(P'^{\downarrow}).$
\end{claim}

\mtodo{I'm not sure about the notation $d_P$ in the above claim, because it's confusing with $d_P$ which is used as the descendant of the highway $P$. Also, we should add a proof.}

\subsection{Algorithm description}

The algorithm works in $L^2 = O(\log^2{n})$ iterations, where each iteration corresponds to two indexes $1 \leq i \leq j \leq L$. In iteration $(i,j)$ we take care of min 2-respecting cuts with one edge in layer $i$ and one edge in layer $j$. We next focus on one such iteration. We assume that at beginning of the computation, each edge $e$ knows $\cov(e)$, which can be obtained in $\tilde{O}(D+\sqrt{n})$ rounds by Claim \ref{claim_learn_cov}. 

At this point, we also assume that the graph is decomposed into fragments \textit{viz.}~Claim \sagnik{Refer to appropriate claim. What will the vertices know?} We will view the juxtaposition of the layering decomposition and the fragment decomposition on $T$ by using the following definition: By a \textit{non-highway path in layer $i$}, we denote the sub-path of a non-highway path (obtained by the fragment decomposition) which is completely contained in layer $i$ (obtained by the layering decomposition). \sagnik{Do we do the same for highway?}

Formally, before the beginning of the algorithm, each vertex $v$ of $G$ will know the following information: \begin{enumerate}
    \item For each edge $e \in T$ incident on $v$, the cover value of $e$, $\cov(e)$ (\textit{viz.}~Claim \ref{claim_learn_cov}),
    \item For each edge $e$ incident on $v$, the index of the layer $i$ such that $e \in E_i$ obtained from the layering decomposition (\textit{viz.}~Property \ref{clmitem:info_vertex} of Claim \ref{claim:-layerDecomp}),
    \item For each edge $e$ incident on $v$, the index of the fragment that $e$ is in, and whether $e$ is a part of the highway or a non-highway of that fragment (\textit{viz.}~Claim \ref{clm:time-fragment}).
\end{enumerate}

Next we describe three parts of the algorithm which happen in parallel. In the first part, the goal is to inform every vertex the minimum cut value $\min \cut(e,e')$ where $e$ and $e'$ both occur in non-highways. In the second part, one of $e$ and $e'$ occur in a highway, and the third part deals with the case where both $e$ and $e'$ occur in highways.

\subsection{Both cut edges in non-highway}

In this section, we prove the following lemma.

\begin{lemma} \label{lem:main_nh-nh}[\yuval{check correctness, checked, seems ok to me for the orthogonal case}]
In time $O(D + \dfrag \log^3 n)$ each vertex $v$ of $G$ will know 
two edges $e', e$ such that $(e',e) = \arg \min_{\{e', e\}} \cut(e',e)$, as well as the value $\cut(e',e),$ where $e'$ and $e$ are edges in a pair of (orthogonal) non-highway paths.
\end{lemma}

\mtodo{In the above lemma I think we also want to learn the edges (I've added this), so we can infer the actual cut. Also, why is the word orthogonal in brackets?}


As stated above, there are $L^2$ many iterations, each of which can be identified with an unordered pair $(i,j)$ where $1 \leq i \leq j \leq L$. In iteration $(i,j)$ we look at all the non-highway paths $P'$ of layer $i$ and compare them to non-highway paths $P$ of layer $j$. We also assume that $P'$ and $P$ are not in the same root to leaf path. Note that all paths in the same layer are not in the same root to leaf path. In addition, by Claims \ref{claim:-layerDecomp} and \ref{claim_interested}, each path from layer $i$ is potentially interested only in $O(\log{n})$ paths from layer $j \geq i$, and all the edges of the path already know the paths they are potentially interested in. \mtodo{what is the exact information they know?}

We next fix a path $P'$ from layer $i$ and a path $P$ in layer $j$ that $P'$ is potentially interested in. Our goal is to find two edges $e' \in P', e \in P$ such that $(e',e) = \arg \min_{\{e' \in P', e \in P\}} \cut(e',e)$, as well as the value $\cut(e',e).$ For this, we show that each edge $e' \in P'$, can learn all the values $\{\cut(e',e)\}_{e \in P}$. All edges learn this simultaneously in a time that is proportional to the diameter of fragments. \mtodo{I currently work with $O(n^{1/3})$ fragments of diameter $O(n^{2/3})$, the numbers should be updated later.}

For proving \Cref{lem:main_nh-nh}, we need the following claims. The first claim states, informally, that it is efficient to broadcast information inside all non-highway paths in the same layer. 

\begin{claim} \label{claim_broadcast}
Fix a layer $j$, and assume that for each non-highway path $P$ in layer $j$ there are $k$ pieces of information of size $O(\log{n})$ where initially each one of them is known by some vertex in $T(P)$. In $O(\dfrag + k)$ rounds, all the vertices in $T(P)$ can learn all the $k$ pieces of information. In addition, this computation can be done in all non-highway paths $P$ in layer $j$ in parallel.
\end{claim}

\begin{proof}
Note that since $P$ is a non-highway path, the entire subtree $T(P)$ is in the fragment of $P$ and has diameter $\dfrag$.
To solve the task, we use pipelined upcast and broadcast in the subtree $T(P)$. First, we collect all $k$ pieces of information in the root $r_P$, and then broadcast them to the whole tree $T(P)$, using pipelining this takes $O(\dfrag + k)$ rounds.  Additionally, as the different trees $T(P)$ of paths $P$ in layer $j$ are edge disjoint by Claim \ref{claim_disjoint}, the computation can be done in parallel for all non-highway paths in layer $j$.  
\end{proof}

The next claim provides sufficient condition for efficient computation of 2-respecting cut values when the pair of constrained edges reside in different non-highway paths. Note that this claim does not assume anything about the orthogonality of these two paths.

\begin{claim} %\label{claim_non_highway}
Let $P'$ be a non-highway path, and assume the following:\begin{itemize}
    \item Let $\{e_i,\cov(e_i)\}_{i=1}^{k}$ be a collection of $k$ tuples that are known to all vertices in $T(P')$,
    \item None of the edges $\set{e_i}_{i \in [k]}$ occur in $T(P')$. \mtodo{Note this property when proving the case of two edges in the same root to leaf path. It seems important which edge does the computation there.}
\end{itemize} Then, in $O(\dfrag+k)$ rounds, each edge $e' \in P'$ can compute all the values $\{e_i,\cut(e',e_i)\}_{i=1}^{k}.$ In addition, for different paths $P'$ that are not in the same root to leaf path, these computations can be done in parallel.
\end{claim}

\begin{proof}
Let $e' \in P'$, and fix an edge $e \in \{e_i\}_{i=1}^k$. By Claim \ref{claim_cover}, $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e)$. Also, $e'$ knows $\cov(e)$ and $\cov(e')$, hence to compute $\cut(e',e)$, $e'$ should compute $\cov(e',e).$ As any edge that covers a tree edge $e'=\{v',p(v')\}$ where $p(v')$ is the parent of $v'$, has one endpoint in the subtree of $v'$, it follows that the edges that cover $e'$ and $e$ are exactly all the edges that cover $e$ and have one endpoint in the subtree of $v'$. This subtree is contained in $T(P')$.
Hence, to learn about the total cost of these edges we need to do one aggregate computation in $T(P')$: letting each vertex $v' \in T(P'^{\downarrow})$ learn about the total cost of edges incident on the subtree of $v'$ that cover $e$. This can be done using a convergecast in $T(P')$, where each vertex sends to its parent the total cost of edges in its subtree that cover $e$, this includes the sum of costs of edges it receives from its children and the cost of such edges adjacent to it. To implement this efficiently we need an efficient way to determine for each non-tree edge whether it covers a specific edge $e$, this can be done using Claim \ref{claim_LCA_labels}. Hence, when we fix an edge $e$, all the edges $e' \in P'$ can compute $\cut(e',e)$ using one convergecast in the subtree of $P'$. To do so for all $k$ edges in $\{e_i\}_{i=1}^k$, we run $k$ such computations in $T(P')$, using pipelining the complexity of all the computations is $O(\dfrag+k)$. At the end, each edge $e' \in P'$ knows the values $\cut(e',e)$ for all edges $e \in \{e_i\}_{i=1}^k.$ 

Since the whole computation was done in $T(P')$, the same computation can be done in parallel for other paths not in the same root to leaf path with $P'$.
\end{proof}

The following claim uses Claim \ref{claim_non_highway} to come up with a procedure to compute 2-respecting cut values where the constrained edges reside on two \textit{orthogonal} non-highway paths. \mtodo{I don't remember which is orthogonal, but you use this terminology both here and in the second case, in one of them it should be not orthogonal.}\yuval{Orthogonal is not the same root to leaf path}

\begin{lemma} \label{lemma_non_highway}
Let $P'$ be a non-highway path in layer $i$, and let $P$ be a non-highway path in layer $j \geq i$ such that $P'$ is potentially interested in $P$, and $P$ is not in the same root to leaf path with $P'$. In $O(\dfrag)$ rounds, each edge $e' \in P'$, learns all the values $\{e, \cut(e',e)\}_{e \in P}$.
\end{lemma}

\begin{proof}
First, we observe the following: 
\begin{itemize}
    \item[(i)] As $P'$ is potentially interested in $P$ there must be an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow})$ by Claim \ref{claim_edge} \mtodo{I think that this is the only place we use the fact that they are not in the same root to leaf path}.
    
    \item[(ii)] Since the trees $T(P^{\downarrow})$ are disjoint for paths in the same layer, the edge $f$ is different for different pairs $P',P$.
\end{itemize}
The goal is to use $f$ \mtodo{we should also explain how to decide about the edge $f$} to let all vertices of $P'$ learn about all the values $\{e,\cov(e)\}_{e \in P}$. Once this is done, using Claim \ref{claim_non_highway}, each edge $e' \in P'$ computes all the values $\{e, \cut(e',e)\}_{e \in P}$ in $O(n^{2/3})$ time. The rest of the proof is to show how the vertices of $P'$ know the required information to compute the cut values.

The procedure can be divided into three phases:
\begin{description}
\item[- Aggregation.] We use Claim \ref{claim_broadcast} to let all vertices in $T(P)$ learn all the values $\{e,\cov(e)\}_{e \in P}$. Note that at the beginning $\cov(e)$ is known to $e \in T(P)$, hence the condition of the claim holds. As $P$ is non-highway, this is $O(n^{2/3})$ information, hence this takes $O(n^{2/3})$ time. This computation is done in all non-highway paths in layer $j$ in parallel.

\item[- Tunnelling.] As $f$ has an endpoint in $T(P)$ and an endpoint in $T(P')$, in $O(n^{2/3})$ time all the information $\{e,\cov(e)\}_{e \in P}$ is also known by a vertex in $T(P')$.

\item[- Dissipation.] We can use Claim \ref{claim_broadcast} again to let all vertices in $T(P')$ learn this information.
\end{description}
To reiterate, after these three steps, each vertex can compute \mtodo{what happened to the end of the proof here?}
\end{proof} 

\begin{proof}[\sagnik{Proof of orthogonal case}] \mtodo{here again you use orthogonal}\yuval{should be not orthogonal here}
For the case when $P$ and $P'$ occur in the same root-to-leaf path, we are going to use the following structures:
\begin{itemize}
    \item[(i)] Note that there can be exactly 1 $P$ in layer $i$ that $P'$ in layer $j$ is (potentially) interested in. \yuval{why is this true? If $j\geq i$, how do you bound the number of paths of lower layer in the same root to leaf path that $j$ is interested in?}
    
    \item[(ii)] $P$ and $P'$ belong to the same fragment. Hence the path between $P$ and $P'$ is of length at most $\dfrag$.
    
    \item[(iii)] All $P'$ that $P$ is interested in share a common LCA which is the only intersection point of such $P'$s.
    
    \item[(iv)] The path between $P$ and the $P$'s that $P$ is interested in is unique for each $P$ in layer $i$.
\end{itemize}

\mtodo{I didn't understand why properties 3 and 4 hold. What happens if we have a path of layer $i$ that many different paths of layer $i-1$ attached to different vertices in it?}

So the procedure goes the following way:
\begin{itemize}
    \item As before, we first employ Claim \ref{claim_broadcast} to let every edge $v \in T(P)$ know the set $\{e, \cov(e)\}_{e \in P}$. This is $O(\dfrag)$-bits of information. We only need the vertex $d_P$ to know this information. \mtodo{again, $d_P$ is used for something else (unique descendant in a fragment) so maybe we can find a different notation.}
    
    \item We then want to let the top vertex of $P'$ know about this information using the path between $P$ and $P'$. To this end, $d_P$ pipelines this information to the LCA of all $P'$'s that $P$ is interested in. This can be done parallely for each $P$ in layer $i$ without any cross-congestion. \mtodo{I think we need a different argument here. The paths are not disjoint, but we want to learn the same information, so it's ok.}
    
    \item We then want to dissipate this information to every edge of $P'$ by again using Claim \ref{claim_broadcast}.
    
    \item Now we use Claim \ref{claim_non_highway} to let every edge $e' \in P'$ compute the set $\set{e, \cut(e, e')}_{e \in P}$. \yuval{the second condition of the claim \ref{claim_non_highway} does not hold though.}
\end{itemize}
\end{proof}

\begin{proof} [Proof of \Cref{lem:main_nh-nh}] We next explain how Lemma \ref{lemma_non_highway} allows to learn about the min 2-respecting cut that is defined by two tree edges in non-highways, not in the same root to leaf path. \Cref{alg:nh-nh} provides a schematic representation of the procedure.

\begin{center}
  \centering
  \begin{minipage}[H]{0.8\textwidth}
\begin{algorithm}[H]
\caption{Schematic algorithm when both edges are in non-highway}\label{alg:nh-nh}
\begin{algorithmic}[1]
\For{every pair $\set{i,j}$ from $L$, $i \leq j$}
    \For{Every non-highway $P'$ in layer $i$ and $P$ in layer $j$}
        \If{$P'$ is potentially interested in $P$}
            \State Each edge $e' \in P'$ computes $\set{e, \cut(e,e')}_{e \in P}$.
            \State $e'$ records $e \in P$ for which $\cut(e,e')$ is the minimum. 
            \Statex \Comment{\Cref{lemma_non_highway}}
        \EndIf
    \EndFor
\EndFor
\State Each edge $e$ performs convergecast along a BFS tree to send the minimum to the root.
\State Root performs downcast to let every vertex know the minimum.
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{center}

As explained above, we have $O(\log^2{n})$ iterations $(i,j)$, where in iteration $(i,j)$ we deal with non-highways in layer $i$ and $j$ for $i \leq j.$ In this iteration, we look at all non-highway paths $P'$ in layer $i$ and the non-highway paths $P$ in layer $j$ they are potentially interested in. Since each path in layer $i$ is potentially interested only in $O(\log{n})$ paths in layer $j$, we just need to apply the computation from Lemma \ref{lemma_non_highway}, $O(\log{n})$ times per path $P'$. In addition, it follows from the proof of Lemma \ref{lemma_non_highway} and Claims \ref{claim_broadcast} and \ref{claim_non_highway} that these computations can be done in parallel for different paths $P'$ in the same layer, as the trees $T(P')$ are edge disjoint for such paths. Summing up over all iterations we get a complexity of $O(\dfrag\log^3{n})$ rounds. At the end of the computation, for any two paths $P',P$ where $P'$ is in layer $i$ and is potentially interested in $P$ in layer $j$, each edge $e' \in P'$ knows the values $\{e, \cut(e',e)\}$ for all $e \in P.$ In particular, for any such 2-respecting cut, there is a vertex that knows about the 2 edges in the cut and the value of the cut. 
At the very end of the computation, we can use convergecast in a BFS tree to let all vertices learn the minimum 2-respecting cut and its value in $O(D)$ rounds. Overall, this sums up to a complexity of $O(D+\dfrag\log^3{n})$ rounds.
\end{proof} 



\subsection{Exactly one cut edge in highway}
\yuval{In all places that mention interested, should be changed to potentially interested+might need to change the $O(\log n)$ to some $polylog(n)$.}
\mtodo{Something we should add to all sections is how we distinguish between different cases: how do we know if we are in a highway/non-highway, orthogonal/non-orthogonal case, etc. In particular, we later break into cases according to whether there are edges between fragments or not, and if so we use a particular edge $f$, we need to explain how do we know in which case we are and how do we find the edge $f$.}

Here we compare non-highway paths $P'$ in layer $i$, to highway paths in layer $j$, where $i,j$ can be any indexes of layers. 
We will use Claim \ref{corol:-_layer_highway} that says that each non-highway path $P'$ is only interested in $O(\log{n})$ root to leaf paths composed of highways. However, note that such root to leaf path $P_H$ may be composed of many (possibly $O(\nfrag)$) different highways, hence just passing to $P'$ the information about all edges in the path $P_H$ can result in a linear complexity.
To get a sublinear complexity we use the following key ingredients. First, we use a certain monotonicity to break the path $P'$ to (almost) disjoint subpaths, each one of them is only interested in one highway in $P_H$.\yuval{Notation here needs to be improved and more formally defined.} Second, for different highways $P \in P_H$ that $P'$ is potentially interested in, we divide the computation between $P'$ and $P$ differently. If there is only small number of edges in $P$ that are interested in $P'$, we pass the relevant information to $P'$ and let $P'$ do the computation. If, on the other hand, many edges in $P$ are interested in $P'$, we let $P$ do the computation. Building on these ideas, we get a sublinear complexity. We next describe the algorithm in detail.

Fix a layer $i$, and a non-highway path $P'$ in layer $i$. As each edge in $P'$ knows about the paths it is potentially interested in and there are $O(\log{n})$ of them per edge, we can also let all vertices in $T(P')$ learn this information using Claim \ref{claim_broadcast} $O(\log{n})$ times, which takes $O(n^{2/3} \log{n})$ time. Using this information, all vertices in $P'$ can learn all the highway paths that $P'$ is potentially interested in. \mtodo{more details about the exact information known.} By Claim \ref{corol:-_layer_highway}, $P'$ is only potentially interested in $O(\log{n})$ root to leaf paths composed of highways. We next fix one such path $P_H.$ 
We focus on the case that $P'$ and $P_H$ are in different fragments, and not in the same root to leaf path.\mtodo{should handle somewhere other cases.}

For the algorithm, we first need to partition $P'$ into sub-segments. We start by describing the partition, and then show how we exploit it in the algorithm. 

\subsubsection*{First part: partitioning $P'$}

Let $P \in P_H$ be a highway. We denote by $e_P^{h},e_P^{\ell}$ the highest and lowest edges in the highway $P$, respectively. 
Define $P'(e_P^{h})$ to be an edge in $P'$ such that $\cut(P'(e_P^{h}),e_P^{h})$ is minimal. If there is more than one such edge, take the edge that is highest in $P'$. Define $P'(e_P^{\ell}) \in P'$ similarly with respect to $e_P^{\ell}$ (again, taking the highest possible edge if there is more than one option). First, we show that we can compute these edges efficiently.

\begin{claim}
In $O(D+n^{2/3})$ rounds, all vertices in $T(P')$ can learn the edges $P'(e_P^{h}), P'(e_P^{\ell})$ for all $P$. In addition, this computation can be done in all paths $P'$ in layer $i$ simultaneously.
\end{claim}

\begin{proof}
First, as there are $O(n^{1/3})$ highways, and we only consider two edges per highway, we can let all the vertices in the graph learn in $O(D+n^{1/3})$ rounds all the values $\{e,\cov(e)\}$ for $e$ that is equal to $e_P^{h}$ or $e_P^{\ell}$ for some highway $P$, using upcast and broadcast in a BFS tree. Then, we use Claim \ref{claim_non_highway}, to let all edges $e' \in P'$ to compute $\cut(e',e)$ for all relevant edges $e$. This requires $O(n^{1/3})$ aggregate computations in $T(P')$, and can be done in the same time for all paths $P'$ in layer $i$. Now per each edge $e$, we use convergecast and broadcast in $T(P')$ to let all vertices learn the highest edge $e'$ such that $\cut(e',e)$ is minimum. Using pipelining, this takes $O(n^{2/3}+n^{1/3})=O(n^{2/3})$ time for all edges. At the end, all vertices of $T(P')$ learn the edges $P'(e_P^{h}), P'(e_P^{\ell})$ for all $P$. As all the computations are done in $T(P')$, we can work in parallel in different paths $P'$ in the same layer.
\end{proof}

\sagnik{There must be a better nomenclature than $P'(e^h_P), E_{P'}(P)$, and $x_{P'}(P)$. We need to find those.}

After computing the minimal edges, we would like to use the monotonicity described in  \Cref{claim_monotonicity}, to divide $P'$ to (almost) disjoint sub-paths, and compare each one of them only to one highway $P \in P_H$. This is done as follows. 
We denote by $E_{P'}(P)$ all the edges in $P'$ between $P'(e_P^{\ell})$ and $P'(e_P^{h})$.
In our algorithm, the only edges in $P'$ that are compared to the highway $P$ are in $E_{P'}(P)$.
Note that all vertices in $T(P')$ know the edges $P'(e_P^{h}), P'(e_P^{\ell})$. We can also assume that all vertices in $T(P')$ know the complete structure of $P'$. This follows, since using pipelined upcast and broadcast, all edges in $T(P')$ can learn all the edges in $P'$ in $O(n^{2/3})$ time, as this is the length of $P'$. Based on this information, all edges in $P'$ know to which subsets $E_{P'}(P)$ each edge of $P'$ belongs, summarized as follows.

\begin{claim} \label{claim_know_Ep}
In $O(n^{2/3})$ time, all vertices in $T(P')$ learn the complete structure of $P'$, and the sets $E_{P'}(P).$ This computation can be done in all paths $P'$ in layer $i$ simultaneously.
\end{claim}
\yuval{proof of this claim needs to be more formal.}

We next show that it is indeed enough to compare only the subset $E_{P'}(P)$ to $P$, and then bound the total number of comparisons required by the algorithm.

\begin{claim} \label{claim_compare}
Assume that $(e',e) = \arg\min_{\{e' \in P', e \in P_H\}} \cut(e',e)$, then even if for any highway $P \in  P_H$, we only compare edges in $E_{P'}(P)$ to $P$, we learn about a min 2-respecting cut with value $\cut(e',e).$
\end{claim}
\yuval{A different wording? Maybe stating that the min value restricted only to the edges we are comparing equals the min value when we compare all pairs of edges.}

\begin{proof}
Let $P \in P_H$ be the highway such that $e \in P.$ If $e=e_P^h$ or $e=e_P^{\ell}$, we already computed an edge $e'' \in P'$ such that $\cut(e'',e)$ is minimal as needed. Otherwise, we use Claim \ref{claim_monotonicity} to show that there is an edge $e'' \in E_{P'}(P)$ such that $\cut(e'',e)$ is minimal. First, note that from Claim \ref{claim_monotonicity}, and since $e_P^{h}$ is above $e_P^{\ell}$, we have that $P'(e_P^{\ell})$ is either equal to $P'(e_P^{h})$ or below it. 
Next, we use Claim \ref{claim_monotonicity} on $e$ and $e_P^{h}$. Since $e_P^{h}$ is closer to the root compared to $e$, we have that the highest edge $e''$ such that $\cut(e'',e)$ is minimal is either $P'(e_P^h)$ or below it. Similarly, from using Claim \ref{claim_monotonicity} on $e$ and $e_P^{\ell}$ which is below $e$, we have that $e''$ is either equal to $P'(e_P^{\ell})$ or it is above it. To conclude, $e'' \in P'$ is between $P'(e_P^{\ell})$ to $P'(e_P^{h})$, hence by definition $e'' \in E_{P'}(P)$ as needed.
\end{proof}

We denote by $x_{P'}(P)$ the number of edges in $P'$ that we compare to the highway $P$. We next bound the number of comparisons required by the algorithm.

\begin{claim} \label{claim_xP'}
$\sum_{P \in P_H} x_{P'}(P) = O(n^{2/3}).$
\end{claim}

\begin{proof}
We have that $x_{P'}(P) = |E_{P'}(P)|$, we next use Claim \ref{claim_monotonicity} to show that the different sets $E_{P'}(P)$ are almost disjoint. The set $E_{P'}(P)$ includes all edges between $P'(e_P^{\ell})$ and $P'(e_P^{h})$. Also, as explained in the proof of Claim \ref{claim_compare}, the edge $P'(e_P^{\ell})$ is equal or below $P'(e_P^{h})$. For any edge $e' \in P'$ which is strictly above $P'(e_P^{\ell})$ and strictly below $P'(e_P^{h})$, we only compare it to $P$. The reason is as follows. From Claim \ref{claim_monotonicity}, for any edge $e \in P_H$ in a highway above $P$, the edge $e'' \in P'$ such that $\cut(e'',e)$ is minimal is $P'(e_P^{h})$ or above it. Similarly, for any edge $e \in P_H$ in a highway below $P$, the edge $e'' \in P'$ such that $\cut(e'',e)$ is minimal is $P'(e_P^{\ell})$ or below it. This means that for any highway $Q \neq P$, both the edges $P'(e_Q^{\ell}),P'(e_Q^{h})$ are either both above $e'$ or both below $e'$. This means that $e'$ is only in the set $E_{P'}(P)$. This means that the set $E_{P'}(P)$ includes $|E_{P'}(P)| - 2$ edges that are not in the set $E_{P'}(Q)$ for any $Q \neq P$ (assuming its size is at least 2), and the two edges $P'(e_P^{\ell}), P'(e_P^{h})$. If we sum over all sets, we get that $$\sum_{P \in P_H} x_{P'}(P) = \sum_{P \in P_H} |E_{P'}(P)| = O(n^{2/3} + n^{1/3}) = O(n^{2/3}).$$ The first term counts all the edges that are only in one set $E_{P'}(P)$, the number is bounded by the $O(n^{2/3})$ edges in $P'$. The second term counts the two edges $P'(e_P^{\ell}), P'(e_P^{h})$ per highway $P$. Here, an edge may be counted more than once, but per highway we only have two such edges, hence the total number is bounded by the number of highways, $O(n^{1/3}).$ This completes the proof.
\end{proof}

\subsubsection*{Second part: finding the min 2-respecting cut}

\sagnik{\begin{enumerate}
    \item The algorithm description needs to be enumerated/itemized.
    
    \item There needs to be a separate notation section.
    
    \item Need to spell out that $P$ in layer $j$, and $P'$ in layer $i \leq j$. \mtodo{the algorithm doesn't have this property, it may be the case that the highway has a lower layer.}
\end{enumerate}}

We next explain how we exploit the partition described above in our algorithm. 
We need the following definitions and claims.
Let $P'$ be a non-highway, and $P$ be a highway not in the same root to leaf path with $P'$. Let $e' \in P', e \in P$. We next take a closer look at the value $\cov(e',e).$ Any edge that covers $e'=\{v',p(v')\}$ and $e=\{v,p(v)\}$ has one endpoint in the subtree of $v'$ and one endpoint in the subtree of $v$. The first is contained in $T(P'^{\downarrow})$, which is contained in the fragment of $P'$, as $P'$ is a non-highway. The second is contained in $T(P^{\downarrow})$, however, since $v$ is on a highway, this subtree is not contained entirely in the fragment $F_P$ of $P$. The subtree of $v$ has one part in $T(P^{\downarrow}) \cap F_P$, and the other part in $T(P^{\downarrow}) \setminus F_P$, which is below the fragment $F_P$. 
We denote by $\cov_{F_P}(e',e)$ the cost of all the edges that cover $e'$ and $e$ and have one endpoint in $T(P^{\downarrow}) \cap F_P$, and by $\cov(e',P)$ the cost of all the edges that cover $e'$ and have one endpoint in $T(P^{\downarrow}) \setminus F_P$. Note that from the structure of the fragments any such edge covers $e'$ and the whole highway $P$, i.e., $\cov(e,e') = \cov_{F_P}(e',e) + \cov(e',P)$. This follows as any such edge has an endpoint in the subtree of the unique descendant $d_P$ of $F_P$, and all the vertices in the subtree of $d_P$ are in the subtrees of all the vertices in the highway $P$. Hence, this second term $\cov(e',P)$ does not depend on the specific choice of $e \in P.$ This is summarized as follows.

\begin{claim} \label{cover_non_highway_highway}
Let $e' \in P', e \in P$ where $P'$ is a non-highway, and $P$ is a highway not in the same root to leaf path with $P'$. Then $\cov(e',e) = \cov_{F_P}(e',e) + \cov(e',P)$, where $\cov_{F_P}(e',e)$ is the cost of all edges that cover $e'$ and $e$ and have one endpoint in the subtree $T(P^{\downarrow}) \cap F_P$, and $\cov(e',P)$ is the cost of all edges that cover $e'$ and have one endpoint in $T(P^{\downarrow}) \setminus F_P$.
\end{claim}

We denote by $x_P(P')$ the number of edges in the highway $P$ that are potentially interested in the non-highway path $P'$. Note that any edge in $P$ is only potentially interested in $O(\log ^3 n)$ paths not in the same root to leaf path \sagnik{Which claim to ref?} \mtodo{update the number if needed}. \yuval{Ill change the number again if needed.} Also, different non-highways in the same layer are not in the same root to leaf path, which means that any edge in $P$ is only potentially interested in $O(1)$ such non-highways. \yuval{why is this true?} As there are $O(n^{2/3})$ edges in $P$, this gives the following.

\begin{claim} \label{claim_xP}
$\sum_{P'} x_P(P') = O(n^{2/3})$, where we sum over all non-highways $P'$ of a fixed layer $i$.
\end{claim}


We now go over all highways $P \in P_H$ and find the min 2-respecting cut of $P'$ and $P$. We have several cases.

\paragraph{There are no edges between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$.}
Let $e' \in P', e \in P.$ From Claim \ref{claim_cover}, we have that $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e).$ 
In addition, from Claim \ref{cover_non_highway_highway}, we have that $\cov(e',e) = \cov_{F_P}(e',e)+\cov(e',P)$. Since any edge that covers $e'$ and $e$ has one endpoint in $T(P'^{\downarrow})$ and one endpoint in $T(P^{\downarrow})$, and there are no edges between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$, we have that $\cov_{F_P}(e',e) = 0$ in our case. This means that $\cov(e',e) = \cov(e',P)$ in our case, which is the cost of edges that cover $e'$ and have one endpoint in $T(P^{\downarrow}) \setminus F_P$. This means that the expression $\cov(e',e)$ does not depend on the specific choice of $e$ in $P$.
Hence, for any $e' \in P'$, the expression $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',P)$ is minimized for $e \in P$ such that $\cov(e)$ is minimal. Also, as this is only one edge $e$ per fragment we can let all vertices learn $e$ and $\cov(e)$ in $O(D+\nfrag)$ rounds using a communication in a BFS tree. Hence, we now only need to compute $\cut(e',e)$ for all $e' \in P',$ for $e \in P$ such that $\cov(e)$ is minimal. This requires one aggregate computation per edge $e$, and can be done for all such highways $P$ in $O(n^{2/3})$ rounds using Claim \ref{claim_non_highway}. Moreover, this is done for all paths $P'$ in layer $i$ simultaneously. 


\paragraph{There are edges between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$, and $x_P(P') \leq x_{P'}(P).$}
Here we let $P'$ compute the values $\cut(e',e)$ for $e' \in P', e \in P.$ For this, we use an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$ to pass to $P'$ the information $\{e,\cov(e)\}$ for all edges in $P$ that are potentially interested in $P'$. Then, we can use Claim \ref{claim_non_highway} to compute the values $\cov(e',e).$ We next describe the computation in detail. Note that since the trees $T(P'^{\downarrow})$ are disjoint for different paths $P'$ in the same layer, and the fragments $F_P$ are disjoint for different highways, the edge $f$ for different pairs $P',P$ is different.

First, as each edge in $P$ is only interested in $O(1)$ non-highway paths in layer $i$ \sagnik{Do we have a claim to ref?}, we can let all vertices of $F_P$ learn for each highway edge $e$ the value $\cov(e)$ and the non-highway paths of layer $i$ that $e$ is potentially interested in, using upcast and broadcast in the fragment $F_P$. This requires time proportional to the diameter of the fragment. In addition, from Claim \ref{claim_know_Ep}, all vertices in $T(P')$ can learn in $O(n^{2/3})$ time about all the values $x_{P'}(P)=|E_{P'}(P)|$, recall that this is the number of edges in $P'$ that we compare to $P$. Now, since $f$ has an endpoint in $T(P')$ and an endpoint in $F_P$, it has an endpoint that knows $x_{P'}(P)$, and an endpoint that knows $x_P(P')$, the number of edges in $P$ that are potentially interested in $P'$, and the values $\{e,\cov(e)\}$ for all such edges. In one round, $f$ can check if $x_P(P') \leq x_{P'}(P)$, and if this is the case it passes the information $\{e,\cov(e)\}$ to $T(P')$ for all $x_P(P')$ edges in $P$ potentially interested in $P'$, which takes $O(n^{2/3} + x_P(P'))=O(n^{2/3} + x_{P'}(P))$ time using Claim \ref{claim_broadcast}.
To do so for all paths $P \in P_H$ from this case simultaneously would result in a complexity of $O(n^{2/3} + \sum_{P \in P_H} x_{P'}(P)) = O(n^{2/3})$ rounds using Claims \ref{claim_broadcast} and \ref{claim_xP'}.
Now, we use Claim \ref{claim_non_highway} to let all edges $e' \in P'$ to compute the value $\cut(e',e)$ for each one of the at most $x_{P'}(P)$ edges of $P$ potentially interested in $P'$. Doing so for all highways $P \in P_H$ would result in a complexity of $O(n^{2/3} + \sum_{P \in P_H} x_{P'}(P)) = O(n^{2/3})$ by Claims \ref{claim_non_highway} and \ref{claim_xP'}.   
The computations described can be done for all paths $P'$ in layer $i$ in parallel, as the trees $T(P')$ are edge disjoint for such paths. 

\paragraph{There are edges between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$, and $x_{P'}(P) \leq x_{P}(P').$}
Here we would like to let $P$ compute the values $\cut(e',e)$ for $e' \in P', e \in P$. To explain the computation, we first fix $e' \in P'$ and take a closer look on $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e).$ We assume that $\cov(e')$ and $\cov(e)$ are already known to vertices in $P$ \yuval{why can we assume this?}, and focus on computing $\cov(e',e).$ For this, we use Claim \ref{cover_non_highway_highway} that shows that $\cov(e',e) = \cov_{F_P}(e',e)+\cov(e',P)$. In addition, by Claim \ref{claim_compare}, we know that it is enough to compare edges from $E_{P'}(P)$ to $P$.
Now, our strategy is as follows. We let all edges $e' \in P'$ that are in the set $E_{P'}(P)$ compute the values $\cov(e',P)$ and send them to $P$ using an edge between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$, note that this requires only one computation in $P'$ per highway $P$. Then, we let the vertices in $T(P)$ compute the values $\cov_{F_P} (e',e)$, which eventually allows each edge $e \in P$ learn the value $\cov(e',e)$ for all $e' \in E_{P'}(P).$ We next elaborate on these steps. 

Recall that $\cov(e',P)$ is the cost of edges that cover $e'$ and have an endpoint in $T(P^{\downarrow}) \setminus F_P$. Note that all such edges have an endpoint in the subtree rooted at $d_P$, the unique descendant of the fragment $F_P$. Hence, computing $\cov(e',P)$ to all edges $e' \in P'$ is equivalent to computing all the edges that cover $e'$ and the tree edge $\{d_P, p(d_P)\}$ between $d_P$ to its parent, excluding the edges with endpoint $d_P$. This computation can be done as in Claim \ref{claim_non_highway}, with one difference that we do not sum the cost of edges with endpoint $d_P.$ This requires one aggregate computation per highway $P$, and overall requires $O(n^{2/3} + n^{1/3})=O(n^{2/3})$ time if we consider all highways. 
Now we want to let all vertices in $T(P')$ learn the following information per edge $e' \in P'$: the value $\cov(e')$ and the values $\cov(e',P)$ for all highways $P \in P_H$ such that $e' \in E_{P'}(P)$. As $x_{P'}(P) = |E_{P'}(P)|$, the total information for all edges is $O(n^{2/3} + \sum_{P \in P_H} x_{P'}(P))=O(n^{2/3})$ by Claim \ref{claim_xP'} \mtodo{This part is the reason we needed the new algorithm and the partitioning of $P'$, I emphasize this as we will probably deal with such cases in other cases of the algorithm.}. Hence, we can use Claim \ref{claim_broadcast} to let all vertices in $T(P')$ learn it. Now we use an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$ to pass the information $\{e',\cov(e'),\cov(e',P)\}$ to $P$ for all $x_{P'}(P)$ edges in $P'$ that are in $E_{P'}(P)$ (note that as explained in the previous case, $f$ can check in one round if $x_{P'}(P) \leq x_{P}(P')$, and determine that we are in this case of the algorithm). The whole subtree $T(P) \cap F_P$ can then learn this information using upcast and broadcast in the fragment. 
We are in the case that the number $x_{P}(P')$ of edges in $P$ potentially interested in $P'$ satisfies $x_{P'}(P) \leq x_{P}(P')$. In addition, by Claim \ref{claim_xP}, $\sum_{P'} x_P(P') = O(n^{2/3})$, where we sum over all non-highways $P'$ of layer $i$.
Hence, the total cost of the upcast and broadcast required in $P$ for comparisons for all non-highway paths $P'$ in layer $i$ in this case is bounded by $O(n^{2/3}+\sum_{P'} x_{P'}(P))$=$O(n^{2/3} + \sum_{P'} x_{P}(P'))=O(n^{2/3}).$ Now, given the values $\{e',\cov(e'),\cov(e',P)\}$ we need one aggregate computation in $T(P)$ to compute $\cut(e',e)$ for all $e \in P.$ This holds since $\cov(e',e)=\cov(e')+\cov(e)-2\cov(e',e)$. The values $\cov(e),\cov(e')$ are known to $e$, and by Claim \ref{cover_non_highway_highway}, $\cov(e',e)=\cov(e',P)+\cov_{F_P}(e',e)$. The first term is already known, and the second can be computed using one aggregate computation in $T(P)$, where each vertex $v \in T(P^{\downarrow})$ learns about the total cost of edges that cover $e'$ and have one endpoint in $T(P^{\downarrow}) \cap F_P$ (the computation follows the one described in Claim \ref{claim_non_highway} for non-highways). Overall we need to do one such computation for $x_{P'}(P) \leq x_{P}(P')$ edges from $P'$. Summing over all possible $P'$ in layer $i$, we get a complexity of $O(n^{2/3} + \sum_{P'} x_{P'}(P)) = O(n^{2/3}),$ by Claim \ref{claim_xP}.

\paragraph{Conclusion.} 
We next explain how the computations described above allow to compute the min 2-respecting cut defined by two edges $e' \in P', e \in P$ such that $P'$ is a non-highway, $P$ is a highway, and $P'$ and $P$ are not in the same fragment and not in the same root to leaf path.
We have $O(\log{n})$ iterations, where in iteration $i$ we take care of paths $P'$ in layer $i$. Each such path is potentially interested in $O(\log{n})$ paths $P_H$ composed of highways that are not in the same root to leaf path, by Claim \ref{corol:-_layer_highway}. We described above the computation for $P'$ and one such path $P_H$ (this path may be composed of many highways $P$). Hence, for each path $P'$ we need to run the algorithm described above $O(\log{n})$ times for the different paths $P_H$. Also, as explained, all the computations can be done in parallel for all paths $P'$ in layer $i$ (this includes computations that are done in highways $P$, as explained in the relevant case). Hence, the overall complexity is $\tilde{O}(D + n^{2/3}).$ 

\remove{
\subsection{Both cut edges in highway}

\mtodo{this is only a very high-level sketch}

To deal with the highway-highway case, we would like to take highway paths $P'_H,P_H$ in layers $i$ and $j$ (each one of them now can be composed of many highways), explain how to do the computation for such pair, and how to simulate many such computations. We can still use the fact that any path of layer $i$ is only potentially interested in $O(\log{n})$ paths in layer at least $i$, not in the same root to leaf path. I think that something more general may hold, maybe this holds for any layers $i,j$ when we consider paths that are not in the same root to leaf path.

We basically need the following ingredients.
\begin{enumerate}
\item Partitioning of $P'_H$ and $P_H$ using the monotonicity.
\item Explain how we compute a min 2-respecting cut with one edge in $P'_H$ and one edge in $P_H.$
\item Explain how to run many such computations in parallel.
\end{enumerate} 

The first two basically extend the non-highway - highway case, but seem to be more involved. I next elaborate on these steps.

\subsubsection*{First part: partitioning}

\paragraph{Defining a partitioning.} Here the goal would be to decompose $P'_H,P_H$ to (almost) disjoint sub-segments of small diameter, and then it should be enough to focus on the sub-problems we get. 
We first need to show that we can get such partitioning satisfying the following: First, if we only solve the smaller sub-problems (where each sub-segment in $P'_H$ is only compared to some sub-segment in $P_H$), we still find the min 2-respecting cut for the original problem (something equivalent to Claim \ref{claim_compare}). Second, every edge in a highway $P' \in P'_H$ is only interested in average in $O(1)$ highways in $P_H$ and vice verse (something equivalent to Claim \ref{claim_xP'}).
More formally, if we denote by $x_{P'}(P)$ the number of edges in the highway $P' \in P'_H$ that we compare to the highway $P \in P_H$, then $\sum_{P} x_{P'}(P) = O(n^{2/3})$ (where $n^{2/3}$ is the diameter of $P'$), and the sum is over all highways $P$ such that we may compare $P'$ to $P$: if $P'$ is in a lower layer, we can just focus on the case that $P \in P_H$, as we only compare $P'_H$ to small number of highway paths of layer greater than $i$. However, we also need such property to hold in the reverse direction ($\sum_{P'} x_P(P') = O(n^{2/3})$) and here a path $P_H$ in a higher layer may be compared to many paths $P'_H$ in lower layers, so we need to bound the contribution of all highways $P'$ that we can compare to $P$ in all such computations (here, we can probably exploit the fact that each edge in $P$ is only interested in $O(1)$ root to leaf paths, and different paths $P'_H$ are in different such paths, see Claim \ref{claim_xP} for a proof for the simpler case that $P'$ is a non-highway.)
 
It seems that we need to use here monotonicity in both directions to obtain the second property described above (in the case of non-highway-highway we only broke the non-highway $P'$ to sub-segments, which is probably not enough here). I think there is probably more than one way to do it, one would be to start breaking $P_H$ to sub-segments (of arbitrary length) based on the fragments of $P'_H$. After this step, each highway $P' \in P'_H$ has a consecutive set of highways in $P_H$ we need to compare $P'$ to. We can let $P'$ do the computation for the first and last such highways, but as there may be many such highways, we don't want it to do the computation for all of them. The good feature here is that because of the monotonicity, for all fragments ``in the middle'', we only need to compare them to $P'$. For such pairs $P',P$, we would like to split the work between them similarly to what we did for non-highway-highway, but this would probably require to refine the partition further such that each edge in $P'$ is on average only interested in $O(1)$ such fragments $P$ (otherwise, $P'$ needs to send too much information for the different highways $P$, even if for some reason only highways $P \in P_H$ do all such computations, see the comment in the last case of the non-highway-highway case).
Also, note that there is some asymmetry here between $P'_H$ and $P_H$, the first is in a lower layer and only interested in $O(1)$ paths $P_H$ of layers above it. The second may be interested in many different paths $P'_H$ in layers below it. So it may affect the complexity of the algorithm if we start by breaking $P'_H$ to segments according to $P_H$ or vice verse (it seems that maybe it would be easier to parallelize  the computations if we start by breaking all paths $P'_H$ to segments according to $P_H$, but it is not really clear, we should probably take a look at several options before deciding). 

\paragraph{Implementation.} After proving the correctness of such partitioning, the next challenge is the implementation, and I think this currently seems like one of the main challenges if we want to get to $\sqrt{n}$ complexity (mostly since we need to run the algorithm for many pairs $P'_H,P_H$ in parallel). If we only deal with one pair of paths $P'_H,P_H$ maybe we can try to use some binary search, not to compute all the partitioning at once, but for example choose the middle fragment in $P_H$, take the first and last edges in the highway and find for them the best edges in $P'_H$, and then break the problem to smaller problems based on monotonicity (I don't really know if such approach can work, this is just an intuition). Since we want to run many such computations in parallel, this becomes more challenging. Currently the root to leaf case seems to me the most challenging, in particular trying to solve the following case: we have some layer $i$ path $P_H$ that many layer $j$ paths below it $(j \leq i)$ are interested in it, and $P_H$ should participate in some way in all the computations.

I next give some implementation idea if we don't try to get an optimal complexity (I think $n^{2/3}$ should probably work).
Basically, the main things we need to compute for the partitioning are computations like the following: we are given some edge $e' \in P'_H$ and we need to find for it the edge $e \in P_H$ such that $\cut(e',e)$ is minimal. Let $P' \in P'_H$ be the fragment of $e'$, and I'll focus on finding the best $e \in P$, where $P \in P_H$, we do this for all highways $P \in P_H.$ (During the algorithm, maybe we can restrict ourselves only to part of them - especially if we want to work in parallel in different disjoint problems, currently I just explain the general idea and assume we look at all highways $P \in P_H$.)
Again $\cut(e',e) = \cov(e)+\cov(e')-2\cov(e',e)$, and as usual the main challenge is to compute $\cov(e',e)$ ($e'$ is fixed so we can assume that $\cov(e')$ is known by all vertices, and $\cov(e)$ is known to $e$.). Since we deal with the highway-highway case, $\cov(e',e)$ is broken up to many different parts. 
\begin{enumerate}
\item Edges that cover entirely the highways $P$ and $P'$ (with endpoints outside their fragments): $\cov(P',P).$ 
\item Edges with endpoint in $F_{P'}$ that cover $e'$ and the whole highway $P$: $\cov(e',P).$
\item Edges with endpoint in $F_{P}$ that cover $e$ and the whole highway $P'$: $\cov(e,P').$
\item Edges that cover $e',e$ and have endpoints in both $F_P$ and $F_{P'}$ (the fragments of $P$ and $P'$): $\cov_{\ell}(e',e)$.
\end{enumerate}

$\cov(P',P)$ is global information, that all vertices can learn in $O(D+n^{2/3})$ time as this is a bound on the number of pairs of highways. \mtodo{If we want a better complexity, we need to bound better the number of highways we actually compare, and in particular have some partitioning that really allows to bound this number better.}
The second term is known by $e'$, the third is known by $e$ and the last can be computed either in $F_P$ or in $F_{P'}$ using an aggregate computation in the fragment. Here we assumed that $e$ wants to compute $\cut(e',e)$. For this it needs to receive $\cov(e'),\cov(e',P)$ from $e'$. This requires from the highway $P'$ one aggregate computation to compute the value $\cov(e',P)$ for all edges $e' \in P'$ per highway $P$. Since the partitioning algorithm only fixes $O(1)$ edges $e' \in P'$ each time, we can also allow to send through a BFS tree all the values $\cov(e',P)$ for $e'$ we are interested in (at most $O(1)$ per fragment), and all highways $P$. The number of information if bounded by $O(n^{2/3})$ (this again is too expensive if we want a better complexity). Now $e$ has all information needed, and using one aggregate computation in $F_P$ is can compute $\cut(e',e)$ for a fixed $e'$. For all possibly $O(n^{1/3})$ edges $e'$ we fix, we need $O(n^{1/3})$ such aggregate computations. Then, we can use convergecast in a BFS tree to find the best $e \in P_H$, such that $cut(e',e)$ is minimal (before we only computed the best edge in each fragment), and we can send everybody the final result as we only consider $O(1)$ edges per fragment. 

I think the algorithm described above can be used to partition for example $P_H$ to subsegments according to $P'_H$. This actually seems to compute all the partitioning at once without iterations, but this idea is quite expensive, if we want a better complexity we should refine it (we can try to work in a binary search fashion, that allows decomposing the problem into disjoint problems, and not do all the computations at once). This doesn't really give the exact partitioning we want, because we also should break $P'_H$ to subsegments according to $P_H$. After we decide what is exactly the partitioning that we want, I guess similar ideas can hopefully be used to construct it.   

\subsubsection*{Second part: Finding the min 2-respecting cut} 
Here the goal would be to extend ideas from the non-highway-highway case. However, the actual computations needed would be more complicated, and in particular $\cov(e',e)$ is now split to more edges. As discussed above, when we fix two highways $P',P$ and look for the min cut with $e' \in P', e \in P$, we have: $$\cov(e',e)=\cov(P',P)+\cov(e',P)+\cov(e,P')+\cov_{\ell}(e',e).$$
We divide into cases, one case is that there are no edges between the fragments of $P'$ and $P$. Hence, $\cov_{\ell}(e',e)=0$, also note that the expression $\cov(P',P)$ does not depend on the specific choice of $e'$ and $e$, the expression $\cov(e',P)$ does not depend on $e$, and the expression $\cov(e,P')$ does not depend on $e'$. Remember that our goal is to minimize the expression $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e)$. This can be broken to the part $\cov(e')-2\cov(e',P)$ that depends only on $e'$, to the part $\cov(e)-2\cov(e,P')$ that depends only on $e$, and to the part $\cov(P',P)$ that does not depend on any of them. Hence, to minimize the expression we just need to find $e' \in P'$ such that $\cov(e')-2\cov(e',P)$ is minimized, and $e \in P$ such that $\cov(e)-2\cov(e,P')$ is minimized. $e'$ can be found using an aggregate computation in $P'$, and $e$ can be found using an aggregate computation in $P$. Then, we can send the information found (the edge, and the value it computed) to all vertices using a BFS tree. This is only $O(1)$ information per pair of highways $P',P$. In general, for all such computations we need $O(D+n^{2/3})$ time, since $O(n^{2/3})$ is a bound on the number of pairs, this complexity also allows all vertices to learn the value $\cov(P',P)$ for all pairs (getting a better complexity, requires a better bound on the number of pairs we compare). 

We next discuss the case that there are edges between the fragments of $P'$ and $P$. Here, basically we want to extend the idea described in the last case of the non-highway-highway algorithm. We decide which one of $P',P$ is responsible for the computations depending on the values $x_{P'}(P),x_P(P')$ (the number of edges in $P'$ compared to the highway $P$, and vice verse). Remember that we want that the partitioning we have would give that $\sum_{P} x_{P'}(P) = O(n^{2/3})$ and vice verse. If $x_{P'}(P) \leq x_P(P')$, we have that $P$ is responsible for the computations, it means it should compute the values $\cov(e',e)$ for $e \in P$, and $e' \in P'$ from the $x_{P'}(P)$ edges compared to $P$. The computation is as follows. Basically to be able to do this computation, for any relevant edge $e'$, it should get the values $\cov(e'), \cov(e',P).$ As discussed in the implementation of the partitioning, the rest of information needed: $\cov(e),\cov(e,P'), \cov(P',P), \cov_{\ell}(e',e)$ is either already known to $e \in P$ or can be computed using one aggregate computation in $T(P).$ Let's analyze the computation required by $P'$ and by $P$ for this case. In $P'$ we should compute the values $\cov(e',P)$ for all $e' \in P'$, and all highways $P$. Letting each edge $e' \in P'$ learn the information relevant for it requires one aggregate computation per highway $P$. Now we want to let all vertices in $T(P')$ learn the values $\cov(e',P)$ for all edges $e'$ that we want to compare to $P$ (we have $x_{P'}(P)$ such edges). Overall, we want to collect $\sum_{P} x_{P'}(P)$ information, which is $O(n^{2/3})$ by the partitioning. Then, we send the information to $T(P)$, using an edge between $T(P')$ and $T(P)$. In $T(P)$, we now need one aggregate computation per each one of the $x_{P'}(P) \leq x_P(P')$ edges $e' \in P'$, to compute the values $\cut(e',e).$ Doing so for all highways $P'$ from this case would result in a complexity of $O(n^{2/3}+\sum_{P'} x_{P'}(P))=O(n^{2/3})$ by the partitioning properties. This completes the case that $x_{P'}(P) \leq x_P(P')$. The other case is symmetric, and now $P'$ does the computations.

\subsection{Other cases}

There are additional cases that are not discussed here at all, maybe the most significant is the case that the two edges are in the \textbf{same root to leaf path}. Maybe some ideas described here can be useful for this case as well, but it seems that there are also different challenges for this case. For example, if we fix some long path of layer $i$ and want to compute the min 2-respecting cut that has both edges in the path, we don't have a vertex $r$ such that we know that one edge is below it and one is above it, so we need to split to different cases and hope that we can work on some of these cases in parallel.

Another case is that the two edges are in the same fragment, this is not dealt yet in all cases, but should probably be fine.

\subsection{An algorithm for two sub-paths}

\mtodo{a different way to look at things, that can hopefully generalize most of the cases.}

During our algorithm, many times we consider two sub-paths $P',P$ of length $O(\dfrag)$, and find the min 2-respecting cut that has one edge in $P'$, and one edge in $P$. We start by describing how to compare two such sub-paths.

\mtodo{we also need to discuss the case that we have one path.}

\mtodo{explain somewhere what is an aggregate computation in a sub-tree.}

\begin{lemma} \label{lemma_paths}
Let $P_0,P_1$ be two disjoint paths between an ancestor to its descendant in the tree, and assume that there is an edge $f$ between $T(P^{\downarrow}_0) \cap F_{P_0}$ and $T(P^{\downarrow}_1) \cap F_{P_1}$. \mtodo{we should see if in the same root to leaf path case we need some different condition on $f$.}
We denote by $x_{P_0}(P_1)$ the number of edges in $P_0$ that we compare to $P_1$, and by $x_{P_1}(P_0)$ the number of edges in $P_1$ that we compare to $P_0$.
For $i \in \{0,1\}$, at the beginning of the computation, the following information is known by all vertices in $T(P_i) \cap F_{P_i}$: \mtodo{Maybe there is some asymmetry and it's enough that one side would know some of the information, we should see in the proof}
\begin{enumerate}
\item The identity of all the edges in $P_i$ that we compare to $P_{1-i}$.
\item For each edge $e \in P_i$ that we compare to $P_{1-i}$, the values $\cov(e),\cov(e,P_{1-i})$.
\item The value $\cov(P_0,P_1).$
\item The identity of the edge $f$.
\end{enumerate}
Assume that $x_{P_0}(P_1) \leq x_{P_1}(P_0)$, then in $O(x_{P_1}(P_0))$ aggregate computations in $T(P_1) \cap F_{P_1}$, each edge $e \in P_1$ that we compare to $P_0$ would know the values $\cut(e,e')$ for all edges $e' \in P_0$ that we compare to $P_1.$
\end{lemma}

Some crucial observations that allow to compare many pairs of paths in parallel are the following.
First, we can work in parallel in disjoint sub-trees.

\begin{claim}
Let $P,P'$ be two sub-paths such that $T(P) \cap F_P$ and $T(P') \cap F_{P'}$ are edge-disjoint, then we can run aggregate computation in $T(P) \cap F_P$ and $T(P') \cap F_{P'}$ in parallel.
\end{claim}

Second, we can pipeline aggregate computations in a sub-tree.

\begin{claim} \label{claim_pipeline}
Assume that the path $P$ participates in the algorithms $A_1,A_2,...,A_k$, and in algorithm $A_i$ we run $x_i$ aggregate computations in $T(P) \cap F_P$, then running all the computations takes $O(\dfrag + \sum_{i=1}^{k} x_i)$ time.
\end{claim}

From Claim \ref{claim_pipeline}, to get a small time complexity we need to bound the value $\sum_{i=1}^{k} x_i$.
We next discuss that case that there is no edge between $P_0$ and $P_1.$

\begin{lemma} 
Let $P_0,P_1$ be two disjoint paths between an ancestor to its descendant in the tree, and assume that there is no edge between $T(P^{\downarrow}_0) \cap F_{P_0}$ and $T(P^{\downarrow}_1) \cap F_{P_1}$. \mtodo{we should see if in the same root to leaf path case we need some different condition on $f$.}
Then, given the values $\cov(P_0,P_1)$, as well as the values $\cov(e),\cov(e,P_0)$ for an edge $e \in P_1$ such that $\cov(e)-2\cov(e,P_0)$ is minimal, using one aggregate computation in $T(P_0) \cap F_{P_0}$, all vertices in $T(P_0) \cap F_{P_0}$ learn the values $e',e, \cut(e',e)$ for edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal.
\end{lemma}
}



==> 9-other.tex <==
Old definitions and terms we no longer need.


\begin{definition}\label{def:-downarrow}
For some vertex $v$ in a rooted spanning tree $T$ of $G$, we denote by $\dw{v}$ the subtree of $T$ rooted at $v$.
\end{definition}






We recall the definitions of \textit{interesting paths} from \TODO{Ref our paper}.


\begin{definition}[Cross-\interest edge] \label{def:cross-int-vertex}
Given an edge $e \in T$, we denote an edge $e' \in T$ ($e \bot e'$) to be cross-\interest with respect to $e$ if $C(u^\da, v^\da) > \frac{\deg(u^\da)} 2$ where $e$ is the parent edge of $u$ and $e'$ is the parent edge of $v$.
\end{definition}



\begin{definition}[\Interest path] \label{def:interest-path}
Given an edge $e$, we denote a path $P \in T$ to be cross-\interest (or down-\interest) with respect to $e$ if there is an edge $e' \in P$ such that $e'$ is cross-\interest (or down-\interest) with respect to $e$. The set of interesting paths w.r.t. $e$ is denoted by $\interesting(e)$. Given two paths $P_1$ and $P_2$, we denote $P_1$ to be cross-\interest (or down-\interest) w.r.t. $P_2$ is there is an edge $e$ in $P_2$ such that $P_1$ is cross-\interest (or down-\interest) w.r.t. $e$. The set of interesting paths w.r.t. a path $P$ is denoted by $\interesting(P)$.
\end{definition}




\begin{observation}\label{obs:int-ancestor}
Given an edge $e$, if an edge $e'$ is cross-\interest w.r.t $e$, then all ancestors of $e'$ are \interest w.r.t $e$. Similarly, if an edge $e''$ is down-\interest w.r.t. $e$, then all ancestors of $e''$ (up to but not including $e$) are down-\interest w.r.t $e$.
\end{observation}


\begin{definition}[Down-\interest edge] \label{def:down-int-vertex}
Given an edge $e$, we denote an edge $e' \in u^\da$ to be down-\interest with respect to $e$ if $C(v^\da, V - u^\da) > \frac{\deg(u^\da)} 2$ where $e$ is the parent edge of $u$ and $e'$ is the parent edge of $v$.
\end{definition}




\begin{observation} \label{obs:int-vbotv}
Given an edge $e$, there cannot be two edges $e'$ and $e''$ such that $e' \bot e''$ and both $e'$ and $e''$ are cross-\interest or down-\interest with respect to $e$.\yuval{Do we define somewhere the orthogonal notation?}
\end{observation}




\yuval{Move old definitions to other.}
\begin{itemize}
    \item \textbf{Cross-\interest.} $C(u^\da, v^\da)$ and $C(u^\da, v'^\da)$ are disjoint for $e' \bot e''$, and hence $\deg(u^\da) \leq C(u^\da, v^\da) + C(u^\da, v'^\da)$. If both $v$ and $v'$ are \interest with respect to $u$, then $C(u^\da, v^\da) + C(u^\da, v'^\da) > \deg(u^\da)$ which is a contradiction. 
    \item \textbf{Down-\interest.} $C(v^\da, V - u^\da)$ and $C(v'^\da, V - u^\da)$ are disjoint for $e' \bot e''$ as well, and hence a similar argument goes through.
\end{itemize}


==> bound-pot-interesting.tex <==
\section{Proof of Lemma \ref{lemma:-cover_all_or_nothing_paths}} \label{sec:bound-pot-interesting}

Consider a path $P=(e_1,...,e_z)$ , and let $P'\in \intpot{P}$ be some path such that $P'\in \cP$, and that $e_z$ is potentially interested in. Here, $e_z$ is the last edge in the path $P$(ordering by distance to the root from smallest to highest). Let $e'$ be the lowest edge in $P'$ that $e_z$ is potentially interested in.

Since $e_z$ is interested in $e'$, we can deduce that $\cov(e_z)<\alpha \cov(e_z,e')$. Now consider some edge $e_j,\ j<z$, s.t. $e_j=(x_j,y_j)$ is potentially interested in some path $P''\in \cP$ s.t. $P''\neq P'$(i.e. these paths are not on the same root to leaf path).
Now, the key observation here, is that by the described property of $\cP$,  we have that $\ECov(e',e_z)\subseteq \ECov(e_j)$, this is since all edges in $\ECov(e',e_z)$ cover $e_z$, so by the property they must cover all of $e_1,...,e_z$, in particular $e_j$, since $j< z$.
Thus it must hold that $\ECov(e_z,e')\subseteq \ECov(e_j)$. 
\paragraph{}
Now, since $e_j$ is  potentially interested in $P''$, let $e''=(x'',y'')\in P''$ be the last edge in $P''$ edge that $e_j$ is potentially interested in. 
Thus, we have that $\cov(e_j)<\alpha \cov(e_j,e'')$. 

An important observation is that the following claim holds, whose proof we defer to the end of the lemma. 
\begin{claim}\label{claim:-lemma_help_claim}
$\ECov(e_z,e'),\ECov(e_j,e'')$ are disjoint. 
\end{claim}
%This is true since the sets of edges $\ECov(e'),\ECov(e'')$ are disjoint, this is true since the paths $P'$ and $P''$ are on different root to leaf paths and the edges $e',e''$ are the last edges on these paths respectively. 
Now, from the fact that \[\ECov(e_z,e')\cup \ECov(e_j,e'')\subseteq \ECov(e_j),\]
we deduce that 
\[
\cov(e_z,e')+\cov(e_j,e'')\leq \cov(e_j)
\]
combining this with $\cov(e_j)<\alpha \cov(e_j,e'')$, we can deduce that $\frac{\cov(e_z,e')}{\alpha -1}<\cov(e_j,e'')$.
\paragraph{}
Now, assume that for some edge $e_k=(x_k,y_k),k<j$, it is potentially interested in a path $P'''\in \cP$ s.t. $P'''\neq P''$ and $P'''\neq P'$(i.e. these paths are not on the same root to leaf path). Denote by $e'''=(x''',y''')$ the last edge in $P'''$ that $e_k$ is potentially interested in. Thus, it holds that $\cov(e_k)<\alpha \cov(e_k,e''')$. 
\paragraph{}
Now, we employ claim \ref{claim:-lemma_help_claim} in the same manner as before to deduce that the sets $$\ECov(e_z,e'),\ECov(e_j,e''),\ECov(e_k,e''')$$ are pairwise disjoint.
%this similarly holds since no two of $P',P'',P'''$ are  on the same root to leaf path and that $e',e'',e'''$ are the last edges in these paths respectively. Thus $\ECov(e'),\ECov(e''),\ECov(e''')$ are pairwise disjoint. 

We employ one more time the property of $\cP$ to deduce that $\ECov(e_z,e')\cup \ECov(e_j,e'')$ is contained in $\ECov(e_k)$, since all edges in $\ECov(e_z,e')\cup \ECov(e_j,e'')$ must cover the edges $e_1,...,e_j$ as well by the property of $\cP$. In particular, all edges in $\ECov(e_z,e')\cup \ECov(e_j,e'')$ cover $e_k$, since $k<j$.

Combining this with the previous observation regarding the disjointness of the edge sets, we deduce that 
\[
\cov(e_z,e')+\cov(e_j,e'')+\cov(e_k,e'')\leq \cov(e_k)
\]


Combining this with $\cov(e_k)<\alpha \cov(e_k,e''')$, we can deduce that
\[\cov(e_z,e')+\cov(e_j,e'')<(\alpha -1)\cov(e_k,e''').\]
Now, combining this with $\frac{\cov(e_z,e')}{\alpha -1}<\cov(e_j,e'')$, we deduce that 
\[
\cov(e_z,e')\left (\frac{1}{\alpha -1}+\frac{1}{(\alpha -1)^2}\right )<\cov(e_k,e''').
\]

\paragraph{}

To generalize this, one can prove the following claim.
\begin{claim}\label{claim:-blowupclaim}
 Given an increasing(i.e. the higher the index, the closer to the root) sequence of edges from $P$, $w_1=(u_1,v_1),...,w_\ell=(u_\ell,v_\ell)$, s.t. $\ell\geq 2$ and each $w_i$ is potentially interested in an ancestor to descendant path $P_i\in \cP$ and an edge $e_i$ in that path, which is not on the same root to leaf path as any of $P_1,...,P_{i-1}$. Then it holds that:
\[
\cov(w_1,e_1)\cdot \sum\limits_{j=1}^{\ell-1} \frac{{\ell-2 \choose j-1}}{(\alpha -1)^j}<\cov(w_\ell,e_\ell)
\]

\end{claim}



\begin{proof}
One can prove this by induction on $\ell$, the base case is $\ell=2$, which we proved, we also proved the case of $\ell=3$. Now assume correctness for some $\ell$ and we prove correctness for $\ell+1$. By the same arguments as for the case of $\ell=2,3$, and claim \ref{claim:-lemma_help_claim}, we can deduce that
\[
\cov(w_{\ell+1})>\sum\limits_{j=1}^{\ell+1} \cov(w_j,e_j).
\]

From here, we use the induction assumption and that $\cov(w_{\ell+1})<\alpha \cov(w_{\ell+1},e_{\ell+1})$ to deduce that
\begin{gather*}
(\alpha-1)\cov(w_{\ell+1},e_{\ell+1})>\cov(w_1,e_1)\left(
1+ \sum\limits_{k=2}^{\ell} \sum\limits_{j=1}^{k-1}\frac{{k-2\choose j-1}}{(\alpha -1)^{j}} \right)\\
=\cov(w_1,e_1)\left(
1+ \sum\limits_{j=1}^{\ell-1} \sum\limits_{k=j+1}^{\ell}\frac{{k-2\choose j-1}}{(\alpha -1)^{j}} \right)=\cov(w_1,e_1)\left(
1+ \sum\limits_{j=1}^{\ell-1} \frac{{\ell-1\choose j}}{(\alpha -1)^{j}} \right)
\end{gather*}


The second transition is due to change of summation order, summing first on the powers in the denominator.

Dividing by $\alpha -1$, we get that
\begin{gather*}
    \cov(w_{\ell+1},e_{\ell+1})>\cov(w_1,e_1)\cdot \left(\frac{1}{\alpha -1}+\sum\limits_{j=1}^{\ell-1} \frac{{\ell-1\choose j}}{(\alpha -1)^{j+1}} \right)\\
    =\cov(w_1,e_1)\cdot \sum\limits_{j=0}^{\ell-1} \frac{{\ell-1\choose j}}{(\alpha -1)^{j+1}}= \cov(w_1,e_1)\cdot \sum\limits_{j=1}^{\ell-1} \frac{{\ell-1\choose j-1}}{(\alpha -1)^{j}}
\end{gather*}
as required. This concludes the proof.

Now, we employ the fact that for all $\ell\geq 2$, it holds that 
\[
\sum\limits_{j=1}^{\ell-1} \frac{{\ell-2 \choose j-1}}{(\alpha -1)^j}=\frac{\alpha^{\ell-2}}{(\alpha-1)^{\ell-1}}
\]

We desire to show that for $\alpha =O(1)$, it suffices that $\ell=O(1)$ to have a constant $c>1$ factor blowup in the value of $\cov(w_{\ell+1},e_{\ell+1})$ compared to $\cov(w_{1},e_{1})$. For this we demand that $\frac{\alpha^{\ell-2}}{(\alpha-1)^{\ell-1}}>1$. This happens iff $\left(\frac{\alpha }{\alpha -1}\right)^{\ell-1}>\alpha$, which in turn, occurs iff $\ell>\log _{\frac{\alpha }{\alpha -1}}(\alpha )+1$. The latter expression is $O(1)$ since $\alpha =O(1)$, thus it suffices that $\ell=O(1)$. 
\end{proof}
We now turn back to show that constant factor blowup every $\ell=O(1)$ edges can not occur. Thus arriving at at contradiction.
\paragraph{}
Now, assume that $|\set{P'\in \cP| P'\in \intpot{P}}|=\omega (\log ^2 n)$, each edge $w$ in $P$ is potentially interested in  $O(1)$ paths, and in particular at most $O(1)$ paths from $\cP$. Thus, by the pigeon hole principal, there are $m(n)=\omega(\log ^2 n)$ edges in $P$ that are potentially interested in a path from $\cP$.
Denote by $w_i$ the $i$-th edge in $P$ that is potentially interested in a path from $\cP$, where enumeration begins at the lowest edge. 
\paragraph{}
Define $\covs(i)$ to equal one if $|\set{P'\in \intpot{w_i}\cap \cP|\forall 1\leq k<i, P'\not\in \intpot{w_k}}|\geq 1$, and 0 otherwise. Less formally, we set $\covs(i)$ to be $0$ if $w_i$ introduces no new paths to the set $\intpot{P}$, compared to the previous edges considered. Otherwise, we set $\covs(i)$ to $1$.
\paragraph{}
Note that in order to get a contradiction, it suffices to show that $\sum\limits_{w_i\in P} ch(i)>\ell\log ^2 n$. This in turn, will show by claim \ref{claim:-blowupclaim} that if we look at the first edge $w_j$ in $P$ s.t. $\covs(j)=1$ and the $(\ell\log ^2 n)$-th edge $w_k$ in $P$ s.t. $\covs(k)=1$, then 
\[
c^{\log ^2 n}\cdot \cov(w_j,e_j)<\cov(w_k,e_k).
\]
Here, $e_j,e_k$ are the corresponding edges in paths $P_j,P_k$ that triggered $\covs(j)=ch(k)=1$, that $w_j,w_k$ are potentially interested in, respectively.

Since $\log ^2 n=\omega(\log n)$, we would arrive at the conclusion that $\cov(w_k,e_k)$ has super-polynomial weight, which is a contradiction. 

Now, we prove that $\sum\limits_{w_i\in P} ch(i)>\ell\log ^2 n$.

assume towards a contradiction that $\sum\limits_{w_i\in P} ch(i)\leq \ell\log ^2 n$. A key observation is that if $\covs(i)=0$ for some edge $w_i$, then by definition of $\covs(i)$ we get that  
\[\set{P'\in \cP|P'\in \bigcup\limits_{j=1}^{i-1} \intpot{w_i}\cap \cP}=\set{P'\in \cP|P'\in \bigcup\limits_{j=1}^i \intpot{w_i}\cap \cP}\]
 Combining this observation with the fact that each edge $w_i\in P$ is potentially interested in $O(1)$ paths in total, thus in particular it is potentially interested in $O(1)$ paths from $\cP$, we can deduce that
\[
|\bigcup\limits_{w_i\in P} \intpot{w_i}\cap \cP|=O(\sum\limits_{w_i\in P} ch(i))=O(\ell \log ^2 n)=O(\log ^2 n)
\]

Which is a contradiction to our assumption that $|\set{P'\in \cP| P'\in \intpot{P}}|=\omega (\log ^2 n)$.

%divide these edge into $z(n)=\frac{m(n)}{\ell\log ^2 n}=\omega(\log n)$ blocks of $\ell\log ^2n $ edges each in the following way. The first block $b_1$ is the $\ell \log ^2 n$ lowest edges. Now we define the block $b_{i+1}$ assuming we defined $b_i$. Denote by $e$ the highest edge of $b_i$, then $e\in b_{i+1}$ and the next $\ell \log ^2 n-1$ consecutive edges in $P$ which are interested in a path from $\cP$ which are higher than $e$ are in $b_{i+1}$. Now we look at a block $b_i$, denote the highest and lowest edges in this block by $e_i^{low},e_i^{high}$.

%We aim to prove that there are $\ell$ edges $e$ in $b_i$ s.t. each of these edges is interested in a different path $P_e\in \cP$. If such set of $\ell$ edges exist, one can assume w.l.o.g that it includes $e_i^{low},e_i^{high}$. This is proved in claim \ref{claim:-help_claim_lemma}. Thus, we will be able to deduce from claim \ref{claim:-blowupclaim} that $c\cdot Cov(w_{{e_i}^{low}},e_i^{low})< Cov(w_{{e_i}^{high}},e_i^{high})$. Here, $w_{{e_i}^{low}},w_{{e_i}^{high}}$ are the corresponding edges in $P_{{e_i}^{low}}, P_{e_i^{high}}$ that ${e_i}^{low},e_i^{high}$ are interested in, respectively. Thus, combining over all block we would get that $c^{z(n)}\cdot Cov(w_{{e_1}^{low}},e_1^{low})<Cov(w_{{e_{z(n)}}^{high}},e_{z(n)}^{high})$. Since $z(n)=\omega(\log n)$, we would arrive at the conclusion that $\cov(w_{{e_{z(n)}}^{high}},e_{z(n)}^{high})$ has super polynomial weight, which is a contradiction.


%\begin{claim}\label{claim:-help_claim_lemma}
%In each block $b_i$, there are $\ell$ edges $e$ s.t. each one of these edges is potentially interested in a different path $P_e\in \cP$.
%\end{claim}
%\begin{proof}
%Define $e^i_j$ the $j$-th edge in the block $b_i$, where the enumeration starts at the lowest edge with $j=1$. denote by $\covs(i,j)$ the value $|\set{P\in \intpot{e^i_j}\cap \cP|\forall 1\leq k<j, P\not\in \intpot{e^i_k}}|$. I.e., the number of paths from $\cP$ that $e^i_j$ is potentially interested in that none of the previous edges in $b_i$ were potentially interested in.
%\end{proof}
\paragraph{}

All that is left to conclude the proof of the lemma is to prove claim \ref{claim:-lemma_help_claim}.
\begin{proof}[Proof of claim \ref{claim:-lemma_help_claim}]
 \mtodo{what happened here? Is the next paragraph a proof of the claim?}
\end{proof}
Assume towards a contradiction that $\ECov(e_z,e'),\ECov(e_j,e'')$ are not disjoint. That means that there exists a non tree edge $e=(w_1,w_2)$ such that $e\in \ECov(e_z,e_j,e',e'')$. We know that $e',e'',e_j$ are on different root to leaf paths, thus $\dw{e'}, \dw{e''},\dw{e_j}$ are pairwise disjoint. Note therefore, that since $e\in \ECov(e')$, it must hold that w.l.o.g $w_1\in \dw{e'}$, this holds since all edges that cover $e'$ are crossing the cut defined by $\dw{e'}$. Similarly, one can deduce that $w_2\in \dw{e''}$. However, one can also deduce by the same reasoning that either $w_1$ or $w_2$ is $\dw{e_j}$. This contradicts the fact that $\dw{e'}, \dw{e''},\dw{e_j}$ are pairwise disjoint. This completes the proof.


==> intro-Daga_et_al.tex <==
%%%!TEX root = main_Min-Cut_latex.tex
%!TEX root = camera_ready.tex
\section{Introduction\label{sec:intro}}

%\thatchaphol{Our sparse $k$-edge connectivity certificate algorithm is the first $\tilde{O}(m)$ work and $\tilde{O}(1)$ depth algorithms for general $k$. I tried look up the literature and it seems all previous works need $\Omega(mk)$ work. (e.g. https://www.sciencedirect.com/science/article/pii/S0196677400911441) 


Edge connectivity is a fundamental graph-theoretic concept measuring the minimum number of edges to be removed to disconnect a graph $G$. We give a new algorithm for computing this measure in the \CONGEST model of distributed networks.
In this model a network is represented by an unweighted, undirected, connected $n$-node graph $G=(V, E)$.
Nodes represent processors with unique IDs and infinite computational power that initially only know their incident edges. 
%
They can communicate with each other in {\em rounds}, where in each round each node can send a message of size $O(\log n)$ to each neighbor. 
%
The goal is for nodes to finish some tasks together in the smallest number of rounds, called {\em time complexity}.
%\footnote{This problem is sometimes referred to as {\em name-independent routing schemes}. See, e.g. \cite{LenzenP_stoc13,LenzenP-podc15}  for discussions and results on another variant called {\em name-dependent routing schemes} which is not considered in this paper.}   
%
%It is usually expressed in terms of $n$ and $D$, where $n$ is the numer of nodes and $\diam$ is the diameter of the network when edge weights are omitted. Throughout we use $\tilde \Theta$, $\tilde O$ and $\tilde \Omega$ to hide polylogarithmic factors in $n$. See \Cref{sec:prelim} for details of the model.
%
The time complexity is usually expressed in terms of $n$ and $D$, the number of nodes and the diameter of the network. Throughout we use $\tilde \Theta$, $\tilde O$ and $\tilde \Omega$ to hide polylogarithmic factors in $n$. (See \Cref{sec:prelim} for details of the model.)

There are two natural objectives for computing a network's edge connectivity. The first is to make every node knows the edge connectivity of the network, denoted by $\lambda$. 
%Another objective is for each node to learn which of its incident edges are in the {\em minimum cut} (in short, {\em mincut}), referring to the set of $\lambda$ edges whose removals disconnect the graph.
The second is to learn about a set $C$ of $\lambda$ edges whose removals disconnect the graph, typically called a {\em mincut}. In this case, it is required that every node knows which of its incident edges are in $C$.\footnote{Readers who are new to distributed computing may wonder whether it is also natural to have a third objective where every node is required to know about {\em all} edges in the mincut. This can be done fairly quickly after we achieve the second objective, i.e. in $O(\min(\lambda,\sqrt{n\lambda})+D)$ rounds \cite{Censor-HillelGK14-decomposition}. 
For this reason, we do not consider this objective here.}
% It is easy to argue that this requires $\Omega(\lambda+D)$ time. Moreover, this can be achieved in $O(\lambda+D)$ time after we achieve the second objective. So, we do not discuss this third objective in the paper.} 
%
Since our results and other results hold for both objectives, we do not distinguish them in the discussion below.

It is typically desired that distributed algorithms run in {\em sublinear time}, meaning that they take $\tilde O(n^{1-\epsilon}+D)$ time for some constant $\epsilon>0$.\footnote{An exception is when a linear-time lower bound can be proved, e.g. for all-pairs shortest paths and diameter (e.g. \cite{BernsteinN19,HuangNS17,Elkin-STOC17,LenzenP_podc13,HolzerW12,FrischknechtHW12,PelegRT12,AbboudCK16}).}. 
%Starting from the dist of Garay, Kutten, and Peleg
%
Such algorithms have been achieved for many problems in the literature, such as minimum spanning tree, single-source shortest paths, and maximum flow \cite{Elkin-STOC17,GhaffariL18,ForsterN18,Censor-HillelGK14-decomposition,BeckerKKL16,Nanongkai-STOC14,NanongkaiS14,GhaffariK13,GhaffariKKLP15,KuttenP98,GarayKP98}. In the context of edge connectivity, the first sublinear-time algorithm, due to Thurimella \cite{Thurimella95}, was for finding if $\lambda=1$ (i.e. finding a {\em cut edge}) and takes $O(\sqrt{n}\log^* n + D)$ time. This running time was improved to $O(D)$ by Pritchard and Thurimella \cite{PritchardT11}, who also presented an algorithm with the same running time for $\lambda=2$ (i.e. they can find a so-called {\em cut pair}). More recently, by adapting Thorup's tree packing \cite{Thorup07}, Nanongkai and Su \cite{NanongkaiS14} presented a $O((\sqrt{n}\log^* n + D)\lambda^4)$-time algorithm, achieving sublinear time for any $\lambda=n^{1/8-\epsilon}$. 

%By random sampling, this algorithm can also be easily extended to a $O((\sqrt{n}\log^* n + D)\epsilon^{-5}\log^3(n))$-time algorithms that can  $(1+\epsilon)$-approximate $\lambda$, for any $\lambda$, as well as the minimum-weight cut, giving an improvement over the previous approximation algorithms by Ghaffari and Kuhn \cite{GhaffariK13}. 

To compute $\lambda$ when $\lambda\geq n^{1/8}$, we are only aware of {\em approximation algorithms}. The state-of-the-art is the $O((\sqrt{n}\log^* n + D)\epsilon^{-5}\log^3(n))$-time $(1+\epsilon)$-approximation algorithm of Nanongkai and Su \cite{NanongkaiS14}, which is an improvement over the previous approximation algorithms by Ghaffari and Kuhn \cite{GhaffariK13}. In fact,  both algorithms can approximate the minimum-weight cut, and the running time of $O((\sqrt{n}\log^* n + D)\epsilon^{-5}\log^3(n))$ matches a lower bound of \cite{DasSarmaHKKNPPW12} up to polylogarithmic factors; this lower bound holds even for $\poly(n)$-approximation algorithms and on unweighted graphs \cite{GhaffariK13} (also see  \cite{ElkinKNP14,KorKP13,Elkin06,PelegR00}).

% (it was also later extended to unweighted graphs \cite{GhaffariK13}). In other words, no significantly better approximation algorithm exists. 

%A more dramatic improvement was made when {\em approximate solutions} are allowed: 
% *** \danupon{I omitted the detailed discussions for lower bounds (commented below) since they are not really relevant.} ***
%
%On the negative side, it was known that $\tilde \Omega(\sqrt{n})$ time is needed even to approximate the minimum-weight cut on unweighted multigraphs on a $O(\log n)$-diameter network, due to  Ghaffari and Kuhn \cite{GhaffariK13} (extending from the lower bound for weighted graphs from \cite{DasSarmaHKKNPPW12}).\footnote{In our distributed setting, unweighted multigraphs are different from weighted graphs in that a multi-edge allows more communication while the edge weights do not affect communication.} This lower bound holds even when a fairly large approximation ratio is allowed. 
%%
%In simple graphs, \cite{GhaffariK13} showed that any $\alpha$-approximation algorithm requires $\tilde \Omega(\sqrt{\frac{n}{\alpha\lambda}})$ time on a $\tilde O(\frac{1}{\lambda}\cdot \sqrt{\frac{n}{\alpha\lambda}})$-diameter network.  

Given that approximating edge connectivity is well-understood, a big open problem that remains is whether we can compute $\lambda$ {\em exactly}. This question in fact reflects a bigger issue in the field of distributed graph algorithms: While there are plenty of sublinear-time {\em approximation} algorithms, many of which are tight, very few sublinear-time {\em exact} algorithms are known. This is the case for, e.g., minimum cut, maximum flow, and maximum matching (e.g. \cite{HenzingerKN-STOC16,BeckerKKL16,Nanongkai-STOC14,NanongkaiS14,GhaffariK13,GhaffariKKLP15,AhmadiKO18-matching}). 
To the best of our knowledge, the only exceptions  are the classic exact algorithms for minimum spanning tree \cite{GarayKP98,KuttenP98} and very recent results on exact single-source and all-pairs shortest paths \cite{Elkin-STOC17,GhaffariL18,ForsterN18,BernsteinN19,HuangNS17}. A fundamental question here is whether other problems also admit sublinear-time exact algorithm, and to what extent such algorithms can be efficient. 
\paragraph{Our Contributions.} 
We present the first sublinear-time algorithm that can compute  $\lambda$ {\em exactly} for any $\lambda$. Our algorithm works on simple graphs, i.e. when the network contains no multi-edge.
\begin{thm}\label{thm:main}
There is a distributed algorithm that, after \sloppy $\tilde O(n^{1-1/353}D^{1/353}+n^{1-1/706})$ time, w.h.p. (i) every node knows the network's edge connectivity $\lambda$, and (ii) there is a cut $C$ of size $\lambda$ such that every node knows which of its incident edges are in $C$.\footnote{We say that an event holds with high probability (w.h.p.) if it holds with probability at least $1-1/n^\epsilon$, where $\epsilon$ is an arbitrarily large constant.}
\end{thm}
As a byproduct of our technique, we also obtain a $O(n \text{ polylog}n)$-round algorithm for computing exact minimum cut in \emph{weighted} graphs (see \Cref{thm:min_cut_o_n_general_graph}).

To achieve \Cref{thm:main}, we develop and combine several new techniques from both distributed and static settings. First, note that we can also assume that we know the approximate value of $\lambda$ from \cite{NanongkaiS14,GhaffariK13}.
%
More importantly, the previous algorithm of \cite{NanongkaiS14} can already compute $\lambda$ in sublinear time when $\lambda$ is small; so, we can focus on the case where $\lambda$ is large here (say $\lambda=\Omega(n^{c})$ for some constant $c>0$). 
%
Our algorithm for this case is influenced by the static connectivity algorithm of Kawarabayashi and Thorup (KT) \cite{kawarabayashi2015deterministic}, but we have to make many detours. The idea is as follows. In \cite{kawarabayashi2015deterministic}, it is shown that if a {\em simple} graph $G=(V, E)$ of minimum degree $\delta$ has edge connectivity strictly less than $\delta$, then there is a near-linear-time static algorithm that partitions nodes in $G$ into  $\tilde O(n/\delta)$ many clusters in such a way that no mincut separates a cluster; i.e. for any mincut $C\subseteq E$, every edge in $C$ must have two end-vertices in different clusters. Once this is found, we can apply a fast static algorithm on a graph where each cluster is contracted into one node.
%a new graph $H$ with$ nodes and $\tilde O(m/\delta)$ edges. 
%
Since in our case $\delta\geq \lambda=\Omega(n^{\epsilon})$, the KT algorithm gives hope that we can partition our network into  $\tilde O(n/\delta)=\tilde O(n^{1-\epsilon})$ clusters. Then we maybe able to design a distributed algorithm that takes time near-linear in the number of clusters. There are however several obstacles:
\begin{enumerate}[label=(\roman*)]
	\item \label{item:sparse_cert} The KT algorithm requires to start from a {\em $\lambda$-edge connectivity certificate}, i.e. a subgraph of $O(n\lambda)$ edges with connectivity $\lambda$. However, existing distributed algorithms can compute this only for $\lambda=o(\sqrt{n})$. 
	\item \label{item:sequential} The KT algorithm is highly sequential. For example, it alternatively applies the contraction and trimming steps to the graph several times. 
	%it consists of a sequence of decomposition and contraction steps of the graph. 
	\item \label{item:mincut_contracted} Even if we can get the desired clustering, it is not clear how to compute $\lambda$ in time linear in the number of clusters. In fact, there is even no 
%\mohit{\textbf{some issue with the sentence structure, perhaps this should be good: there does not exist even an}} 
$\tilde O(n)$-time algorithm for computing $\lambda$. 
\end{enumerate}

For the first obstacle, the previous algorithm for computing a $\lambda$-edge connectivity certificate is by Thurimella \cite{Thurimella95}. It takes $O((\sqrt{n}\log^*n+D)\lambda)$, which is too slow when $\lambda$ is large. To get around this obstacle, we design a new distributed algorithm that can compute a $\lambda$-edge connectivity certificate in $\tilde O(\sqrt{n\lambda}+D)$ time. 
%
The algorithm is fairly intuitive: We randomly partition edges into $c=\lambda/\polylog(n)$ groups. Then we compute an $O(\polylog(n))$-edge connectivity certificate for each group {\em simultaneously}. This is doable in $\tilde O(\sqrt{nc}+D)$ time by fine-tuning parameters of Kutten-Peleg's minimum spanning tree algorithm \cite{KuttenP98} and using the scheduling of \cite{ghaffari2015near}, as discussed in \cite{ghaffari2015near}. 

This algorithm also leads to the first parallel algorithm for computing a $2$-edge connectivity certificate with polylogarithmic depth and near-linear work. To the best of our knowledge, previous near-linear work algorithms are essentially sequential and previous polylogarithmic-depth algorithms require $\Omega(mk)$ work in the worst case (e.g. \cite{KargerM97}). 

For the second obstacle, we first observe that the complex sequential
algorithm for finding clusters in the KT algorithm can be significantly
simplified into a few-step algorithm, if we have a black-box algorithm called
\emph{expander decomposition}. Expander decomposition was introduced
by Kannan et al. \cite{KannanVV00} and is proven to be useful for
devising many fast algorithms \cite{SpielmanT04,OrecchiaV11,OrecchiaSV12,KelnerLOS14,CohenKPPRSV17,ChuGPSSW18}
and also dynamic algorithms \cite{NanongkaiS16,NanongkaiSW17,Wulff-Nilsen16a}. 
%
With this algorithm, we do not need most of the KT algorithm, except some simple procedures called trimming and shaving, which can be done locally at each node. More importantly, we can avoid the long sequence of contraction and trimming steps (we need to apply these steps only once). 
%More importantly, we can avoid the long sequence of contraction, decomposition, shaving, and trimming steps (we need the shaving and trimming steps only once). 
%
Unfortunately, there is no efficient distributed algorithm for computing the expander decomposition.\footnote{It would be possible to obtain this using the balanced sparse cut  algorithm claimed by Kuhn and Molla \cite{KuhnM15}, but as noted in \cite{chang2018distributed}, the claim is incorrect. We thank Fabian Kuhn for clarifying this issue. After our paper is announced, an efficient distributed algorithm for computing balanced sparse cut is correctly shown in \cite{ChangS19}.} However, we can slightly adjust a very recent algorithm by Chang~et~al.~\cite{chang2018distributed} to obtain a weaker variant of the expander decomposition, which is enough for us.
%to achieved something close enough. 
%We can adjust their algorithm to get a decomposition that we need.  


For the third obstacle, our main insight is the observation that the clusters obtained from the KT algorithm (even after our modification) has {\em low average diameter} ($O(n^c)$ for some small constant $c$). Intuitively, if every cluster has small diameter, then we can run an algorithm on a smaller network where we pretend that each cluster is a node. The fact that clusters have lower average degree is not as good, but it is good enough for our purpose: we can adjust Karger's near-linear-time algorithm \cite{karger2000minimum} to compute $\lambda$ in time near-linear in the number of clusters. 

%To this end, we note that running the algorithm without the clust

%we first observe that we can compute $\lambda$ in $\tilde O(n)$ time by adjusting Karger's near-linear-time algorithm \cite{karger2000minimum}. 
 

\endinput





%
Second, we show that by combining the recent  distributed expander decomposition technique of [Chang, Pettie, Zhang, SODA'19] with some techniques from the sequential deterministic edge connectivity algorithm of [Kawarabayashi, Thorup, STOC'15], we can decompose the network into sublinear number of clusters with {\em small average diameter} and without any mincut separating a cluster (except the ``trivial'' ones). This leads to a simplification of Kawarabayashi-Thorup framework (except that we are randomized while they are deterministic). This might make this framework more useful in other models of computation. 
%
Finally, by extending the tree  packing technique from [Karger STOC'96], we can find the minimum cut in time proportional to the number of components.


% it was known from \cite{DasSarmaHKKNPPW12} that $\tilde \Omega(\sqrt{n}+D)$ time is needed even to approximate the minimum-weight cut. 

\danupon{TO DO: Say that we didn't try to optimize exponent. Note that lower bound for simple graph is not tight. }
\danupon{CITE: Mohsen's congested clique mincut}






\endinput




We present the first sublinear-time algorithm that can compute edge connectivity $\lambda$ {\em exactly} on distributed message-passing networks (the CONGEST model), as long as the network contains no multi-edge. Our algorithm takes $\tilde O(n^{1-1/41}D^{1/41})$ time to compute $\lambda$ and a cut of cardinality $\lambda$ with high probability, where $n$ and $D$ are the number of nodes and the diameter of the network, respectively, and $\tilde O$ hides polylogarithmic factors. This running time is sublinear in $n$ (i.e. $\tilde O(n^{1-\epsilon})$) whenever $D$ is. 
%
Previous sublinear-time distributed algorithms can do this either (i) exactly only when $\lambda=o(n^{1/8})$ [Thurimella PODC'95; Pritchard, Thurimella, ACM Trans. Algorithms'11; Nanongkai, Su, DISC'14], and (ii)  approximately [Ghaffari, Kuhn, DISC'13; Nanongkai, Su, DISC'14].\footnote{Note that the algorithms of [Ghaffari, Kuhn, DISC'13] and [Nanongkai, Su, DISC'14] can in fact approximate the minimum-weight cut.} 

To achieve this, we develop and combine several new techniques.
First, we design the first distributed algorithm that can compute a {\em $k$-sparse certificate} for any $k=O(n^{1-\epsilon})$; its time is $\tilde O(\sqrt{nk}+D)$. The previous sublinear-time algorithm can do so only when $k=o(\sqrt{n})$ [Thurimella PODC'95]. 
\danupon{The running time in actually $\tilde O(\sqrt{nk}+D)$ but this is not stated yet.}
%Our algorithm takes $\tilde O(\sqrt{nk}+D)$ time, whic
In fact, our algorithm can be turned into the first parallel algorithm with polylogarithmic depth and near-linear work. Previous near-linear work algorithms are essentially sequential and previous polylogarithmic-depth algorithms require $\Omega(mk)$ work in the worst case (e.g. [Karger, Motwani, STOC'93]). 
\danupon{The theorem is not stated or proven.}
%
Second, we show that by combining the recent  distributed expander decomposition technique of [Chang, Pettie, Zhang, SODA'19] with some techniques from the sequential deterministic edge connectivity algorithm of [Kawarabayashi, Thorup, STOC'15], we can decompose the network into sublinear number of clusters with {\em small average diameter} and without any mincut separating a cluster (except the ``trivial'' ones). This leads to a simplification of Kawarabayashi-Thorup framework (except that we are randomized while they are deterministic). This might make this framework more useful in other models of computation. 
%
Finally, by extending the tree  packing technique from [Karger STOC'96], we can find the minimum cut in time proportional to the number of components.
%	
%	- sublinear component when graph has high min-degree
%	
%	- connectivity certificate in sublinear time ... Thurimella can only do for small $\lambda$. Side: PRAM polylogarithmic depth (indep of $\lambda$), near-linear work. Previously near-linear work algorithms require depth depending on $\lambda$. [Cheriyan, Thurimella, STOC'91]
%	
%	- Thorup is pretty sequential  (also Henzinger...) ... Also conceptually simpler 
%	



Computing fundamental graph properties on distributed message-passing networks (the CONGEST model) have been actively studied in the last decade, leading to many near-optimal approximation algorithms for many problems, such as shortest paths, minimum cut, and maximum flow. When it comes to {\em exact} algorithms, however, not much is known except a few very recent shortest paths algorithms. Edge connectivity
% -- the minimum number of edges whose deletion disconnects the network -- 
is among basic problems facing this situation. 
%
Its first non-trivial approximation algorithms were found  in 2013 by Ghaffari and Kuhn \cite{GhaffariK13}, 
%from 2013 [Ghaffari, Kuhn, DISC'13], 
and were later improved by the $(1+\epsilon)$-approximation $\tilde O((\sqrt{n}\log^* n+D)\epsilon^{-5}\log^{3} n)$-time algorithm of Nanongkai and Su \cite{NanongkaiS14}; here, $n$ and $D$ are the number of nodes and the diameter of the network and $\tilde O$ hides polylogarithmic factors.
%
The latter algorithm is essentially tight due to the lower bounds from \cite{DasSarmaHKKNPPW12,GhaffariK13}.\footnote{All mentined algorithms \cite{GhaffariK13,NanongkaiS14}


==> old_2respecting.tex <==
\section{Finding the min 2-respecting cut}

\mtodo{I think this whole part can be removed for now. Just left it here in case somebody needs it.}

We will next explain how to find the 2 tree edges $e,e'$ that define the minimum cut, we will focus first on the case that $e,e'$ are not in the same root to leaf path. We will divide to cases depending if the edges $e,e'$ are part of a highway or a non-highway.
We need the following definitions and claims.

%\begin{claim} \label{claim_layer}
%Each path in layer $i$ is potentially interested in $O(\log{n})$ paths from layer $j \geq i$.
%\end{claim}














\begin{claim} \label{claim_interested}
In ... time, all edges can learn about $O(\log{n})$ paths they are potentially interested in, that include all the paths they are interested in. \mtodo{what is the exact information they learn about the paths? We should add a clear explanations somewhere and also explain how this information is used in the algorithm.}
\end{claim}

\remove{
\begin{claim} \label{claim_edge}
If $P$ and $P'$ are two paths between an ancestor to a descendant, not in the same root to leaf path, and $P'$ is potentially interested in $P$, then there is an edge between $T(P^{\downarrow})$ and $T(P'^{\downarrow}).$
\end{claim} 

\mtodo{add proof.}
}

\begin{claim}[\sagnik{New}] \label{claim_edge_nonortho}
If $P$ and $P'$ are two paths between an ancestor to a descendant in the same root to leaf path where $P'$ occurs further from the root than $P$, and $P'$ is potentially interested in $P$. Also assume that the deepest node of $P$ is $d_P$. Then there is an edge between $T - T(d_P^{\downarrow})$ and $T(P'^{\downarrow}).$
\end{claim}

\mtodo{I'm not sure about the notation $d_P$ in the above claim, because it's confusing with $d_P$ which is used as the descendant of the highway $P$. Also, we should add a proof.}

\subsection{Algorithm description}

The algorithm works in $L^2 = O(\log^2{n})$ iterations, where each iteration corresponds to two indexes $1 \leq i \leq j \leq L$. In iteration $(i,j)$ we take care of min 2-respecting cuts with one edge in layer $i$ and one edge in layer $j$. We next focus on one such iteration. We assume that at beginning of the computation, each edge $e$ knows $\cov(e)$, which can be obtained in $\tilde{O}(D+\sqrt{n})$ rounds by Claim \ref{claim_learn_cov}. 

At this point, we also assume that the graph is decomposed into fragments \textit{viz.}~Claim \sagnik{Refer to appropriate claim. What will the vertices know?} We will view the juxtaposition of the layering decomposition and the fragment decomposition on $T$ by using the following definition: By a \textit{non-highway path in layer $i$}, we denote the sub-path of a non-highway path (obtained by the fragment decomposition) which is completely contained in layer $i$ (obtained by the layering decomposition). \sagnik{Do we do the same for highway?}

Formally, before the beginning of the algorithm, each vertex $v$ of $G$ will know the following information: \begin{enumerate}
    \item For each edge $e \in T$ incident on $v$, the cover value of $e$, $\cov(e)$ (\textit{viz.}~Claim \ref{claim_learn_cov}),
    \item For each edge $e$ incident on $v$, the index of the layer $i$ such that $e \in E_i$ obtained from the layering decomposition (\textit{viz.}~Property \ref{clmitem:info_vertex} of Claim \ref{claim:-layerDecomp}),
    \item For each edge $e$ incident on $v$, the index of the fragment that $e$ is in, and whether $e$ is a part of the highway or a non-highway of that fragment (\textit{viz.}~Claim \ref{clm:time-fragment}).
\end{enumerate}

Next we describe three parts of the algorithm which happen in parallel. In the first part, the goal is to inform every vertex the minimum cut value $\min \cut(e,e')$ where $e$ and $e'$ both occur in non-highways. In the second part, one of $e$ and $e'$ occur in a highway, and the third part deals with the case where both $e$ and $e'$ occur in highways.

\subsection{Both cut edges in non-highway}

In this section, we prove the following lemma.

\begin{lemma} \label{lem:main_nh-nh}[\yuval{check correctness, checked, seems ok to me for the orthogonal case}]
In time $O(D + \dfrag \log^3 n)$ each vertex $v$ of $G$ will know 
two edges $e', e$ such that $(e',e) = \arg \min_{\{e', e\}} \cut(e',e)$, as well as the value $\cut(e',e),$ where $e'$ and $e$ are edges in a pair of (orthogonal) non-highway paths.
\end{lemma}

\mtodo{In the above lemma I think we also want to learn the edges (I've added this), so we can infer the actual cut. Also, why is the word orthogonal in brackets?}


As stated above, there are $L^2$ many iterations, each of which can be identified with an unordered pair $(i,j)$ where $1 \leq i \leq j \leq L$. In iteration $(i,j)$ we look at all the non-highway paths $P'$ of layer $i$ and compare them to non-highway paths $P$ of layer $j$. We also assume that $P'$ and $P$ are not in the same root to leaf path. Note that all paths in the same layer are not in the same root to leaf path. In addition, by Claims \ref{claim:-layerDecomp} and \ref{claim_interested}, each path from layer $i$ is potentially interested only in $O(\log{n})$ paths from layer $j \geq i$, and all the edges of the path already know the paths they are potentially interested in. \mtodo{what is the exact information they know?}

We next fix a path $P'$ from layer $i$ and a path $P$ in layer $j$ that $P'$ is potentially interested in. Our goal is to find two edges $e' \in P', e \in P$ such that $(e',e) = \arg \min_{\{e' \in P', e \in P\}} \cut(e',e)$, as well as the value $\cut(e',e).$ For this, we show that each edge $e' \in P'$, can learn all the values $\{\cut(e',e)\}_{e \in P}$. All edges learn this simultaneously in a time that is proportional to the diameter of fragments. \mtodo{I currently work with $O(n^{1/3})$ fragments of diameter $O(n^{2/3})$, the numbers should be updated later.}

For proving \Cref{lem:main_nh-nh}, we need the following claims. The first claim states, informally, that it is efficient to broadcast information inside all non-highway paths in the same layer. 

\begin{claim} \label{claim_broadcast}
Fix a layer $j$, and assume that for each non-highway path $P$ in layer $j$ there are $k$ pieces of information of size $O(\log{n})$ where initially each one of them is known by some vertex in $T(P)$. In $O(\dfrag + k)$ rounds, all the vertices in $T(P)$ can learn all the $k$ pieces of information. In addition, this computation can be done in all non-highway paths $P$ in layer $j$ in parallel.
\end{claim}

\begin{proof}
Note that since $P$ is a non-highway path, the entire subtree $T(P)$ is in the fragment of $P$ and has diameter $\dfrag$.
To solve the task, we use pipelined upcast and broadcast in the subtree $T(P)$. First, we collect all $k$ pieces of information in the root $r_P$, and then broadcast them to the whole tree $T(P)$, using pipelining this takes $O(\dfrag + k)$ rounds.  Additionally, as the different trees $T(P)$ of paths $P$ in layer $j$ are edge disjoint by Claim \ref{claim_disjoint}, the computation can be done in parallel for all non-highway paths in layer $j$.  
\end{proof}

The next claim provides sufficient condition for efficient computation of 2-respecting cut values when the pair of constrained edges reside in different non-highway paths. Note that this claim does not assume anything about the orthogonality of these two paths.

\begin{claim} %\label{claim_non_highway}
Let $P'$ be a non-highway path, and assume the following:\begin{itemize}
    \item Let $\{e_i,\cov(e_i)\}_{i=1}^{k}$ be a collection of $k$ tuples that are known to all vertices in $T(P')$,
    \item None of the edges $\set{e_i}_{i \in [k]}$ occur in $T(P')$. \mtodo{Note this property when proving the case of two edges in the same root to leaf path. It seems important which edge does the computation there.}
\end{itemize} Then, in $O(\dfrag+k)$ rounds, each edge $e' \in P'$ can compute all the values $\{e_i,\cut(e',e_i)\}_{i=1}^{k}.$ In addition, for different paths $P'$ that are not in the same root to leaf path, these computations can be done in parallel.
\end{claim}

\begin{proof}
Let $e' \in P'$, and fix an edge $e \in \{e_i\}_{i=1}^k$. By Claim \ref{claim_cover}, $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e)$. Also, $e'$ knows $\cov(e)$ and $\cov(e')$, hence to compute $\cut(e',e)$, $e'$ should compute $\cov(e',e).$ As any edge that covers a tree edge $e'=\{v',p(v')\}$ where $p(v')$ is the parent of $v'$, has one endpoint in the subtree of $v'$, it follows that the edges that cover $e'$ and $e$ are exactly all the edges that cover $e$ and have one endpoint in the subtree of $v'$. This subtree is contained in $T(P')$.
Hence, to learn about the total cost of these edges we need to do one aggregate computation in $T(P')$: letting each vertex $v' \in T(P'^{\downarrow})$ learn about the total cost of edges incident on the subtree of $v'$ that cover $e$. This can be done using a convergecast in $T(P')$, where each vertex sends to its parent the total cost of edges in its subtree that cover $e$, this includes the sum of costs of edges it receives from its children and the cost of such edges adjacent to it. To implement this efficiently we need an efficient way to determine for each non-tree edge whether it covers a specific edge $e$, this can be done using Claim \ref{claim_LCA_labels}. Hence, when we fix an edge $e$, all the edges $e' \in P'$ can compute $\cut(e',e)$ using one convergecast in the subtree of $P'$. To do so for all $k$ edges in $\{e_i\}_{i=1}^k$, we run $k$ such computations in $T(P')$, using pipelining the complexity of all the computations is $O(\dfrag+k)$. At the end, each edge $e' \in P'$ knows the values $\cut(e',e)$ for all edges $e \in \{e_i\}_{i=1}^k.$ 

Since the whole computation was done in $T(P')$, the same computation can be done in parallel for other paths not in the same root to leaf path with $P'$.
\end{proof}

The following claim uses Claim \ref{claim_non_highway} to come up with a procedure to compute 2-respecting cut values where the constrained edges reside on two \textit{orthogonal} non-highway paths. \mtodo{I don't remember which is orthogonal, but you use this terminology both here and in the second case, in one of them it should be not orthogonal.}\yuval{Orthogonal is not the same root to leaf path}

\begin{lemma} \label{lemma_non_highway}
Let $P'$ be a non-highway path in layer $i$, and let $P$ be a non-highway path in layer $j \geq i$ such that $P'$ is potentially interested in $P$, and $P$ is not in the same root to leaf path with $P'$. In $O(\dfrag)$ rounds, each edge $e' \in P'$, learns all the values $\{e, \cut(e',e)\}_{e \in P}$.
\end{lemma}

\begin{proof}
First, we observe the following: 
\begin{itemize}
    \item[(i)] As $P'$ is potentially interested in $P$ there must be an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow})$ by Claim \ref{claim_edge} \mtodo{I think that this is the only place we use the fact that they are not in the same root to leaf path}.
    
    \item[(ii)] Since the trees $T(P^{\downarrow})$ are disjoint for paths in the same layer, the edge $f$ is different for different pairs $P',P$.
\end{itemize}
The goal is to use $f$ \mtodo{we should also explain how to decide about the edge $f$} to let all vertices of $P'$ learn about all the values $\{e,\cov(e)\}_{e \in P}$. Once this is done, using Claim \ref{claim_non_highway}, each edge $e' \in P'$ computes all the values $\{e, \cut(e',e)\}_{e \in P}$ in $O(n^{2/3})$ time. The rest of the proof is to show how the vertices of $P'$ know the required information to compute the cut values.

The procedure can be divided into three phases:
\begin{description}
\item[- Aggregation.] We use Claim \ref{claim_broadcast} to let all vertices in $T(P)$ learn all the values $\{e,\cov(e)\}_{e \in P}$. Note that at the beginning $\cov(e)$ is known to $e \in T(P)$, hence the condition of the claim holds. As $P$ is non-highway, this is $O(n^{2/3})$ information, hence this takes $O(n^{2/3})$ time. This computation is done in all non-highway paths in layer $j$ in parallel.

\item[- Tunnelling.] As $f$ has an endpoint in $T(P)$ and an endpoint in $T(P')$, in $O(n^{2/3})$ time all the information $\{e,\cov(e)\}_{e \in P}$ is also known by a vertex in $T(P')$.

\item[- Dissipation.] We can use Claim \ref{claim_broadcast} again to let all vertices in $T(P')$ learn this information.
\end{description}
To reiterate, after these three steps, each vertex can compute \mtodo{what happened to the end of the proof here?}
\end{proof} 

\begin{proof}[\sagnik{Proof of orthogonal case}] \mtodo{here again you use orthogonal}\yuval{should be not orthogonal here}
For the case when $P$ and $P'$ occur in the same root-to-leaf path, we are going to use the following structures:
\begin{itemize}
    \item[(i)] Note that there can be exactly 1 $P$ in layer $i$ that $P'$ in layer $j$ is (potentially) interested in. \yuval{why is this true? If $j\geq i$, how do you bound the number of paths of lower layer in the same root to leaf path that $j$ is interested in?}
    
    \item[(ii)] $P$ and $P'$ belong to the same fragment. Hence the path between $P$ and $P'$ is of length at most $\dfrag$.
    
    \item[(iii)] All $P'$ that $P$ is interested in share a common LCA which is the only intersection point of such $P'$s.
    
    \item[(iv)] The path between $P$ and the $P$'s that $P$ is interested in is unique for each $P$ in layer $i$.
\end{itemize}

\mtodo{I didn't understand why properties 3 and 4 hold. What happens if we have a path of layer $i$ that many different paths of layer $i-1$ attached to different vertices in it?}

So the procedure goes the following way:
\begin{itemize}
    \item As before, we first employ Claim \ref{claim_broadcast} to let every edge $v \in T(P)$ know the set $\{e, \cov(e)\}_{e \in P}$. This is $O(\dfrag)$-bits of information. We only need the vertex $d_P$ to know this information. \mtodo{again, $d_P$ is used for something else (unique descendant in a fragment) so maybe we can find a different notation.}
    
    \item We then want to let the top vertex of $P'$ know about this information using the path between $P$ and $P'$. To this end, $d_P$ pipelines this information to the LCA of all $P'$'s that $P$ is interested in. This can be done parallely for each $P$ in layer $i$ without any cross-congestion. \mtodo{I think we need a different argument here. The paths are not disjoint, but we want to learn the same information, so it's ok.}
    
    \item We then want to dissipate this information to every edge of $P'$ by again using Claim \ref{claim_broadcast}.
    
    \item Now we use Claim \ref{claim_non_highway} to let every edge $e' \in P'$ compute the set $\set{e, \cut(e, e')}_{e \in P}$. \yuval{the second condition of the claim \ref{claim_non_highway} does not hold though.}
\end{itemize}
\end{proof}

\begin{proof} [Proof of \Cref{lem:main_nh-nh}] We next explain how Lemma \ref{lemma_non_highway} allows to learn about the min 2-respecting cut that is defined by two tree edges in non-highways, not in the same root to leaf path. \Cref{alg:nh-nh} provides a schematic representation of the procedure.

\begin{center}
  \centering
  \begin{minipage}[H]{0.8\textwidth}
\begin{algorithm}[H]
\caption{Schematic algorithm when both edges are in non-highway}\label{alg:nh-nh}
\begin{algorithmic}[1]
\For{every pair $\set{i,j}$ from $L$, $i \leq j$}
    \For{Every non-highway $P'$ in layer $i$ and $P$ in layer $j$}
        \If{$P'$ is potentially interested in $P$}
            \State Each edge $e' \in P'$ computes $\set{e, \cut(e,e')}_{e \in P}$.
            \State $e'$ records $e \in P$ for which $\cut(e,e')$ is the minimum. 
            \Statex \Comment{\Cref{lemma_non_highway}}
        \EndIf
    \EndFor
\EndFor
\State Each edge $e$ performs convergecast along a BFS tree to send the minimum to the root.
\State Root performs downcast to let every vertex know the minimum.
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{center}

As explained above, we have $O(\log^2{n})$ iterations $(i,j)$, where in iteration $(i,j)$ we deal with non-highways in layer $i$ and $j$ for $i \leq j.$ In this iteration, we look at all non-highway paths $P'$ in layer $i$ and the non-highway paths $P$ in layer $j$ they are potentially interested in. Since each path in layer $i$ is potentially interested only in $O(\log{n})$ paths in layer $j$, we just need to apply the computation from Lemma \ref{lemma_non_highway}, $O(\log{n})$ times per path $P'$. In addition, it follows from the proof of Lemma \ref{lemma_non_highway} and Claims \ref{claim_broadcast} and \ref{claim_non_highway} that these computations can be done in parallel for different paths $P'$ in the same layer, as the trees $T(P')$ are edge disjoint for such paths. Summing up over all iterations we get a complexity of $O(\dfrag\log^3{n})$ rounds. At the end of the computation, for any two paths $P',P$ where $P'$ is in layer $i$ and is potentially interested in $P$ in layer $j$, each edge $e' \in P'$ knows the values $\{e, \cut(e',e)\}$ for all $e \in P.$ In particular, for any such 2-respecting cut, there is a vertex that knows about the 2 edges in the cut and the value of the cut. 
At the very end of the computation, we can use convergecast in a BFS tree to let all vertices learn the minimum 2-respecting cut and its value in $O(D)$ rounds. Overall, this sums up to a complexity of $O(D+\dfrag\log^3{n})$ rounds.
\end{proof} 



\subsection{Exactly one cut edge in highway}
\yuval{In all places that mention interested, should be changed to potentially interested+might need to change the $O(\log n)$ to some $polylog(n)$.}
\mtodo{Something we should add to all sections is how we distinguish between different cases: how do we know if we are in a highway/non-highway, orthogonal/non-orthogonal case, etc. In particular, we later break into cases according to whether there are edges between fragments or not, and if so we use a particular edge $f$, we need to explain how do we know in which case we are and how do we find the edge $f$.}

Here we compare non-highway paths $P'$ in layer $i$, to highway paths in layer $j$, where $i,j$ can be any indexes of layers. 
We will use Claim \ref{corol:-_layer_highway} that says that each non-highway path $P'$ is only interested in $O(\log{n})$ root to leaf paths composed of highways. However, note that such root to leaf path $P_H$ may be composed of many (possibly $O(\nfrag)$) different highways, hence just passing to $P'$ the information about all edges in the path $P_H$ can result in a linear complexity.
To get a sublinear complexity we use the following key ingredients. First, we use a certain monotonicity to break the path $P'$ to (almost) disjoint subpaths, each one of them is only interested in one highway in $P_H$.\yuval{Notation here needs to be improved and more formally defined.} Second, for different highways $P \in P_H$ that $P'$ is potentially interested in, we divide the computation between $P'$ and $P$ differently. If there is only small number of edges in $P$ that are interested in $P'$, we pass the relevant information to $P'$ and let $P'$ do the computation. If, on the other hand, many edges in $P$ are interested in $P'$, we let $P$ do the computation. Building on these ideas, we get a sublinear complexity. We next describe the algorithm in detail.

Fix a layer $i$, and a non-highway path $P'$ in layer $i$. As each edge in $P'$ knows about the paths it is potentially interested in and there are $O(\log{n})$ of them per edge, we can also let all vertices in $T(P')$ learn this information using Claim \ref{claim_broadcast} $O(\log{n})$ times, which takes $O(n^{2/3} \log{n})$ time. Using this information, all vertices in $P'$ can learn all the highway paths that $P'$ is potentially interested in. \mtodo{more details about the exact information known.} By Claim \ref{corol:-_layer_highway}, $P'$ is only potentially interested in $O(\log{n})$ root to leaf paths composed of highways. We next fix one such path $P_H.$ 
We focus on the case that $P'$ and $P_H$ are in different fragments, and not in the same root to leaf path.\mtodo{should handle somewhere other cases.}

For the algorithm, we first need to partition $P'$ into sub-segments. We start by describing the partition, and then show how we exploit it in the algorithm. 

\subsubsection*{First part: partitioning $P'$}

Let $P \in P_H$ be a highway. We denote by $e_P^{h},e_P^{\ell}$ the highest and lowest edges in the highway $P$, respectively. 
Define $P'(e_P^{h})$ to be an edge in $P'$ such that $\cut(P'(e_P^{h}),e_P^{h})$ is minimal. If there is more than one such edge, take the edge that is highest in $P'$. Define $P'(e_P^{\ell}) \in P'$ similarly with respect to $e_P^{\ell}$ (again, taking the highest possible edge if there is more than one option). First, we show that we can compute these edges efficiently.

\begin{claim}
In $O(D+n^{2/3})$ rounds, all vertices in $T(P')$ can learn the edges $P'(e_P^{h}), P'(e_P^{\ell})$ for all $P$. In addition, this computation can be done in all paths $P'$ in layer $i$ simultaneously.
\end{claim}

\begin{proof}
First, as there are $O(n^{1/3})$ highways, and we only consider two edges per highway, we can let all the vertices in the graph learn in $O(D+n^{1/3})$ rounds all the values $\{e,\cov(e)\}$ for $e$ that is equal to $e_P^{h}$ or $e_P^{\ell}$ for some highway $P$, using upcast and broadcast in a BFS tree. Then, we use Claim \ref{claim_non_highway}, to let all edges $e' \in P'$ to compute $\cut(e',e)$ for all relevant edges $e$. This requires $O(n^{1/3})$ aggregate computations in $T(P')$, and can be done in the same time for all paths $P'$ in layer $i$. Now per each edge $e$, we use convergecast and broadcast in $T(P')$ to let all vertices learn the highest edge $e'$ such that $\cut(e',e)$ is minimum. Using pipelining, this takes $O(n^{2/3}+n^{1/3})=O(n^{2/3})$ time for all edges. At the end, all vertices of $T(P')$ learn the edges $P'(e_P^{h}), P'(e_P^{\ell})$ for all $P$. As all the computations are done in $T(P')$, we can work in parallel in different paths $P'$ in the same layer.
\end{proof}

\sagnik{There must be a better nomenclature than $P'(e^h_P), E_{P'}(P)$, and $x_{P'}(P)$. We need to find those.}

After computing the minimal edges, we would like to use the monotonicity described in  \Cref{claim_monotonicity}, to divide $P'$ to (almost) disjoint sub-paths, and compare each one of them only to one highway $P \in P_H$. This is done as follows. 
We denote by $E_{P'}(P)$ all the edges in $P'$ between $P'(e_P^{\ell})$ and $P'(e_P^{h})$.
In our algorithm, the only edges in $P'$ that are compared to the highway $P$ are in $E_{P'}(P)$.
Note that all vertices in $T(P')$ know the edges $P'(e_P^{h}), P'(e_P^{\ell})$. We can also assume that all vertices in $T(P')$ know the complete structure of $P'$. This follows, since using pipelined upcast and broadcast, all edges in $T(P')$ can learn all the edges in $P'$ in $O(n^{2/3})$ time, as this is the length of $P'$. Based on this information, all edges in $P'$ know to which subsets $E_{P'}(P)$ each edge of $P'$ belongs, summarized as follows.

\begin{claim} \label{claim_know_Ep}
In $O(n^{2/3})$ time, all vertices in $T(P')$ learn the complete structure of $P'$, and the sets $E_{P'}(P).$ This computation can be done in all paths $P'$ in layer $i$ simultaneously.
\end{claim}
\yuval{proof of this claim needs to be more formal.}

We next show that it is indeed enough to compare only the subset $E_{P'}(P)$ to $P$, and then bound the total number of comparisons required by the algorithm.

\begin{claim} \label{claim_compare}
Assume that $(e',e) = \arg\min_{\{e' \in P', e \in P_H\}} \cut(e',e)$, then even if for any highway $P \in  P_H$, we only compare edges in $E_{P'}(P)$ to $P$, we learn about a min 2-respecting cut with value $\cut(e',e).$
\end{claim}
\yuval{A different wording? Maybe stating that the min value restricted only to the edges we are comparing equals the min value when we compare all pairs of edges.}

\begin{proof}
Let $P \in P_H$ be the highway such that $e \in P.$ If $e=e_P^h$ or $e=e_P^{\ell}$, we already computed an edge $e'' \in P'$ such that $\cut(e'',e)$ is minimal as needed. Otherwise, we use Claim \ref{claim_monotonicity} to show that there is an edge $e'' \in E_{P'}(P)$ such that $\cut(e'',e)$ is minimal. First, note that from Claim \ref{claim_monotonicity}, and since $e_P^{h}$ is above $e_P^{\ell}$, we have that $P'(e_P^{\ell})$ is either equal to $P'(e_P^{h})$ or below it. 
Next, we use Claim \ref{claim_monotonicity} on $e$ and $e_P^{h}$. Since $e_P^{h}$ is closer to the root compared to $e$, we have that the highest edge $e''$ such that $\cut(e'',e)$ is minimal is either $P'(e_P^h)$ or below it. Similarly, from using Claim \ref{claim_monotonicity} on $e$ and $e_P^{\ell}$ which is below $e$, we have that $e''$ is either equal to $P'(e_P^{\ell})$ or it is above it. To conclude, $e'' \in P'$ is between $P'(e_P^{\ell})$ to $P'(e_P^{h})$, hence by definition $e'' \in E_{P'}(P)$ as needed.
\end{proof}

We denote by $x_{P'}(P)$ the number of edges in $P'$ that we compare to the highway $P$. We next bound the number of comparisons required by the algorithm.

\begin{claim} \label{claim_xP'}
$\sum_{P \in P_H} x_{P'}(P) = O(n^{2/3}).$
\end{claim}

\begin{proof}
We have that $x_{P'}(P) = |E_{P'}(P)|$, we next use Claim \ref{claim_monotonicity} to show that the different sets $E_{P'}(P)$ are almost disjoint. The set $E_{P'}(P)$ includes all edges between $P'(e_P^{\ell})$ and $P'(e_P^{h})$. Also, as explained in the proof of Claim \ref{claim_compare}, the edge $P'(e_P^{\ell})$ is equal or below $P'(e_P^{h})$. For any edge $e' \in P'$ which is strictly above $P'(e_P^{\ell})$ and strictly below $P'(e_P^{h})$, we only compare it to $P$. The reason is as follows. From Claim \ref{claim_monotonicity}, for any edge $e \in P_H$ in a highway above $P$, the edge $e'' \in P'$ such that $\cut(e'',e)$ is minimal is $P'(e_P^{h})$ or above it. Similarly, for any edge $e \in P_H$ in a highway below $P$, the edge $e'' \in P'$ such that $\cut(e'',e)$ is minimal is $P'(e_P^{\ell})$ or below it. This means that for any highway $Q \neq P$, both the edges $P'(e_Q^{\ell}),P'(e_Q^{h})$ are either both above $e'$ or both below $e'$. This means that $e'$ is only in the set $E_{P'}(P)$. This means that the set $E_{P'}(P)$ includes $|E_{P'}(P)| - 2$ edges that are not in the set $E_{P'}(Q)$ for any $Q \neq P$ (assuming its size is at least 2), and the two edges $P'(e_P^{\ell}), P'(e_P^{h})$. If we sum over all sets, we get that $$\sum_{P \in P_H} x_{P'}(P) = \sum_{P \in P_H} |E_{P'}(P)| = O(n^{2/3} + n^{1/3}) = O(n^{2/3}).$$ The first term counts all the edges that are only in one set $E_{P'}(P)$, the number is bounded by the $O(n^{2/3})$ edges in $P'$. The second term counts the two edges $P'(e_P^{\ell}), P'(e_P^{h})$ per highway $P$. Here, an edge may be counted more than once, but per highway we only have two such edges, hence the total number is bounded by the number of highways, $O(n^{1/3}).$ This completes the proof.
\end{proof}

\subsubsection*{Second part: finding the min 2-respecting cut}

\sagnik{\begin{enumerate}
    \item The algorithm description needs to be enumerated/itemized.
    
    \item There needs to be a separate notation section.
    
    \item Need to spell out that $P$ in layer $j$, and $P'$ in layer $i \leq j$. \mtodo{the algorithm doesn't have this property, it may be the case that the highway has a lower layer.}
\end{enumerate}}

We next explain how we exploit the partition described above in our algorithm. 
We need the following definitions and claims.
Let $P'$ be a non-highway, and $P$ be a highway not in the same root to leaf path with $P'$. Let $e' \in P', e \in P$. We next take a closer look at the value $\cov(e',e).$ Any edge that covers $e'=\{v',p(v')\}$ and $e=\{v,p(v)\}$ has one endpoint in the subtree of $v'$ and one endpoint in the subtree of $v$. The first is contained in $T(P'^{\downarrow})$, which is contained in the fragment of $P'$, as $P'$ is a non-highway. The second is contained in $T(P^{\downarrow})$, however, since $v$ is on a highway, this subtree is not contained entirely in the fragment $F_P$ of $P$. The subtree of $v$ has one part in $T(P^{\downarrow}) \cap F_P$, and the other part in $T(P^{\downarrow}) \setminus F_P$, which is below the fragment $F_P$. 
We denote by $\cov_{F_P}(e',e)$ the cost of all the edges that cover $e'$ and $e$ and have one endpoint in $T(P^{\downarrow}) \cap F_P$, and by $\cov(e',P)$ the cost of all the edges that cover $e'$ and have one endpoint in $T(P^{\downarrow}) \setminus F_P$. Note that from the structure of the fragments any such edge covers $e'$ and the whole highway $P$, i.e., $\cov(e,e') = \cov_{F_P}(e',e) + \cov(e',P)$. This follows as any such edge has an endpoint in the subtree of the unique descendant $d_P$ of $F_P$, and all the vertices in the subtree of $d_P$ are in the subtrees of all the vertices in the highway $P$. Hence, this second term $\cov(e',P)$ does not depend on the specific choice of $e \in P.$ This is summarized as follows.

\begin{claim} \label{cover_non_highway_highway}
Let $e' \in P', e \in P$ where $P'$ is a non-highway, and $P$ is a highway not in the same root to leaf path with $P'$. Then $\cov(e',e) = \cov_{F_P}(e',e) + \cov(e',P)$, where $\cov_{F_P}(e',e)$ is the cost of all edges that cover $e'$ and $e$ and have one endpoint in the subtree $T(P^{\downarrow}) \cap F_P$, and $\cov(e',P)$ is the cost of all edges that cover $e'$ and have one endpoint in $T(P^{\downarrow}) \setminus F_P$.
\end{claim}

We denote by $x_P(P')$ the number of edges in the highway $P$ that are potentially interested in the non-highway path $P'$. Note that any edge in $P$ is only potentially interested in $O(\log ^3 n)$ paths not in the same root to leaf path \sagnik{Which claim to ref?} \mtodo{update the number if needed}. \yuval{Ill change the number again if needed.} Also, different non-highways in the same layer are not in the same root to leaf path, which means that any edge in $P$ is only potentially interested in $O(1)$ such non-highways. \yuval{why is this true?} As there are $O(n^{2/3})$ edges in $P$, this gives the following.

\begin{claim} \label{claim_xP}
$\sum_{P'} x_P(P') = O(n^{2/3})$, where we sum over all non-highways $P'$ of a fixed layer $i$.
\end{claim}


We now go over all highways $P \in P_H$ and find the min 2-respecting cut of $P'$ and $P$. We have several cases.

\paragraph{There are no edges between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$.}
Let $e' \in P', e \in P.$ From Claim \ref{claim_cover}, we have that $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e).$ 
In addition, from Claim \ref{cover_non_highway_highway}, we have that $\cov(e',e) = \cov_{F_P}(e',e)+\cov(e',P)$. Since any edge that covers $e'$ and $e$ has one endpoint in $T(P'^{\downarrow})$ and one endpoint in $T(P^{\downarrow})$, and there are no edges between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$, we have that $\cov_{F_P}(e',e) = 0$ in our case. This means that $\cov(e',e) = \cov(e',P)$ in our case, which is the cost of edges that cover $e'$ and have one endpoint in $T(P^{\downarrow}) \setminus F_P$. This means that the expression $\cov(e',e)$ does not depend on the specific choice of $e$ in $P$.
Hence, for any $e' \in P'$, the expression $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',P)$ is minimized for $e \in P$ such that $\cov(e)$ is minimal. Also, as this is only one edge $e$ per fragment we can let all vertices learn $e$ and $\cov(e)$ in $O(D+\nfrag)$ rounds using a communication in a BFS tree. Hence, we now only need to compute $\cut(e',e)$ for all $e' \in P',$ for $e \in P$ such that $\cov(e)$ is minimal. This requires one aggregate computation per edge $e$, and can be done for all such highways $P$ in $O(n^{2/3})$ rounds using Claim \ref{claim_non_highway}. Moreover, this is done for all paths $P'$ in layer $i$ simultaneously. 


\paragraph{There are edges between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$, and $x_P(P') \leq x_{P'}(P).$}
Here we let $P'$ compute the values $\cut(e',e)$ for $e' \in P', e \in P.$ For this, we use an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$ to pass to $P'$ the information $\{e,\cov(e)\}$ for all edges in $P$ that are potentially interested in $P'$. Then, we can use Claim \ref{claim_non_highway} to compute the values $\cov(e',e).$ We next describe the computation in detail. Note that since the trees $T(P'^{\downarrow})$ are disjoint for different paths $P'$ in the same layer, and the fragments $F_P$ are disjoint for different highways, the edge $f$ for different pairs $P',P$ is different.

First, as each edge in $P$ is only interested in $O(1)$ non-highway paths in layer $i$ \sagnik{Do we have a claim to ref?}, we can let all vertices of $F_P$ learn for each highway edge $e$ the value $\cov(e)$ and the non-highway paths of layer $i$ that $e$ is potentially interested in, using upcast and broadcast in the fragment $F_P$. This requires time proportional to the diameter of the fragment. In addition, from Claim \ref{claim_know_Ep}, all vertices in $T(P')$ can learn in $O(n^{2/3})$ time about all the values $x_{P'}(P)=|E_{P'}(P)|$, recall that this is the number of edges in $P'$ that we compare to $P$. Now, since $f$ has an endpoint in $T(P')$ and an endpoint in $F_P$, it has an endpoint that knows $x_{P'}(P)$, and an endpoint that knows $x_P(P')$, the number of edges in $P$ that are potentially interested in $P'$, and the values $\{e,\cov(e)\}$ for all such edges. In one round, $f$ can check if $x_P(P') \leq x_{P'}(P)$, and if this is the case it passes the information $\{e,\cov(e)\}$ to $T(P')$ for all $x_P(P')$ edges in $P$ potentially interested in $P'$, which takes $O(n^{2/3} + x_P(P'))=O(n^{2/3} + x_{P'}(P))$ time using Claim \ref{claim_broadcast}.
To do so for all paths $P \in P_H$ from this case simultaneously would result in a complexity of $O(n^{2/3} + \sum_{P \in P_H} x_{P'}(P)) = O(n^{2/3})$ rounds using Claims \ref{claim_broadcast} and \ref{claim_xP'}.
Now, we use Claim \ref{claim_non_highway} to let all edges $e' \in P'$ to compute the value $\cut(e',e)$ for each one of the at most $x_{P'}(P)$ edges of $P$ potentially interested in $P'$. Doing so for all highways $P \in P_H$ would result in a complexity of $O(n^{2/3} + \sum_{P \in P_H} x_{P'}(P)) = O(n^{2/3})$ by Claims \ref{claim_non_highway} and \ref{claim_xP'}.   
The computations described can be done for all paths $P'$ in layer $i$ in parallel, as the trees $T(P')$ are edge disjoint for such paths. 

\paragraph{There are edges between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$, and $x_{P'}(P) \leq x_{P}(P').$}
Here we would like to let $P$ compute the values $\cut(e',e)$ for $e' \in P', e \in P$. To explain the computation, we first fix $e' \in P'$ and take a closer look on $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e).$ We assume that $\cov(e')$ and $\cov(e)$ are already known to vertices in $P$ \yuval{why can we assume this?}, and focus on computing $\cov(e',e).$ For this, we use Claim \ref{cover_non_highway_highway} that shows that $\cov(e',e) = \cov_{F_P}(e',e)+\cov(e',P)$. In addition, by Claim \ref{claim_compare}, we know that it is enough to compare edges from $E_{P'}(P)$ to $P$.
Now, our strategy is as follows. We let all edges $e' \in P'$ that are in the set $E_{P'}(P)$ compute the values $\cov(e',P)$ and send them to $P$ using an edge between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$, note that this requires only one computation in $P'$ per highway $P$. Then, we let the vertices in $T(P)$ compute the values $\cov_{F_P} (e',e)$, which eventually allows each edge $e \in P$ learn the value $\cov(e',e)$ for all $e' \in E_{P'}(P).$ We next elaborate on these steps. 

Recall that $\cov(e',P)$ is the cost of edges that cover $e'$ and have an endpoint in $T(P^{\downarrow}) \setminus F_P$. Note that all such edges have an endpoint in the subtree rooted at $d_P$, the unique descendant of the fragment $F_P$. Hence, computing $\cov(e',P)$ to all edges $e' \in P'$ is equivalent to computing all the edges that cover $e'$ and the tree edge $\{d_P, p(d_P)\}$ between $d_P$ to its parent, excluding the edges with endpoint $d_P$. This computation can be done as in Claim \ref{claim_non_highway}, with one difference that we do not sum the cost of edges with endpoint $d_P.$ This requires one aggregate computation per highway $P$, and overall requires $O(n^{2/3} + n^{1/3})=O(n^{2/3})$ time if we consider all highways. 
Now we want to let all vertices in $T(P')$ learn the following information per edge $e' \in P'$: the value $\cov(e')$ and the values $\cov(e',P)$ for all highways $P \in P_H$ such that $e' \in E_{P'}(P)$. As $x_{P'}(P) = |E_{P'}(P)|$, the total information for all edges is $O(n^{2/3} + \sum_{P \in P_H} x_{P'}(P))=O(n^{2/3})$ by Claim \ref{claim_xP'} \mtodo{This part is the reason we needed the new algorithm and the partitioning of $P'$, I emphasize this as we will probably deal with such cases in other cases of the algorithm.}. Hence, we can use Claim \ref{claim_broadcast} to let all vertices in $T(P')$ learn it. Now we use an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow}) \cap F_P$ to pass the information $\{e',\cov(e'),\cov(e',P)\}$ to $P$ for all $x_{P'}(P)$ edges in $P'$ that are in $E_{P'}(P)$ (note that as explained in the previous case, $f$ can check in one round if $x_{P'}(P) \leq x_{P}(P')$, and determine that we are in this case of the algorithm). The whole subtree $T(P) \cap F_P$ can then learn this information using upcast and broadcast in the fragment. 
We are in the case that the number $x_{P}(P')$ of edges in $P$ potentially interested in $P'$ satisfies $x_{P'}(P) \leq x_{P}(P')$. In addition, by Claim \ref{claim_xP}, $\sum_{P'} x_P(P') = O(n^{2/3})$, where we sum over all non-highways $P'$ of layer $i$.
Hence, the total cost of the upcast and broadcast required in $P$ for comparisons for all non-highway paths $P'$ in layer $i$ in this case is bounded by $O(n^{2/3}+\sum_{P'} x_{P'}(P))$=$O(n^{2/3} + \sum_{P'} x_{P}(P'))=O(n^{2/3}).$ Now, given the values $\{e',\cov(e'),\cov(e',P)\}$ we need one aggregate computation in $T(P)$ to compute $\cut(e',e)$ for all $e \in P.$ This holds since $\cov(e',e)=\cov(e')+\cov(e)-2\cov(e',e)$. The values $\cov(e),\cov(e')$ are known to $e$, and by Claim \ref{cover_non_highway_highway}, $\cov(e',e)=\cov(e',P)+\cov_{F_P}(e',e)$. The first term is already known, and the second can be computed using one aggregate computation in $T(P)$, where each vertex $v \in T(P^{\downarrow})$ learns about the total cost of edges that cover $e'$ and have one endpoint in $T(P^{\downarrow}) \cap F_P$ (the computation follows the one described in Claim \ref{claim_non_highway} for non-highways). Overall we need to do one such computation for $x_{P'}(P) \leq x_{P}(P')$ edges from $P'$. Summing over all possible $P'$ in layer $i$, we get a complexity of $O(n^{2/3} + \sum_{P'} x_{P'}(P)) = O(n^{2/3}),$ by Claim \ref{claim_xP}.

\paragraph{Conclusion.} 
We next explain how the computations described above allow to compute the min 2-respecting cut defined by two edges $e' \in P', e \in P$ such that $P'$ is a non-highway, $P$ is a highway, and $P'$ and $P$ are not in the same fragment and not in the same root to leaf path.
We have $O(\log{n})$ iterations, where in iteration $i$ we take care of paths $P'$ in layer $i$. Each such path is potentially interested in $O(\log{n})$ paths $P_H$ composed of highways that are not in the same root to leaf path, by Claim \ref{corol:-_layer_highway}. We described above the computation for $P'$ and one such path $P_H$ (this path may be composed of many highways $P$). Hence, for each path $P'$ we need to run the algorithm described above $O(\log{n})$ times for the different paths $P_H$. Also, as explained, all the computations can be done in parallel for all paths $P'$ in layer $i$ (this includes computations that are done in highways $P$, as explained in the relevant case). Hence, the overall complexity is $\tilde{O}(D + n^{2/3}).$ 

\remove{
\subsection{Both cut edges in highway}

\mtodo{this is only a very high-level sketch}

To deal with the highway-highway case, we would like to take highway paths $P'_H,P_H$ in layers $i$ and $j$ (each one of them now can be composed of many highways), explain how to do the computation for such pair, and how to simulate many such computations. We can still use the fact that any path of layer $i$ is only potentially interested in $O(\log{n})$ paths in layer at least $i$, not in the same root to leaf path. I think that something more general may hold, maybe this holds for any layers $i,j$ when we consider paths that are not in the same root to leaf path.

We basically need the following ingredients.
\begin{enumerate}
\item Partitioning of $P'_H$ and $P_H$ using the monotonicity.
\item Explain how we compute a min 2-respecting cut with one edge in $P'_H$ and one edge in $P_H.$
\item Explain how to run many such computations in parallel.
\end{enumerate} 

The first two basically extend the non-highway - highway case, but seem to be more involved. I next elaborate on these steps.

\subsubsection*{First part: partitioning}

\paragraph{Defining a partitioning.} Here the goal would be to decompose $P'_H,P_H$ to (almost) disjoint sub-segments of small diameter, and then it should be enough to focus on the sub-problems we get. 
We first need to show that we can get such partitioning satisfying the following: First, if we only solve the smaller sub-problems (where each sub-segment in $P'_H$ is only compared to some sub-segment in $P_H$), we still find the min 2-respecting cut for the original problem (something equivalent to Claim \ref{claim_compare}). Second, every edge in a highway $P' \in P'_H$ is only interested in average in $O(1)$ highways in $P_H$ and vice verse (something equivalent to Claim \ref{claim_xP'}).
More formally, if we denote by $x_{P'}(P)$ the number of edges in the highway $P' \in P'_H$ that we compare to the highway $P \in P_H$, then $\sum_{P} x_{P'}(P) = O(n^{2/3})$ (where $n^{2/3}$ is the diameter of $P'$), and the sum is over all highways $P$ such that we may compare $P'$ to $P$: if $P'$ is in a lower layer, we can just focus on the case that $P \in P_H$, as we only compare $P'_H$ to small number of highway paths of layer greater than $i$. However, we also need such property to hold in the reverse direction ($\sum_{P'} x_P(P') = O(n^{2/3})$) and here a path $P_H$ in a higher layer may be compared to many paths $P'_H$ in lower layers, so we need to bound the contribution of all highways $P'$ that we can compare to $P$ in all such computations (here, we can probably exploit the fact that each edge in $P$ is only interested in $O(1)$ root to leaf paths, and different paths $P'_H$ are in different such paths, see Claim \ref{claim_xP} for a proof for the simpler case that $P'$ is a non-highway.)
 
It seems that we need to use here monotonicity in both directions to obtain the second property described above (in the case of non-highway-highway we only broke the non-highway $P'$ to sub-segments, which is probably not enough here). I think there is probably more than one way to do it, one would be to start breaking $P_H$ to sub-segments (of arbitrary length) based on the fragments of $P'_H$. After this step, each highway $P' \in P'_H$ has a consecutive set of highways in $P_H$ we need to compare $P'$ to. We can let $P'$ do the computation for the first and last such highways, but as there may be many such highways, we don't want it to do the computation for all of them. The good feature here is that because of the monotonicity, for all fragments ``in the middle'', we only need to compare them to $P'$. For such pairs $P',P$, we would like to split the work between them similarly to what we did for non-highway-highway, but this would probably require to refine the partition further such that each edge in $P'$ is on average only interested in $O(1)$ such fragments $P$ (otherwise, $P'$ needs to send too much information for the different highways $P$, even if for some reason only highways $P \in P_H$ do all such computations, see the comment in the last case of the non-highway-highway case).
Also, note that there is some asymmetry here between $P'_H$ and $P_H$, the first is in a lower layer and only interested in $O(1)$ paths $P_H$ of layers above it. The second may be interested in many different paths $P'_H$ in layers below it. So it may affect the complexity of the algorithm if we start by breaking $P'_H$ to segments according to $P_H$ or vice verse (it seems that maybe it would be easier to parallelize  the computations if we start by breaking all paths $P'_H$ to segments according to $P_H$, but it is not really clear, we should probably take a look at several options before deciding). 

\paragraph{Implementation.} After proving the correctness of such partitioning, the next challenge is the implementation, and I think this currently seems like one of the main challenges if we want to get to $\sqrt{n}$ complexity (mostly since we need to run the algorithm for many pairs $P'_H,P_H$ in parallel). If we only deal with one pair of paths $P'_H,P_H$ maybe we can try to use some binary search, not to compute all the partitioning at once, but for example choose the middle fragment in $P_H$, take the first and last edges in the highway and find for them the best edges in $P'_H$, and then break the problem to smaller problems based on monotonicity (I don't really know if such approach can work, this is just an intuition). Since we want to run many such computations in parallel, this becomes more challenging. Currently the root to leaf case seems to me the most challenging, in particular trying to solve the following case: we have some layer $i$ path $P_H$ that many layer $j$ paths below it $(j \leq i)$ are interested in it, and $P_H$ should participate in some way in all the computations.

I next give some implementation idea if we don't try to get an optimal complexity (I think $n^{2/3}$ should probably work).
Basically, the main things we need to compute for the partitioning are computations like the following: we are given some edge $e' \in P'_H$ and we need to find for it the edge $e \in P_H$ such that $\cut(e',e)$ is minimal. Let $P' \in P'_H$ be the fragment of $e'$, and I'll focus on finding the best $e \in P$, where $P \in P_H$, we do this for all highways $P \in P_H.$ (During the algorithm, maybe we can restrict ourselves only to part of them - especially if we want to work in parallel in different disjoint problems, currently I just explain the general idea and assume we look at all highways $P \in P_H$.)
Again $\cut(e',e) = \cov(e)+\cov(e')-2\cov(e',e)$, and as usual the main challenge is to compute $\cov(e',e)$ ($e'$ is fixed so we can assume that $\cov(e')$ is known by all vertices, and $\cov(e)$ is known to $e$.). Since we deal with the highway-highway case, $\cov(e',e)$ is broken up to many different parts. 
\begin{enumerate}
\item Edges that cover entirely the highways $P$ and $P'$ (with endpoints outside their fragments): $\cov(P',P).$ 
\item Edges with endpoint in $F_{P'}$ that cover $e'$ and the whole highway $P$: $\cov(e',P).$
\item Edges with endpoint in $F_{P}$ that cover $e$ and the whole highway $P'$: $\cov(e,P').$
\item Edges that cover $e',e$ and have endpoints in both $F_P$ and $F_{P'}$ (the fragments of $P$ and $P'$): $\cov_{\ell}(e',e)$.
\end{enumerate}

$\cov(P',P)$ is global information, that all vertices can learn in $O(D+n^{2/3})$ time as this is a bound on the number of pairs of highways. \mtodo{If we want a better complexity, we need to bound better the number of highways we actually compare, and in particular have some partitioning that really allows to bound this number better.}
The second term is known by $e'$, the third is known by $e$ and the last can be computed either in $F_P$ or in $F_{P'}$ using an aggregate computation in the fragment. Here we assumed that $e$ wants to compute $\cut(e',e)$. For this it needs to receive $\cov(e'),\cov(e',P)$ from $e'$. This requires from the highway $P'$ one aggregate computation to compute the value $\cov(e',P)$ for all edges $e' \in P'$ per highway $P$. Since the partitioning algorithm only fixes $O(1)$ edges $e' \in P'$ each time, we can also allow to send through a BFS tree all the values $\cov(e',P)$ for $e'$ we are interested in (at most $O(1)$ per fragment), and all highways $P$. The number of information if bounded by $O(n^{2/3})$ (this again is too expensive if we want a better complexity). Now $e$ has all information needed, and using one aggregate computation in $F_P$ is can compute $\cut(e',e)$ for a fixed $e'$. For all possibly $O(n^{1/3})$ edges $e'$ we fix, we need $O(n^{1/3})$ such aggregate computations. Then, we can use convergecast in a BFS tree to find the best $e \in P_H$, such that $cut(e',e)$ is minimal (before we only computed the best edge in each fragment), and we can send everybody the final result as we only consider $O(1)$ edges per fragment. 

I think the algorithm described above can be used to partition for example $P_H$ to subsegments according to $P'_H$. This actually seems to compute all the partitioning at once without iterations, but this idea is quite expensive, if we want a better complexity we should refine it (we can try to work in a binary search fashion, that allows decomposing the problem into disjoint problems, and not do all the computations at once). This doesn't really give the exact partitioning we want, because we also should break $P'_H$ to subsegments according to $P_H$. After we decide what is exactly the partitioning that we want, I guess similar ideas can hopefully be used to construct it.   

\subsubsection*{Second part: Finding the min 2-respecting cut} 
Here the goal would be to extend ideas from the non-highway-highway case. However, the actual computations needed would be more complicated, and in particular $\cov(e',e)$ is now split to more edges. As discussed above, when we fix two highways $P',P$ and look for the min cut with $e' \in P', e \in P$, we have: $$\cov(e',e)=\cov(P',P)+\cov(e',P)+\cov(e,P')+\cov_{\ell}(e',e).$$
We divide into cases, one case is that there are no edges between the fragments of $P'$ and $P$. Hence, $\cov_{\ell}(e',e)=0$, also note that the expression $\cov(P',P)$ does not depend on the specific choice of $e'$ and $e$, the expression $\cov(e',P)$ does not depend on $e$, and the expression $\cov(e,P')$ does not depend on $e'$. Remember that our goal is to minimize the expression $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e)$. This can be broken to the part $\cov(e')-2\cov(e',P)$ that depends only on $e'$, to the part $\cov(e)-2\cov(e,P')$ that depends only on $e$, and to the part $\cov(P',P)$ that does not depend on any of them. Hence, to minimize the expression we just need to find $e' \in P'$ such that $\cov(e')-2\cov(e',P)$ is minimized, and $e \in P$ such that $\cov(e)-2\cov(e,P')$ is minimized. $e'$ can be found using an aggregate computation in $P'$, and $e$ can be found using an aggregate computation in $P$. Then, we can send the information found (the edge, and the value it computed) to all vertices using a BFS tree. This is only $O(1)$ information per pair of highways $P',P$. In general, for all such computations we need $O(D+n^{2/3})$ time, since $O(n^{2/3})$ is a bound on the number of pairs, this complexity also allows all vertices to learn the value $\cov(P',P)$ for all pairs (getting a better complexity, requires a better bound on the number of pairs we compare). 

We next discuss the case that there are edges between the fragments of $P'$ and $P$. Here, basically we want to extend the idea described in the last case of the non-highway-highway algorithm. We decide which one of $P',P$ is responsible for the computations depending on the values $x_{P'}(P),x_P(P')$ (the number of edges in $P'$ compared to the highway $P$, and vice verse). Remember that we want that the partitioning we have would give that $\sum_{P} x_{P'}(P) = O(n^{2/3})$ and vice verse. If $x_{P'}(P) \leq x_P(P')$, we have that $P$ is responsible for the computations, it means it should compute the values $\cov(e',e)$ for $e \in P$, and $e' \in P'$ from the $x_{P'}(P)$ edges compared to $P$. The computation is as follows. Basically to be able to do this computation, for any relevant edge $e'$, it should get the values $\cov(e'), \cov(e',P).$ As discussed in the implementation of the partitioning, the rest of information needed: $\cov(e),\cov(e,P'), \cov(P',P), \cov_{\ell}(e',e)$ is either already known to $e \in P$ or can be computed using one aggregate computation in $T(P).$ Let's analyze the computation required by $P'$ and by $P$ for this case. In $P'$ we should compute the values $\cov(e',P)$ for all $e' \in P'$, and all highways $P$. Letting each edge $e' \in P'$ learn the information relevant for it requires one aggregate computation per highway $P$. Now we want to let all vertices in $T(P')$ learn the values $\cov(e',P)$ for all edges $e'$ that we want to compare to $P$ (we have $x_{P'}(P)$ such edges). Overall, we want to collect $\sum_{P} x_{P'}(P)$ information, which is $O(n^{2/3})$ by the partitioning. Then, we send the information to $T(P)$, using an edge between $T(P')$ and $T(P)$. In $T(P)$, we now need one aggregate computation per each one of the $x_{P'}(P) \leq x_P(P')$ edges $e' \in P'$, to compute the values $\cut(e',e).$ Doing so for all highways $P'$ from this case would result in a complexity of $O(n^{2/3}+\sum_{P'} x_{P'}(P))=O(n^{2/3})$ by the partitioning properties. This completes the case that $x_{P'}(P) \leq x_P(P')$. The other case is symmetric, and now $P'$ does the computations.

\subsection{Other cases}

There are additional cases that are not discussed here at all, maybe the most significant is the case that the two edges are in the \textbf{same root to leaf path}. Maybe some ideas described here can be useful for this case as well, but it seems that there are also different challenges for this case. For example, if we fix some long path of layer $i$ and want to compute the min 2-respecting cut that has both edges in the path, we don't have a vertex $r$ such that we know that one edge is below it and one is above it, so we need to split to different cases and hope that we can work on some of these cases in parallel.

Another case is that the two edges are in the same fragment, this is not dealt yet in all cases, but should probably be fine.

\subsection{An algorithm for two sub-paths}

\mtodo{a different way to look at things, that can hopefully generalize most of the cases.}

During our algorithm, many times we consider two sub-paths $P',P$ of length $O(\dfrag)$, and find the min 2-respecting cut that has one edge in $P'$, and one edge in $P$. We start by describing how to compare two such sub-paths.

\mtodo{we also need to discuss the case that we have one path.}

\mtodo{explain somewhere what is an aggregate computation in a sub-tree.}

\begin{lemma} \label{lemma_paths}
Let $P_0,P_1$ be two disjoint paths between an ancestor to its descendant in the tree, and assume that there is an edge $f$ between $T(P^{\downarrow}_0) \cap F_{P_0}$ and $T(P^{\downarrow}_1) \cap F_{P_1}$. \mtodo{we should see if in the same root to leaf path case we need some different condition on $f$.}
We denote by $x_{P_0}(P_1)$ the number of edges in $P_0$ that we compare to $P_1$, and by $x_{P_1}(P_0)$ the number of edges in $P_1$ that we compare to $P_0$.
For $i \in \{0,1\}$, at the beginning of the computation, the following information is known by all vertices in $T(P_i) \cap F_{P_i}$: \mtodo{Maybe there is some asymmetry and it's enough that one side would know some of the information, we should see in the proof}
\begin{enumerate}
\item The identity of all the edges in $P_i$ that we compare to $P_{1-i}$.
\item For each edge $e \in P_i$ that we compare to $P_{1-i}$, the values $\cov(e),\cov(e,P_{1-i})$.
\item The value $\cov(P_0,P_1).$
\item The identity of the edge $f$.
\end{enumerate}
Assume that $x_{P_0}(P_1) \leq x_{P_1}(P_0)$, then in $O(x_{P_1}(P_0))$ aggregate computations in $T(P_1) \cap F_{P_1}$, each edge $e \in P_1$ that we compare to $P_0$ would know the values $\cut(e,e')$ for all edges $e' \in P_0$ that we compare to $P_1.$
\end{lemma}

Some crucial observations that allow to compare many pairs of paths in parallel are the following.
First, we can work in parallel in disjoint sub-trees.

\begin{claim}
Let $P,P'$ be two sub-paths such that $T(P) \cap F_P$ and $T(P') \cap F_{P'}$ are edge-disjoint, then we can run aggregate computation in $T(P) \cap F_P$ and $T(P') \cap F_{P'}$ in parallel.
\end{claim}

Second, we can pipeline aggregate computations in a sub-tree.

\begin{claim} \label{claim_pipeline}
Assume that the path $P$ participates in the algorithms $A_1,A_2,...,A_k$, and in algorithm $A_i$ we run $x_i$ aggregate computations in $T(P) \cap F_P$, then running all the computations takes $O(\dfrag + \sum_{i=1}^{k} x_i)$ time.
\end{claim}

From Claim \ref{claim_pipeline}, to get a small time complexity we need to bound the value $\sum_{i=1}^{k} x_i$.
We next discuss that case that there is no edge between $P_0$ and $P_1.$

\begin{lemma} 
Let $P_0,P_1$ be two disjoint paths between an ancestor to its descendant in the tree, and assume that there is no edge between $T(P^{\downarrow}_0) \cap F_{P_0}$ and $T(P^{\downarrow}_1) \cap F_{P_1}$. \mtodo{we should see if in the same root to leaf path case we need some different condition on $f$.}
Then, given the values $\cov(P_0,P_1)$, as well as the values $\cov(e),\cov(e,P_0)$ for an edge $e \in P_1$ such that $\cov(e)-2\cov(e,P_0)$ is minimal, using one aggregate computation in $T(P_0) \cap F_{P_0}$, all vertices in $T(P_0) \cap F_{P_0}$ learn the values $e',e, \cut(e',e)$ for edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal.
\end{lemma}
}

==> paths_algorithm.tex <==


\mtodo{I'm currently still working on this part on a local version (and not directly on overleaf), so if you have any comment/want to change anything let me know.}

\mtodo{We should see if some of this should move to the preliminaries at the beginning of the paper.}

\subsection{Preliminaries} \label{sec:preliminaries_paths}

During our algorithm many times we run basic computations in trees, mostly in the trees $T(P)$ of non-highways, on the trees $F_P$ defined by fragments, and on a BFS tree of the graph. We next discuss such computations and explain how to run many such computations in a pipelined manner.

\paragraph{Broadcast.} In a broadcast computation, the root of the fragment has a message of size $O(\log n)$ to pass to the whole tree. 
This requires time proportional to the diameter of the tree, as the root starts by sending the message to its children, that in the next round pass it to their children, and so on. Note that the computation requires sending only one message on each one of the edges of the tree.

\remove{
\begin{claim}
Let $T'$ be a tree of diameter $O(D_{T'})$, and let $z$ be a message of size $O(\log n)$ initially known to the root. In $O(D_{T'})$ rounds, all vertices in $T'$ learn $z$. Moreover, the computation uses only edges of $T'$.
\end{claim}
}

\paragraph{Aggregate computation in a tree.} 

\mtodo{I discuss here aggregate computations, should see if we need it earlier, currently some variant appears earlier in the file.}

In an aggregate computation in a tree $T'$ (sometimes called convergecast), we have an associative and commutative function $f$ with inputs and output of size $O(\log n)$ (for example, $f$ can be sum or minimum).
Each vertex $v \in T'$ initially has some value $x_v$ of $O(\log n)$ bits, and the goal of each vertex is to learn the output of $f$ on the inputs $\set{x_v}_{v\in T'_{v}}$, where $T'_{v}$ is the subtree rooted at $v$. 

Computing an aggregate function is done easily, as follows. We start in the leaves, each one of them $v$ sends to its parent its value $x_v$, each internal vertex applies $f$ on its input and the inputs it receives from its children, and passes the result to its parent. The time complexity is proportional to the diameter of the tree. Moreover, the algorithm requires sending only one message on each one of the tree edges, which allows to pipeline such computations easily.

\begin{claim} \label{claim_pipeline}
Let $T'$ be a tree of diameter $D_{T'}$, and assume we want to compute $c_1$ broadcast computations and $c_2$ aggregate computations in $T'$. Then, we can do all computations in $O(D_{T'} + c_1 + c_2)$ time. Moreover, we can work in parallel in trees that are edge-disjoint.
\end{claim}

\begin{proof}
As explained above, each broadcast or aggregate computation requires $O(D_{T'})$ time, and the computation requires only communication on edges of the tree. To complete the proof, we explain how to pipeline the computations efficiently. By the description, each broadcast requires sending only one message from each vertex to each one of its children, when we go over the tree from the root to the leaves, hence clearly we can pipeline such computations. Similarly, an aggregate computation requires sending one message from each vertex to its parent, when we go over the tree from the leaves to the root, which can also be pipelined easily. Since the two types of computations send messages in opposite directions, they do not interfere with one another, and we can run broadcast and aggregate computations in the same time, which results in a complexity of $O(D_{T'} + c_1 + c_2)$ time.
\end{proof}

\paragraph{Tree computations in a fragment $F_P$.}

When we work on fragments $F_P$ during the algorithm, we use aggregate computations in two different directions. Recall that each fragment $F_P$, has a highway $P$, which is a path between the root $r_P$ and descendant $d_P$ of the fragment, and additional sub-trees attached to $P$ that are contained entirely in the fragment. We will need to do \emph{standard} aggregate computations as described above, where $r_P$ is the root, but also computation \emph{in the reverse direction}, where we think about $d_P$ as the root and orient all edges in the fragment accordingly. See Figure \ref{orientation_pic} for an illustration. 

\setlength{\intextsep}{2pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.5]{orientation.pdf}
 \caption{Possible orientations of the fragment $F_P$. On the left appears a standard orientation where $r_P$ is the root, and on the right appears an orientation where $d_P$ is the root. Note that the only edges that changed their orientation are highway edges.}
\label{orientation_pic}
\end{figure}

We next show that we can pipeline aggregate computations in both directions and broadcast computations efficiently.

\begin{claim} \label{claim_pipeline_fragment}
Let $F_P$ be a fragment with highway $P$, and assume we want to compute $c_1$ broadcast computations, $c_2$ aggregate computations, and $c_3$ aggregate computations in the reverse direction in $F_P$. Then, we can do all computations in $O(\dfrag + c_1 + c_2 + c_3)$ time. Moreover, we can work in parallel in different fragments.
\end{claim}

\begin{proof}
Pipelining of broadcast and aggregate computations is already discussed in the proof of Claim \ref{claim_pipeline}. We next explain how we pipeline also aggregate computations where $d_P$ is the root. To pipeline aggregate computations in two different directions (where $r_P$ and $d_P$ are the roots in the two computations), we work as follows. Note that orienting edges towards $d_P$ only changes the orientation of highway edges (see Figure \ref{orientation_pic} for an illustration), hence in all subtrees attached to the highway, the communication pattern in the two computations is identical, and we can just pipeline them as before. On highway edges, we send messages in opposite directions in both computations, hence they do not interfere and we can run them on the same time. To pipeline a broadcast (from $r_P$) and an aggregate computation with root $d_P$, we work as follows. On the subtrees attached to the highway, we send messages on opposite directions in these computations, hence they do not interfere. On highway edges, we send messages on the same direction, from $r_P$ towards $d_P$, since both computations send one message per edge in the same direction, we can just pipeline them, as we would pipeline two broadcast computations. This completes the proof.
\end{proof}


We next discuss additional notation and claims required.
We denote by $p(v)$ the parent of $v$.

\begin{claim} \label{claim_subtree}
Let $x$ be an edge that covers the tree edge $e=\{v,p(v)\}$, then $x$ has an endpoint in the subtree $T_v$ rooted at $v$.
\end{claim}

\begin{proof}
This follows as disconnecting $e$ from the tree leaves $T_v$ as one of the connected components. Any tree path that contains $e$ must have at least one vertex in this component, which shows that any edge that covers $e$ must have an endpoint in $T_v$. 
\end{proof}

For the algorithm, we first make sure that the highest and lowest edges in each highway are known to all vertices, which takes $O(D+\nfrag)$ time.

\begin{claim} \label{claim_high_low}
In $O(D+\nfrag)$ time all vertices can learn the highest and lowest edges in each highway.
\end{claim}

\begin{proof}
This requires collecting and sending $O(1)$ information per fragment, which can be done in $O(D+\nfrag)$ time using upcast and broadcast in a BFS tree.
\end{proof}

\subsection{An algorithm for two short paths}

During our algorithm, many times we consider two ancestor to a descendant sub-paths $P',P$ of length $O(\dfrag)$, and find the min 2-respecting cut that has one edge in $P'$, and one edge in $P$. We start by describing how to compare two such sub-paths.
We divide to cases according to whether $P'$ and $P$ are in a highway or not. In all our claims we assume that each edge $e$ knows the value $\cov(e)$, which can be obtained from Claim \ref{claim_learn_cov}.

\subsubsection*{Simple cases where $P'$ is a non-highway} \label{sec:non_highway_simple}


In this section we discuss the following cases:
\begin{enumerate}
\item $P'$ and $P$ are non-highways.
\item $P'$ is a non-highway and $P$ is the highway in the fragment of $P'$.
\item The two edges defining the cut are in the same non-highway path $P'$.
\end{enumerate}

We start with the following claim that is useful for cases involving a non-highway.

\begin{claim} \label{claim_non_highway}
Let $P'$ be a non-highway path, and let $e$ be an edge outside $T(P')$, such that $\{e,\cov(e)\}$ is known to all vertices in $T(P')$. 
Then, using one aggregate computation in $T(P')$, each edge $e' \in P'$ can compute the value $\cut(e',e).$ In addition, for different paths $P'$ that are not in the same root to leaf path, these computations can be done in parallel.
\end{claim}

\begin{proof}
Let $e' \in P'$. By Claim \ref{claim_cover}, $\cut(e',e)=\cov(e')+\cov(e)-2\cov(e',e)$. Also, $e'$ knows $\cov(e)$ and $\cov(e')$, hence to compute $\cut(e',e)$, the edge $e'$ should compute $\cov(e',e).$ As any edge that covers a tree edge $e'=\{v',p(v')\}$ where $p(v')$ is the parent of $v'$, has one endpoint in the subtree of $v'$ by Claim \ref{claim_subtree}, it follows that the edges that cover $e'$ and $e$ are exactly all the edges that cover $e$ and have exactly one endpoint in the subtree of $v'$. This subtree is contained in $T(P')$. Note that any edge $x$ that covers $e'$ and $e$ cannot have both endpoints in $T(P')$, as otherwise the tree path covered by $x$ is contained entirely in $T(P')$, but as $e$ is outside $T(P')$, $x$ cannot cover $e$ in this case, which leads to a contradiction.
Hence, to learn about the total cost of the edges that cover $e$ and $e'$ we need to do one aggregate computation in $T(P')$: letting each vertex $v' \in T(P'^{\downarrow})$ learn about the total cost of edges incident on the subtree of $v'$ that cover $e$. This can be done using a convergecast in $T(P')$, where each vertex sends to its parent the total cost of edges in its subtree that cover $e$, this includes the sum of costs of edges it receives from its children and the cost of such edges adjacent to it. To implement this efficiently we need an efficient way to determine for each non-tree edge whether it covers a specific edge $e$, this can be done using Claim \ref{claim_LCA_labels}. Hence, all the edges $e' \in P'$ can compute $\cut(e',e)$ using one aggregate computation in the subtree of $P'$.
Since the whole computation was done in $T(P')$, the same computation can be done in parallel for other paths not in the same root to leaf path with $P'$.
\end{proof}

Claim \ref{claim_non_highway} immediately solves the case that $P'$ is a non-highway and $P$ is either a non-highway above $P'$ in the same fragment, or the highway of the fragment of $P$, as we show next.

\begin{claim} \label{claim_non_highway_fragment}
Let $P'$ be a non-highway in the fragment $F_{P'}$ and assume that all vertices in $T(P')$ know the complete structure of $P'$. In $O(\dfrag)$ time, all edges $e' \in P'$, can compute the values $\cut(e',e)$ for all edges $e \in F_{P'}$ that are either above $P'$ in the same fragment, or in the highway of $F_{P'}$. The computation can be done in parallel for different paths $P'$ not in the same root to leaf path.
\end{claim}

\begin{proof}
First, using Claim \mtodo{add relevant claim to the decomposition section}, in $O(\dfrag)$ time, all edges $e'$ in the fragment of $P'$ can learn the values $\{e,\cov(e)\}$ for all edges $e$ on the paths between $e'$ to the root $r_{P'}$ and descendant $d_{P'}$ of the fragment $F_{P'}$. This can be done for all edges and all fragments simultaneously. If we focus our attention to edges $e' \in P'$, the paths it learned about contain some non-highway path above $e'$ that connects $e'$ to the highway, and all the edges of the highway $P$ of $F_{P'}$. If we exclude from these paths all edges contained in $P'$ (which can be done easily as $P'$ is known), we have that the rest of edges, denoted by $E'$, include exactly all non-highways above $P'$ in the fragment, and the highway $P$. All the edges of $E'$ are not in $T(P')$. Additionally, $|E'| = O(\dfrag)$, as it is composed of two paths inside the fragment. Hence, we can use Claim \ref{claim_non_highway}, and compute the values $\cut(e',e)$ for all $e' \in P', e \in E'$ using $O(\dfrag)$ aggregate computations. Using pipelining, the overall complexity is $O(\dfrag)$. As the computation was inside $T(P')$, it can be done in parallel for other paths not in the same root to leaf path.
\end{proof}

Also, we can adapt the proof of Claim \ref{claim_non_highway} to take care of the case that both edges defining the cut are in the same non-highway $P'$.

\begin{claim}
Let $P'$ be a non-highway, and assume that all vertices in $T(P')$ know all the values $\{e,\cov(e)\}_{e \in P'}$. Then, in $O(\dfrag)$ time, each edge $e' \in P'$, can compute the values $\cut(e',e)$ for all edges $e$ above it in $P'$. The computation can be done in parallel for different paths $P'$ not in the same root to leaf path.
\end{claim}

\begin{proof}
Fix an edge $e = \{v,p(v)\} \in P'$. Let $T_v \subset T(P')$ be the subtree rooted at $v$. We run an aggregate computation in $T_v$ to let all edges $e' \in T_v$ compute the value $\cut(e',e).$ The computation is identical to the computation described in the proof of Claim \ref{claim_non_highway}, with the difference that we stop the computation in $v$, i.e., the computation is only inside $T_v$ and not in $T(P')$, as $e \not \in T_v$, we can follow the same computation. At the end of the computation, all edges $e'$ below $e$ in $P'$ know the value $\cut(e',e).$ To do so for all edges $e \in P$, we pipeline the computations which takes $O(\dfrag)$ time.
\end{proof}

We are now left with the case that $P'$ and $P$ are orthogonal non-highways. We use Claim \ref{claim_non_highway} again to deal with this case. Note that the non-orthogonal case was already covered in Claim \ref{claim_non_highway_fragment}, as a non-highway path $P$ can be in the same root to leaf path with $P'$ only if they are in the same fragment, as the path from a non-highway path to the root is composed of a non-highway inside the fragment, and highways above it in other fragments. We will later show in our algorithm that we only compare orthogonal non-highway paths $P'$ and $P$ such that there is an edge between $T(P')$ and $T(P)$. Hence, we focus in this case.

\begin{claim}
Let $P'$ be a non-highway and let $P$ be a non-highway path not in the same root to leaf path with $P'$. Assume that there is an edge $f$ between $T(P'^{\downarrow})$ and $T(P^{\downarrow})$, that is known to all vertices in $T(P) \cup T(P').$
Also, assume that at the beginning of the computation all vertices in $T(P)$ know all values $\{e,\cov(e)\}_{e \in P}$. Then, in $O(\dfrag)$ time, all edges $e' \in P'$ can compute the values $\{e,\cut(e',e)\}_{e \in P}.$ The computation can be done in parallel for different paths $P'$ not in the same root to leaf path.
\end{claim}

\begin{proof}
As all vertices in $T(P)$ know the values $\{e,\cov(e)\}_{e \in P}$, and the edge $f$ has an endpoint in $T(P)$ and an endpoint in $T(P')$, it knows this information, and can pass it to all vertices in $T(P')$ using $O(\dfrag)$ aggregate and broadcast computations in $T(P').$ As $P$ and $P'$ are not in the same root to leaf path, we have that all edges $e \in P$ are not in $T(P')$, hence we can use Claim \ref{claim_non_highway} to let all edges $e' \in P'$ learn the values $\{e,\cut(e',e)\}$, this takes $O(\dfrag)$ time using pipelining.
\end{proof}

\subsubsection*{$P'$ is a non-highway and $P$ is a highway}

Here we focus on the case that $P'$ is a non-highway and $P$ is a highway in a different fragment. The case that $P$ is in the same fragment was already discussed in the previous section.
Let $e' \in P', e \in P$, we next look at the value $\cov(e',e).$ See Figure \ref{non_highway_highway} for an illustration.
We need the following definitions. 
\begin{itemize}
\item $\cov_{F}(e',e)$ is the cost of all edges that cover $e'$ and $e$ and have one endpoint in $T(P'^\downarrow)$ and one endpoint in the fragment $F_P$ of $P$.
\item $\cov(e',P)$ the cost of all edges that cover $e'$ and the whole highway $P$, and have one endpoint in $T(P')$ and both endpoints outside $F_P$.
\end{itemize}

We next show that all all the edges that cover $e'$ and $e$ are in one of the above categories.

\setlength{\intextsep}{0pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.4]{non_highway_highway.pdf}
 \caption{Examples of a non-highway $P'$ and a highway $P$. On the left, $P'$ and $P$ are orthogonal, and on the right, $P$ is above $P'$. The edges $x_1$ and $y_1$ are examples of edges counted in $\cov_F(e',e)$, and the edges $x_2$ and $y_2$ are examples of edges counted in $\cov(e',P).$}
\label{non_highway_highway}
\end{figure}

\begin{claim} \label{cover_non_highway_highway_new}
Let $e' \in P', e \in P$ where $P'$ is a non-highway, and $P$ is a highway in a different fragment $F_P$. Then $\cov(e',e) = \cov_{F}(e',e) + \cov(e',P)$.
\end{claim}

\begin{proof}
First note that by Claim \ref{claim_subtree}, any edge $x$ that covers $e'$ has one endpoint in the subtree $T(P'^\downarrow)$ which is inside the fragment $F_{P'}$ of $P'$. 
Now the edges that cover $e'$ and $e$ are all the edges with one endpoint in $T(P')$ that cover $e'$ and $e$. If the second endpoint of the edge is in the fragment $F_P$, these edges are counted in $\cov_{F}(e',e)$. To complete the proof, we need to show that any edge $x$ that covers $e'$ and $e$ and has both endpoints outside $F_P$, must cover the whole highway $P$. If $x = \{u,v\}$ covers both $e'$ and $e$ with both endpoints outside $F_P$ and $u \in T(P')$, the unique $u-v$ path in the tree starts in the fragment $F_{P'}$, and then enters and leaves the fragment $F_{P}$. From the structure of the decomposition, the only two vertices in $F_P$ that are connected by an edge to vertices outside the fragment are the ancestor $r_P$ and descendant $d_P$ of the fragment, hence any path that enters and leaves $F_P$ must include $r_P$ and $d_P$ and the whole path between them, which is the highway $P$. Hence, $x$ must cover the whole highway $P$ as needed. 
\end{proof}

We next explain how $\cov_{F}(e',e)$ and $\cov(e',P)$ are computed.

\paragraph{Computing $\cov_{F}(e',e)$.}

\begin{claim} \label{claim_covF_nh}
Let $P'$ be a non-highway and let $P$ be a highway of the fragment $F_P$. 
Given an edge $e \in P$, using an aggregate computation in $T(P')$, all edges $e' \in P'$ can compute the value $\cov_{F}(e',e)$.
\end{claim}

\begin{proof}
The proof is similar to the proof of Claim \ref{claim_non_highway}. When we fix an edge $e \in P$, computing $\cov_{F}(e',e)$ for all edges $e' \in P'$ is an aggregate computation in $T(P').$ This follows as the edges counted in $\cov_{F}(e',e)$ for $e' = \{v',p(v')\}$ are all the edges with one endpoint in the subtree of $v'$ (which is contained in $T(P')$) and one endpoint in $F_P$ that cover $e'$ and $e$. To compute the cost of those we just run an aggregate computation in $T(P')$. Note that for each edge $x$ with an endpoint $v$ in $T(P')$, $v$ knows if the second endpoint is in $F_P$, and also can deduce from the LCA labels using Claim \ref{claim_LCA_labels} whether $x$ covers $e$ and $e'$, which allows computing the aggregate function. At the end of the computation, each vertex $v' \in T(P')$ knows exactly the cost of edges in its subtree that cover $e'$ and $e$ with the second endpoint in $F_P$, which is exactly $\cov_{F}(e',e)$ for $e' = \{v',p(v')\}.$ 
\end{proof}

\begin{claim} \label{claim_covF_h}
Let $P'$ be a non-highway and let $P$ be a highway of the fragment $F_P$. 
Given an edge $e' \in P'$, using an aggregate computation in $F_P$, all edges $e \in P$ can compute the value $\cov_{F}(e',e)$.
\end{claim}

\begin{proof}
Here we break into cases according to the connection between $P'$ and $P$.
One case is that they are orthogonal, and one case is that $P$ is a highway above $P'$.
Note that from the structure of the decomposition, there are no other cases, as any path in the tree between a descendant and an ancestor starts with a non-highway and highways above it, so we cannot have $P'$ above $P$. Note also that all vertices know the complete structure of the skeleton tree, and can deduce accordingly in which one of the two cases we are.

\emph{Case 1: $P'$ and $P$ are orthogonal.} Here we know that $T(P')$ and $T(P)$ are disjoint, hence from Claim \ref{claim_subtree} it follows that all edges that cover $e' \in P$ and $e \in P$ have one endpoint in $T(P')$ and one endpoint in $T(P).$ Note that $T(P)$ is not necessarily contained in $F_P$, but since we are interested only in computing $\cov_{F}(e',e)$, we are only interested in edges with one endpoint in $T(P')$ and one endpoint in $T(P) \cap F_P$ that cover $e'$ and $e$. Computing the total cost of these edges requires one aggregate computation in $T(P) \cap F_P$, and follows exactly the computation described in the proof of Claim \ref{claim_covF_nh}.

\emph{Case 2: $P$ is above $P'$.} Here we need to do an aggregate computation in the reverse direction, to explain this we first take a closer look on edges that cover $e'$ and $e$ in this case. Since $e'$ is below $e$ in the tree, any tree path that contains both of them must include the whole tree path between them, which in particular includes a part between the descendent $d_P$ of the fragment $F_P$ to $e \in P.$ Hence, we need to sum the cost of edges that cover $e'$ and $e$ and also the whole path between $e$ and $d_P$. To compute it, it would be helpful to reverse the orientation in the fragment $F_P$, such that now $d_P$ is the \emph{root} of the fragment. Now if $e = \{v,d(v)\}$ where $d(v)$ is the vertex closer to $d_P$, all edges that cover $e'$ and the path between $e$ and $d_P$ and have an endpoint in $F_P$, must have an endpoint in the subtree of $v$ according to the new orientation (the subtree that includes everything below $v$ when we think about $d_P$ as the root). Hence, to compute the total cost of edges that cover $e'$ and $e$ and have one endpoint in $F_P$, we just do one aggregate computation in $F_P$ in the reverse direction to sum the costs of these edges. At the end of the computation, the vertex $v$ such that $e = \{v,d(v)\}$ knows exactly $\cov_F(e',e).$ Similarly, for each edge $e \in P$, one of its endpoints knows $\cov_F(e',e)$ as needed.
\end{proof}

\paragraph{Computing $\cov(e',P)$.}

\begin{claim} \label{claim_cov_eP_nh}
In $O(\dfrag + \nfrag)$ time, all edges $e'$ in the non-highway $P'$ can compute the values $\cov(e',P)$ for all highways $P$. Moreover, this computation can be done in all non-highways in the same layer simultaneously.
\end{claim}

\begin{proof}
Let $e' = \{v',p(v')\} \in P$, and fix a highway $P$. The edges that cover $e'$ have one endpoint in $T(P') \subseteq F_{P'}$ by Claim \ref{claim_subtree}. Hence, to compute the total cost of edges that cover $e'$ and the whole highway $P$ we just need to do one aggregate computation in $T(P').$ To implement the computation, we need to explain how given an edge $x$ we know if it covers the whole highway $P$ and if both its endpoints are outside $F_P.$ The second is immediate. For the first, note that $x$ covers the whole highway $P$ iff it covers the highest and lowest edges in the highway, since in this case it must cover the whole path between them which is the highway. As the highest and lowest edges in the highway are known to all vertices by Claim \ref{claim_high_low}, and since we can use LCA labels of edges to learn if $x$ covers some edge by Claim \ref{claim_LCA_labels}, we can compute the aggregate function. At the end of the computation, each vertex $v' \in P'$ knows the total cost of edges in its subtree that cover the whole highway $P$ and have both endpoints outside $F_P$, this is exactly $\cov(e',P)$ for the edge $\{v',p(v')\}.$
This requires one aggregate computation. To compute the values $\cov(e',P)$ for all highways we run $O(\nfrag)$ such computations, which results in $O(\dfrag + \nfrag)$ time as we pipeline the computations. As the whole computation was inside $T(P')$, we can run in parallel in disjoint subtrees, and in particular we can run the computations in parallel for all non-highways $P'$ in the same layer.
\end{proof}

\paragraph{An algorithm for two paths.}

We next explain how given a non-highway $P_0$ and a highway $P_1$ we compute the values $\{\cut(e',e)\}_{e' \in P_0, e \in P_1}.$ We start by discussing the case that there is an edge between $T(P_0)$ and $F_{P_1}.$

\begin{lemma} \label{lemma_paths_nh_h}
Let $P_0$ be a non-highway in the fragment $F_{P_0}$ and let $P_1$ be the highway of a different fragment $F_{P_1}$, and assume that there is an edge $f$ between $T(P_0^\downarrow)$ and $F_{P_1}$. 
Let $E_0 \subseteq P_0$ be a set of edges in $P_0$ we compare to $P_1$, and $E_1 \subseteq P_1$ be a set of edges in $P_1$ that we compare to $P_0$.
Additionally, assume that at the beginning of the computation the following information is known:
\begin{itemize}
\item All vertices in $T(P_0)$ know the identity of the edge $f$, The identity of all the edges in $E_0$, and for each edge $e' \in E_0$, the values $\cov(e'),\cov(e',P_1)$.
\item All vertices in $F_{P_1}$ know the identity of the edge $f$, the identity of all the edges in $E_1$, and for each edge $e \in P_1$, the value $\cov(e)$.
\end{itemize}

We can compute the values $\{\cut(e',e)\}_{e' \in P_0, e \in P_1}$ in the following two ways.
\begin{enumerate}
\item In $O(|E_1|)$ aggregate and broadcast computations in $T(P_0)$, where at the end of the computation each edge $e' \in E_0$ would know the values $\cut(e',e)$ for all edges $e \in E_1$. \label{P0_compute}
\item In $O(|E_0|)$ aggregate and broadcast computations in $F_{P_1}$, where at the end of the computation each edge $e \in E_1$ would know the values $\cut(e',e)$ for all edges $e' \in E_0$. \label{P1_compute}
\end{enumerate}
\end{lemma}

\begin{proof}
We start by proving Case \ref{P0_compute} where the computations are done in $T(P_0)$.
First, we use the edge $f$ that has an endpoint in $T(P_0)$ and an endpoint in $F_{P_1}$ to pass information from $F_{P_1}$ to $T(P_0)$.
As $f$ has an endpoint in $F_{P_1}$ it knows the values $\{e,\cov(e)\}_{e \in E_1}$ and can pass them to all vertices in $T(P_0)$ using $O(|E_1|)$ aggregate and broadcast computations in $T(P_0)$. Let $e' \in E_0, e \in E_1.$
From Claims \ref{claim_cover} and \ref{cover_non_highway_highway_new}, we have $$\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e,e'),$$ $$\cov(e',e) = \cov_{F}(e',e) + \cov(e',P_1).$$ An edge $e' \in E_0$ already knows $\cov(e')$ and $\cov(e',P_1),$ and from the broadcast it also knows the value $\cov(e)$ for all edges $e \in E_1.$ Hence, to compute the value $\cut(e',e)$ for a specific edge $e \in E_1$, it only needs to compute $\cov_{F}(e',e)$. By Claim \ref{claim_covF_nh}, all edges $e' \in P_0$ can compute the value $\cut(e',e)$ for a fixed $e$ using one aggregate computation in $T(P_0).$ To compute this value for all edges $e \in E_1$, we pipeline $|E_1|$ such aggregate computations, which concludes the proof of Case \ref{P0_compute}.   

We next discuss Case \ref{P1_compute}, where the computations are done in $F_{P_1}.$
Here we use $f$ to pass the information $\{e',\cov(e'),\cov(e',P_1)\}_{e' \in E_0}$ from $T(P_0)$ to $F_{P_1}$, which requires $O(|E_0|)$ broadcast and aggregate computation in $F_{P_1}$. Now, after this each edge $e \in E_1$ knows the value $\cov(e)$ as well as the values $\{e',\cov(e'),\cov(e',P_1)\}_{e' \in E_0}$. As discussed in the proof of Case \ref{P0_compute}, the only information missing to compute $\cut(e',e)$ is $\cov_{F}(e',e)$. Given an edge $e' \in E_0$, all edges $e \in P_1$ can compute $\cut(e',e)$ using one aggregate computation in $F_{P_1}$ by Claim \ref{claim_covF_h}. To do so for all edges $e' \in E_0$, we pipeline $|E_0|$ such aggregate computations, which completes the proof.
\end{proof}

We next discuss the case that there are no edges between $T(P_0)$ and $F_{P_1}.$
Let $P$ be a highway, we denote by $e^P_{min}$ the edge $e \in P$ such that $\cov(e)$ is minimal. First, we make sure that the values $\cov(e^P_{min})$ are known to all vertices.

\begin{claim}
In $O(D+\nfrag + \dfrag)$ time all vertices learn the values $\{e^P_{min}, \cov(e^P_{min})\}$ for all highways $P$.
\end{claim}  

\begin{proof}
First, in each highway, finding the edge $e^P_{min}$ requires an aggregate computation inside the fragment, which takes $O(\dfrag)$ time.
Next we send this information to all vertices.
As there is only one edge $e^P_{min}$ per highway, and there are $\nfrag$ highways, this only requires collecting and broadcasting $\nfrag$ information in a BFS tree, which takes $O(D+\nfrag)$ time.
\end{proof}

\begin{lemma}
Let $P_0$ be a non-highway, and $P_1$ be a highway in a different fragment, such that there are no edges between $T(P_0^\downarrow)$ and $F_{P_1}$. Then if each edge $e' \in P_0$ knows the values $\cov(e'),\cov(e',P_1)$, as well as the values $\{e^{P_1}_{min}, \cov(e^{P_1}_{min})\}$, using one aggregate and broadcast computations in $P_0$, all vertices in $P_0$ learn about the values $\{e',e,\cut(e',e)\}$ for edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal.
\end{lemma}

\begin{proof}
Let $e' \in P_0, e \in P_1$.
Again, from Claims \ref{claim_cover} and \ref{cover_non_highway_highway_new}, we have $$\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e,e'),$$ $$\cov(e',e) = \cov_{F}(e',e) + \cov(e',P_1).$$
Now if there are no edges between $T(P_0^\downarrow)$ and $F_{P_1}$, from the definition $\cov_{F}(e',e) = 0$ for any pair of edges $e' \in P_0, e \in P_1$, as this is the sum of costs of edges with one endpoint in $T(P_0^\downarrow)$ and the second in $F_{P_1}$.
Hence, in this case, we have $$\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e',P_1).$$ Note that the expression $\cov(e') - 2\cov(e',P_1)$ does not depend on the specific choice of $e \in P_1$, hence to minimize the expression $\cut(e',e)$ for a specific $e' \in P_0$, we just need to find an edge $e \in P_1$ where $\cov(e)$ is minimal, this is the edge $e^{P_1}_{min}$. As each edge $e' \in P_0$ knows the values $e^{P_1}_{min},\cov(e^{P_1}_{min}), \cov(e'),\cov(e',P_1)$ it can compute $\cut(e',e)$ for an edge $e \in P_1$ such that $\cut(e',e)$ is minimal. To find the minimum over all choices of $e'$ we just need one aggregate computation in $P_0$ to find the minimum value computed, we can then broadcast the information to let all vertices in $P_0$ learn the values $\{e',e,\cut(e',e)\}$ for edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal.
\end{proof}

\subsubsection*{$P'$ and $P$ are highways}

Let $e' \in P', e \in P$ be two tree edges in the highways $P',P$ such that $F_{P'},F_P$ are the fragments of $P'$ and $P$, respectively. The value $\cov(e',e)$ is broken up to the following different parts. See Figure \ref{highway_highway} for an illustration.

\begin{enumerate}
\item The cost of edges that cover entirely the highways $P$ and $P'$, with endpoints outside $F_{P'} \cup F_P$: $\cov(P',P).$ 
\item The cost of edges with one endpoint in $F_{P'}$ and one endpoint outside $F_{P'} \cup F_P$ that cover $e'$ and the whole highway $P$: $\cov(e',P).$
\item The cost of edges with one endpoint in $F_{P}$ and one endpoint outside $F_{P'} \cup F_P$ that cover $e$ and the whole highway $P'$: $\cov(e,P').$
\item The cost of edges that cover $e',e$ and have endpoints in both $F_P$ and $F_{P'}$: $\cov_{F}(e',e)$.
\end{enumerate}

To see that these are all the options we use the structure of the decomposition. 

\setlength{\intextsep}{0pt}
\begin{figure}[h]
\centering
\setlength{\abovecaptionskip}{-2pt}
\setlength{\belowcaptionskip}{6pt}
\includegraphics[scale=0.4]{highway_highway.pdf}
 \caption{Example of two highways $P'$ and $P$, for the special case that the tree is a path, and $P$ and $P'$ are subpaths of it. The edges $x_1,x_2,x_3,x_4$ are counted in $\cov(P',P),\cov(e',P),\cov(e,P'),\cov_F(e',e)$, respectively.}
\label{highway_highway}
\end{figure}

\begin{claim} \label{claim_cov_highways}
Let $e' \in P', e \in P$ be two tree edges in the highways $P',P$. Then, $$\cov(e',e) = \cov(P',P) + \cov(e',P) + \cov(e,P') + \cov_{F}(e',e).$$
\end{claim}

\begin{proof}
First, if $x = \{u,v\}$ is an edge that covers $e \in P$, then the unique tree path between $u$ and $v$ contains $e$. As the the only vertices in $F_{P}$ that are connected by an edge to a vertex outside $F_{P}$ are the root $r_P$ and unique descendant $d_P$ of the fragment, any path in the tree that contains $e$ and have both endpoints outside the fragment, must also contain the whole highway between $r_P$ and $d_P$ (as otherwise, at least one of the endpoints would be inside the fragment). Hence, if both endpoints of $x$ are outside $F_P$, it covers the whole highway $P$. 

Now any edge $x$ that covers $e'$ and $e$, has the following options.
\begin{enumerate}
\item $x$ has both endpoints outside $F_{P'}$ and $F_P$, in this case it follows that $x$ must cover the whole highways $P'$ and $P$, which is exactly counted by $\cov(P',P).$
\item $x$ has one endpoint in $F_{P'}$ but two endpoints outside $F_P$, in this case $x$ must cover the whole highway $P$, which is exactly counted in $\cov(e', P).$
\item $x$ has one endpoint in $F_{P}$ but two endpoints outside $F_{P'}$, in this case $x$ must cover the whole highway $P'$, which is exactly counted in $\cov(e, P').$
\item $x$ has two endpoints in $F_{P'} \cup F_{P}$, in this case it must be the case that $x$ has one endpoint in $F_{P'}$ and one endpoint in $F_{P}$, as otherwise the unique tree path defined by $x$ is contained entirely in one of the fragments and cannot cover both edges $e' \in P', e \in P$. This is counted by $\cov_{F}(e',e)$.
\end{enumerate} 
\end{proof}

We next explain how we compute the different ingredients in the expression $\cov(e,e').$

\paragraph{Computing $\cov(P,P')$.}

\begin{claim}
Let $P,P'$ be two highways. Using one aggregate and one broadcast computation in a BFS tree, all vertices can learn $\cov(P,P')$. Computing this value for $k$ different pairs takes $O(D+k)$ time.
\end{claim}

\begin{proof}
Given some edge $x = \{u,v\}$, it knows if its endpoints are outside $F_P \cup F_{P'}$. In addition, it can learn if it covers the highway $P$ as follows. An edge $x$ covers the whole highway $P$ iff it covers both the highest and lowest edges in $P$: $e_1, e_2$, because in this case it follows that the unique tree path between $u$ and $v$ contains the unique tree path between $e_1$ and $e_2$ which is the highway $P$. Using the LCA labels of edges and Claim \ref{claim_LCA_labels}, $x$ can learn if it covers $e_1,e_2$. Similarly, $x$ can learn if it covers the whole highway $P'$, and then deduce if it covers both $P$ and $P'$. Now to compute $\cov(P,P')$ we sum the cost of all edges that cover both $P$ and $P'$ and have both endpoints outside $F_P \cup F_{P'}$, this is a sum of values that can be computed using an aggregate computation in a BFS tree. For each edge $x$ outside $F_P \cup F_{P'}$ that covers both $P$ and $P'$, one of its endpoints represents $x$ in the computation, and adds its cost to the sum computed. To let all vertices learn the value $\cov(P,P')$ we use a broadcast in the BFS tree. If we have $k$ different pairs, we pipeline the computations to get a complexity of $O(D+k)$.    
\end{proof}

\paragraph{Computing $\cov_F(e',e)$.}

\begin{claim} \label{claim_covl}
Let $P,P'$ be highways of the fragments $F_P$ and $F_{P'}$, respectively, and let $e \in P$.
Using one aggregate computation in $F_{P'}$, all edges $e' \in P'$ can compute the value $\cov_{F}(e',e)$.
\end{claim}


\begin{proof}
If we look at the highways $P$ and $P'$, there are several cases:
\begin{enumerate}
\item $P$ and $P'$ are orthogonal. \label{case_or}
\item $P$ and $P'$ are in the same root to leaf path with $P'$ below $P$. \label{case_below}
\item $P$ and $P'$ are in the same root to leaf path with $P$ below $P'$. \label{case_above}
\end{enumerate}
Note that all vertices know the complete structure of the skeleton tree, hence they can distinguish between the cases.
We start with the first two cases.

\emph{Cases \ref{case_or} and \ref{case_below}}. In these cases, we show that any edge $x$ that covers $e \in P$ and some edge $e' = \{v',p(v')\} \in P'$ and has endpoint in $F_{P'}$ has an endpoint in the subtree of $v'$ in $F_{P'}$. 
This is justified as follows. We know that any edge $x$ that covers $e'$ has an endpoint $u$ in the subtree rooted at $v'$ by Claim \ref{claim_subtree}. Assume to the contrary that $u \not \in F_{P'}$, but rather the second endpoint of $x$, $u'$, is in $F_{P'}$. Now the path between $u$ and $u'$ has a part in $F_{P'}$, and a part below it, as $u$ is in the subtree rooted at $v' \in P'$. This path can only cover edges in $F_{P'}$ or below it, but we are in the case that $P$ is orthogonal to $P'$ or above it, hence it does not have any edge in $F_{P'}$ or below it, which means that $x$ cannot cover $e \in P$, a contradiction.

Hence, we know that any edge that covers $e \in P$ and $e' \in P'$ and also has an endpoint in $F_{P'}$ has an endpoint in $T(P') \cap F_{P'}$.
Hence, given an edge $e \in P$, computing the values $\cov_{F}(e',e)$ for all edges $e' \in P'$ requires one aggregate computation in $F_{P'}$, in which every vertex $v' \in F_{P'}$ learns the total cost of edges adjacent to its subtree in $F_{P'}$ that cover also $e$, and have the second endpoint in $F_P$. As explained in the proof of Claim \ref{claim_non_highway} this is an aggregate computation in the subtree, and it can be computed as for each non-tree edge $x$ we can deduce it it covers $e$ using its LCA labels (see Claim \ref{claim_LCA_labels}). At the end of the computation, the vertex $v'$ such that $e' = \{v',p(v')\}$ knows exactly the value $\cov_{F} (e',e).$

\emph{Case \ref{case_above}.} In this case $P$ and $P'$ are in the same root to leaf path with $P$ below $P'$. 
Let $e' \in P', e \in P$, we start by analysing the structure of edges that cover $e'$ and $e$ in this case. Since $P$ is below $P'$, any edge $x$ that covers $e'$ and $e$ covers the whole path between $e'$ and $e$. In particular, it covers the whole path between $e' \in P'$ to the unique descendant $d_{P'}$ of the fragment $F_{P'}$. Hence, we need to sum the costs of edges that cover $e'$ and $e$, have endpoints in $F_{P'}$ and $F_P$, and also cover the whole path between $e'$ and $d_P$.
To compute the cost of these edges, it would be helpful to change the orientation in the fragment $F_{P'}$, such that now $d_{P'}$ is the \emph{root}. We write $e' = \{v,d(v)\}$ where $d(v)$ is the vertex closer to $d_{P'}$ (this is the reverse orientation compared to the previous cases). Now, given an edge $e \in P$, we want to compute the total cost of edges adjacent to the subtree of $v$ in $F_{P'}$ that cover $e,e'$ and have the second endpoint in $F_P$, where the subtree is with respect to the new orientation (having $d_{P'}$ as the new root). This gives exactly $\cov_{F} (e',e).$ Again, this is an aggregate computation in the fragment $F_{P'}.$

Note that the aggregate computation in Case \ref{case_above} is in a different direction than the aggregate computations in Cases \ref{case_or} and \ref{case_below}. However, since all vertices know the structure of the skeleton tree, they all know in which case we are, and can change the orientation accordingly, which only requires changing the orientation for highway edges, as discussed in Section \ref{sec:preliminaries_paths}.
\end{proof}

\paragraph{Computing $\cov(e,P)$.}

\begin{claim} \label{claim_cov_eP}
In $O(\dfrag + \nfrag)$ time, all edges $e$ that are in a highway can compute the values $\cov(e,P)$ for all highways $P$.
\end{claim}

\begin{proof}
First, we fix two highways $P',P$, and show how all edges $e' \in P'$ compute $\cov(e',P).$ 
The edges that cover $e'$ and the whole highway $P$ are exactly the edges that cover $e'$ and the highest and lowest edges in $P$: $e_1,e_2.$
To compute $\cov(e',P)$, which is the sum of all such edges that have one endpoint in $F_{P'}$ and one endpoint outside $F_{P'} \cup F_{P}$ we use an aggregate computation in $F_{P'}$. This aggregate computation is very similar to the computation done in the proof of Claim \ref{claim_covl}, with the difference that now instead of summing the cost of edges that cover $e'$ and a specific edge $e$, we sum the cost of edges that cover $e'$ and $e_1,e_2$, and also make sure that the second endpoint is not in $F_{P'} \cup F_{P}$, the computation can be done in the same manner. For each highway we have one aggregate computation to compute $\cov(e',P)$ for all edges $e' \in P'.$ To do so for all highways $P$, we need $\nfrag$ such computations. Since the whole computation was done inside $F_{P'}$, we can do the same computation in all fragments simultaneously, the overall complexity is $O(\dfrag + \nfrag)$.
\end{proof}

\paragraph{An algorithm for two paths.}

We next explain how given two highways $P_0,P_1$, we compute $\cut(e',e)$ for edges $e' \in P_0, e \in P_1$. We start with the case that there is an edge between $F_{P_0}$ and $F_{P_1}.$

\begin{lemma} \label{lemma_paths}
Let $P_0,P_1$ be two disjoint highways, and assume that there is an edge $f$ between $F_{P_0}$ and $F_{P_1}$. 
Let $E_0 \subseteq P_0$ be a set of edges in $P_0$ we compare to $P_1$, and $E_1 \subseteq P_1$ be a set of edges in $P_1$ that we compare to $P_0$.
For $i \in \{0,1\}$, at the beginning of the computation, the following information is known by all vertices in $F_{P_i}$: 
\begin{enumerate}
\item The identity of all the edges $E_i$.
\item For each edge $e \in E_i$, the values $\cov(e),\cov(e,P_{1-i})$.
\item The value $\cov(P_0,P_1).$
\item The identity of the edge $f$.
\end{enumerate}
We can compute the values $\{\cut(e',e)\}_{e' \in P_0, e \in P_1}$ in the following two ways.
\begin{enumerate}
\item In $O(|E_1|)$ aggregate and broadcast computations in $F_{P_0}$, where at the end of the computation each edge $e' \in E_0$ would know the values $\cut(e',e)$ for all edges $e \in E_1$. 
\item In $O(|E_0|)$ aggregate and broadcast computations in $F_{P_1}$, where at the end of the computation each edge $e' \in E_1$ would know the values $\cut(e',e)$ for all edges $e \in E_0$. 
\end{enumerate}
\end{lemma}

\begin{proof}
We focus on the case where the computations are done in $F_{P_1}$, the second case is symmetric.
We work as follows. First, we use the edge $f$ to pass information from $F_{P_0}$ to $F_{P_1}$. Note that all vertices in $F_{P_0}$, know all the values $\{\cov(e),\cov(e,P_1)\}_{e \in E_0}$. Since $f$ has one endpoint in  $F_{P_0}$ it knows this information and can pass it to all vertices in $F_{P_1}$ using $O(|E_0|)$ aggregate and broadcast computations. Now, for each edge $e \in E_0$, we run one aggregate computation in $F_{P_1}$, that allows each edge $e' \in P_1$ compute $\cut(e,e').$ This is done as follows. First, by Claim \ref{claim_cover}, we know that $\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e,e').$ Also, by Claim \ref{claim_cov_highways}, $\cov(e',e) = \cov(P_0,P_1) + \cov(e',P_0) + \cov(e,P_1) + \cov_{F}(e',e)$. Now, for $e' \in E_1$, it already knows $\cov(e'), \cov(e',P_0), \cov(P_0,P_1)$ at the beginning of the computation. Also, it learns the values $\cov(e),\cov(e,P_1)$ as $f$ passed this information to $F_{P_1}$. Hence, the only thing missing to complete the computation is computing $\cov_{F}(e',e)$ which requires one aggregate computation in $F_{P_1}$ per edge $e \in E_0$ by Claim \ref{claim_covl}. To compute the values $\cut(e',e)$ for all $e \in E_0$, we pipeline $O(|E_0|)$ such computations, which completes the proof.
\end{proof}

We next consider the case that there is no edge between $F_{P_0}$ and $F_{P_1}$.

\begin{lemma} 
Let $P_0,P_1$ be two disjoint highways, and assume that there is no edge between $F_{P_0}$ and $F_{P_1}$. 
Then, given the values $\cov(P_0,P_1)$, using one aggregate computation in $F_{P_0}$ and in $F_{P_1}$, 
and by communicating $O(1)$ information over a BFS tree, all vertices learn the values $e',e, \cut(e',e)$ for edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal.
\end{lemma}

\begin{proof}
Let $e' \in P_0, e \in P_1$. By Claim \ref{claim_cover}, we have $\cut(e,e') = \cov(e) + \cov(e') - 2\cov(e,e').$ Also, by Claim \ref{claim_cov_highways}, $\cov(e',e) = \cov(P_0,P_1) + \cov(e,P_0) + \cov(e',P_1) + \cov_{F}(e',e)$. Now since there are no edges between $F_{P_0}$ and $F_{P_1}$, by definition $\cov_{F}(e',e) = 0$ as this is the sum of costs of edges between $F_{P_0}$ and $F_{P_1}$ that cover $e'$ and $e$. Also, $\cov(P_0,P_1)$ does not depend on the specific choice of $e'$ and $e$. Hence, if we want to minimize the expression $\cut(e,e')$, it is equivalent to minimizing the expression $(\cov(e) - 2\cov(e, P_0)) + (\cov(e') - 2\cov(e',P_1))$. Note that the expression $\cov(e) - 2\cov(e, P_0)$ does not depend on $e'$, and the expression $\cov(e') - 2\cov(e',P_1)$ does not depend on $e$. Hence, minimizing the whole expression is equivalent to minimizing each one of the expressions separately.
We next show that we can find $e \in P_1$ such that $\cov(e) - 2\cov(e, P_0)$ is minimal, as well as compute this value using one aggregate computation in $P_1$. Similarly, we can find $e' \in P_0$ such that  $\cov(e') - 2\cov(e',P_1)$ is minimal using one aggregate computation in $P_0.$
Then, if $P_0$ sends the message $P_0, e', \cov(e') - 2\cov(e',P_1)$, and $P_1$ sends the message $P_1, e, \cov(e) - 2\cov(e, P_0)$, for the minimal edges found, using a BFS tree, all vertices can compute the values $e',e,\cut(e',e)$ for the edges $e' \in P_0, e \in P_1$ such that $\cut(e',e)$ is minimal. As discussed above, this value equals to $(\cov(e) - 2\cov(e, P_0)) + (\cov(e') - 2\cov(e',P_1)) - 2\cov(P_0,P_1)$, and we assume that $\cov(P_0,P_1)$ is known.

Hence, to complete the proof, we explain how to compute $\cov(e) - 2\cov(e, P_0)$ in $P_1$ (the equivalent computation in $P_0$ is done in the same way). From Claim \ref{claim_cov_eP}, all edges $e \in P_1$ know the value $\cov(e,P_0)$, and they also know $\cov(e)$. Hence, each edge $e \in P_1$ knows the value $\cov(e) - 2\cov(e, P_0)$. To find the edge $e$ that minimizes this expression, we only need to run one aggregate computation in $P_1$ for finding the minimum.
\end{proof}

==> preamble.tex <==
\usepackage[bookmarks,colorlinks,breaklinks]{hyperref}
\hypersetup{urlcolor=blue, colorlinks=true, citecolor=green!50!black, linkcolor=blue}
\usepackage[letterpaper, left=1in, right=1in, top=0.9in, bottom=0.9in]{geometry}
\usepackage[utf8]{inputenc}
\usepackage[american]{babel}



\usepackage[normalem]{ulem}

% Graphics
\usepackage{graphicx}
\graphicspath{{images/}{../images/}}

\usepackage{amsmath, amssymb, cases}
\usepackage{theoremstyles}
\usepackage{cleveref}
\usepackage{enumitem}
%\usepackage{natbib}
\usepackage{mdframed}
\usepackage{bbm}
\usepackage{bm}

%\usepackage{algorithmicx}               
%\usepackage{algorithm}
\usepackage[ruled]{algorithm}
\usepackage[]{algpseudocode}

 
\usepackage{microtype}

\usepackage{mdframed}
\usepackage{xcolor}

\bibliographystyle{alpha}% the recommended bibstyle



\input{commands}
